Simple Cues Lead to a Strong Multi-Object Tracker

For a long time, the most common paradigm in Multi-Object Tracking was tracking-by-detection (TbD), where objects are first detected and then associated over video frames. For association, most models resourced to motion and appearance cues, e.g., re-identification networks. Recent approaches based on attention propose to learn the cues in a data-driven manner, showing impressive results. In this paper, we ask ourselves whether simple good old TbD methods are also capable of achieving the performance of end-to-end models. To this end, we propose two key ingredients that allow a standard re-identification network to excel at appearance-based tracking. We extensively analyse its failure cases, and show that a combination of our appearance features with a simple motion model leads to strong tracking results. Our tracker generalizes to four public datasets, namely MOT17, MOT20, BDD100k, and DanceTrack, achieving state-of-the-art performance. https://github.com/dvl-tum/GHOST.

==> chapters/Intro.tex <==
\section{Introduction}
\label{sec:intro}
\iffalse
\begin{itemize}
    \item Multi-object tracking (MOT) aims to track multiple objects over video sequences
    \item classic paradigm tracking-by-detection
    \item nowadays also joint detection and tracking
    \item trackers use location, motion and appearance cues
    \item Recently trackers leverage sophisticated motion models as well as embedded ReID
    \item We provide a strong baseline for Multi-Object Tracking
    \item We claim depsite its simplicity a mixture of a simple ReID and a simple motion model is enough to achieve state of the art
    \item Contributions: Analysis when motion and when ReID, show that simple motion model and ReID complement each other, achieve state of the art.
\end{itemize}
\fi

% MOT and TbD
We revise Multi-Object Tracking (MOT) which aims at finding the trajectories of all moving objects in a video. The dominant paradigm in the field is Tracking by Detection (TbD), which consists in first detecting objects across video frames, and then linking them into temporally coherent trajectories, i.e., performing \textit{data association}. While the performance of approaches following the TbD paradigm can be significantly improved by the underlying detections, we focus on the less studied yet profoundly important association step. \ili{do we need the last sentence? every tracking paper focuses on the association step.}

% Criticism of field/motivation
\ili{agree that it is too long, and needs to be more conciser}
\alj{This section is too verbose. Also, unsure about the message. The message appears as “do we need complex frameworks for data assoc”, but I think this has been questioned and answered over and over: turns out that with good detectors and ReID models, once can get away with the most simplistic association techniques (Hungarian, greedy based on regressed offset as in centertrack, etc)} \jenny{I'm not 100\% sure about what would be the optimal message here then.}
Advances in learning-based object detectors have benefited the field, as evidenced by the widespread adoption of Faster R-CNN variants among top-performing approaches \REF. In contrast, progress in data association has been \textcolor{red}{more difficult to observe}, as current state-of-the-art methods have taken seemingly divergent paths. However, there is a common theme among them: a strong focus on sophisticated learning-based pipelines. Some examples are attention-based networks \REF, graph neural networks \REF or end-to-end joint detection and embedding frameworks \REF, as well as the trend of using increased amounts of labelled data such as single-image training \REF. %As a consequence of their focus on learning, recent methods also tend to have increased needs for training data. 
Given the significant differences and increasing complexity of these approaches, comparisons among them are notoriously difficult. Moreover, it is unclear which advances are driving progress in the field. These issues make the following question arise: \textit{do we really need to use sophisticated learning-based frameworks for data association?}

\jenny{Ideas for the upper paragraph: we show how much we can improve the performance by taking a step back and re-visting morion and ReID cues.}


% Overview of our approach
In this work, we address this question by showing that taking a step back and re-visting the association step can significantly improve upon complex state-of-the-art methods on \textcolor{red}{several} datasets. We show that by exploiting motion and appearance, which are standard cues, within a well-known online TbD framework, we can obtain a strong tracker. Our tracker, without bells and whistles, outperforms state-of-the-art trackers, and we demonstrate with our experimental analysis that our strong performance originates from improved data association.
\jenny{can we say this? If we would use purely the detections of QDTrack for example it would not be as good as it is now}, 


% More detailed explanation of our appraoch
% \alj{Also this section, rephrase. Bi-partite matching is probably irrelevant at this stage. Seems to me that at the core of your method are the appearance and motion model, and “a policy” on how/when trust whom, or how to combine them? Dont use words such as “simple tricks”!}
Our approach consists of a matching-based tracker that leverages a single affinity score taking appearance and motion cues between past tracks and current detections, at every frame into account.
%
We obtain our appearance term from a standard re-identification (ReID) network, whose performance we enhance with two design choices: different handling of active and inactive tracklets and on-the-fly domain adaptation.
%
Our motion term relies on the predictions of a linear motion model over past tracks. 
%
Undertaking an extensive analysis we determine three factors, namely, visibility, occlusion time, and camera movement, that heavily influence the performance of ReID and motion, respectively. \ili{i think that the previous sentence should not be here, but somewhere in methodology.} Based on those three factors we introduce a policy to determine in which scenarios motion and ReID give a more trustworthy similarity predictions and combine the appropriately.
%
%Overall, we show how to design a strong prior on tracking behavior combining simple features that outperforms sophisticated learning-based predictions.  

% Our message
We expect our work to serve two main purposes. First, to demonstrate that given good detections, data association can be mostly solved with a strong yet simple association scheme. We believe that this is valuable by itself, and expect it to make future work question the need for sophisticated learning-based approaches. Second, the analysis we conduct to derive our tracking policy sheds light on what are the pressing challenges of tracking that both our method as well as previous top-performing ones still struggle to address. We hope that the insights we derive will encourage subsequent methods to target their effort towards solving them.
%
Overall, we make the following contributions:
\begin{itemize}
    \item We provide a strong scheme for data association combining simple appearance and motion cues with a policy derived from an analysis of their applicability under different tracking conditions.
    \item We obtain state-of-the art results on several benchmarks, etc. \ili{more precise, give numbers already}
\end{itemize}




\ili{too much mentioning of the simple, also we should add another contribution, maybe something with respect to analysis.}

%In this work, we take a step back and address show that a simple baseline with minimal learning involved
\iffalse
Rough structure:
\noindent{\textbf{1) Background + Motivation}}
\begin{itemize}
\item[$\bullet$]   MOT definition, TbD=det + data association,  it's still the dominant paradigm.
\item[$\bullet$]  Progress in detection has clearly benefited tracking (cite MOTCha paper), and most TbD approaches stick to standard FRCNN and variants.
\item[$\bullet$] (Criticism of status of field:) But progress in data association has been less clear, as different methods have taken seemingly completely different directions. Common trends:
\begin{itemize}
\item Strong focus on learning with ever increasing complexity in architectures (attention, GNNs, e2e detection+appearance)
\item Increase in data needs (e.g. extra datasets, single-image training) 
\item Generally, methods still exploiting classical appearance and motion cues, but possibly in fancy ways.
\end{itemize}
\item[$\bullet$] Comparisons among methods are hard, and it's overall unclear what's driving progress in the field. Do we really need all the fancy stuff?
\end{itemize}
\noindent{\textbf{2) Our solution}}
\begin{itemize}
\item[$\bullet$] High-level view of contribution: We take a step back, and show that appearance and motion cues can be exploited in a remarkably simple way, and without any complex learning scheme. Despite its simplicity, we demonstrate that when evaluated on the same detections of other trackers, our approach consistently outperforms sophisticated methods
\item[$\bullet$]Method overview: our approach consists of a simple bipartite-matching-based online tracker, that combines an appearance term with a motion term to obtain a single cost.
\begin{itemize}
	\item  Our appearance term comes from the embedding similarity produced by a standard ReID network, with some simple tricks. 
	\item Our motion term comes from the prediction of a simple linear motion model
	\item Our policy to combine them is derived from an extensive analysis of the performance of these two terms. 'We replace learning by 'analysis' and manually setting strong priors' kinda argument'.
\end{itemize}
\item[$\bullet$] (Wrap-up again? maybe skip) despite the simplicity of our features and (lack/simplicity) of our learning scheme, we show that our approach systematically outperforms SOTA methods when evaluated over the same set of detections --> We show superior association! 
\end{itemize}
\noindent{\textbf{3) General message and contributions}}
\begin{itemize}
\item[$\bullet$] Our message: given good detections, data association can be mostly solved with a simple scheme Future methods should make sure that
\begin{itemize}
\item[$\bullet$] They can surpass this baselines before resourcing to fancy learning-based approaches
\item[$\bullet$] They focus on the bits of tracking such as long-term association that, as showed in our analysis, remain unaddressed
\end{itemize}
\item[$\bullet$] Our contributions:
\begin{itemize}
\item[$\bullet$] Simple strong baseline
\item[$\bullet$] Analysis
\item[$\bullet$] SOTA results
\end{itemize}

\end{itemize}

\fi

==> chapters/intro_shortened.tex <==
\section{Introduction}

% intro to tracking and TBD
Multi-Object Tracking (MOT) aims at finding the trajectories of all moving objects in a video. The dominant paradigm in the field has been tracking-by-detection, which divides tracking into two steps: (i) frame-wise object detection, (ii) data association to link the detections and form trajectories. 
%
In online tracking, where only the past is accessible, one of the simplest forms of data association is frame-by-frame matching using the Hungarian algorithm~\cite{hungarian} %\ili{should you define what are online trackers before mentioning them?}. %\lau{Unsure whether to mention offline trackers, maybe not, only at related work we do LP, MPN, etc)}.
%
Matching is then driven by cues such as appearance, \eg, re-identification (reID) features \cite{DBLP:conf/cvpr/0004GLL019,DBLP:journals/corr/HermansBL17,DBLP:conf/iccv/QuanDWZY19,DBLP:conf/cvpr/ChengGZWZ16,DBLP:conf/eccv/SunZYTW18,DBLP:conf/eccv/VariorHW16,DBLP:conf/cvpr/ZhangLZ019} or motion cues \cite{DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/nips/RenHGS15,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/eccv/PengWWWWTWLHF20}.
%

%Obtaining robust appearance and motion cues even evolved as tasks on their own, namely, re-identification and trajectory prediction. \lau{cite,cite} \gui{Is this true? I see ReID as a task on its own: e.g. chinese government wants to fine you --> it needs to retrieve you from database, doesn't care about your trajectory. Or trajectory prediction is needed for action planning in autonomous driving, regardless of tracking. no?}
%



%Even new learning-based trackers are in need of motion and appearance cues, \eg, Tracktor \cite{DBLP:conf/iccv/BergmannML19} uses external reID and motion priors.
%
Recent learning-based trackers still rely on motion priors~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20} or appearance cues, which may include external reid models~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/WuCS00Y21}. 
%
Modern trackers based on Transformers \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247} learn all necessary cues from data through self- and cross-attention between frames and tracked objects.
%
While powerful, these methods rely on large amounts of training data, e.g., pre-training on the large scale CrowdHuman~\cite{crowdhuman} has become a necessity to obtain state-of-the-art results. %\jenny{actually just realized that this is also done for Byte detections. Maybe we can change it somehow that using an off the shelf object detector pretrained also on several datasets is way easier / that the pre-trainig is a game changer / performance boost for the methods.} \lau{I think the main difference here is that you need to train the whole tracker with these extra datasets, which we do not do, so i think the message can still be said this way. Ofc we use strong private detections, but that is beyond the point here.}

%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects.


%
%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects. 
%
% In a third line, joint-detection-and-embedding approaches emerged that take appearance features directly from the detection backbone. 
%
%While powerful, these methods rely more and more on large amounts of training data, e.g., pre-training on the detection dataset CrowdHuman \lau{cite} has become a necessity to obtain state-of-the-art results. 
%




%\lau{Next is just the spirit of what we want to say, need to find better words.}

%In our view, it would make sense to revisit TbD to see if we can obtain a strong tracker that does not heavily depend on training data.

%\lau{Alternative, you know what i mean...}

%We believe tracking-by-detection should not be discarded just yet, as it shows the clear advantage of being a simple tracker that can be built without large amounts of data. Our question is then: \textit{Can we bring the performance of TbD closer to new paradigms?} \gui{I like this! I don't yet have solid proposal, but I'd like to have an additional motivation for TbD. Do we have any other options? (e.g. long history of research that can be exploited). I think that the link TbD $\approx$ small amounts of data is not super obvious. Another thing that comes to mind (going too deep maybe) is that I believe that the reason why our simple TbD method works so well is partly bc detections are now so good. And detections are so good bc of large amounts of training data... so not sure how solid it is to sell (overall) TbD as good in the low-data regime.}



%While they both differ with respect to their detailed pipeline, they have a strong focus on complex learning-based pipelines. \gui{Not sure that this applies to tracktor/centertrack.}.\lau{Def not, I would say that they do needs large amounts of data to be trained, that is actually true. CT was the first to introduce CH pretraining, so that shows you how much data they need. Trackformer same... tracktor a bit less, but we can generalize here.} Moreover, approaches based on the tracking-by-attention paradigm as well as joint-detection-and-embedding approaches require a large amount of training data. \gui{talking about joint-detection-and-embeddings but they have not yet been introduced }


%A recent work \cite{DBLP:journals/corr/abs-2110-06864} showed that in the presence of high quality object detections, a simple Kalman filter suffices to achieve state-of-the-art performance in MOT. This rises the question which advances are driving the progress in the field. \gui{This last sentence now feels a bit detached from what we've been saying} \lau{I do not know either. I would say, this motivates us to restudy TbD with the new knowledge in machine learning, detectors and architectures.}


% Introducing our approach
%In this work, we follow the spirit of revisiting the TbD paradigm but take the thought further. Instead of solely relying on motion cues which are said to perform bad with respect to long-term associations \textcolor{red}{REF} \gui{I don't like how 'are said to perform bad' sounds, it seems like a weakly presented 'argument from authority'. We need something more powerful as we'are about to motivate what we do differently}, we also utilize appearance features which are often used to overcome those shortcomings. Therefore, we ask the question: How can we leverage synergies between motion and appearance features to further make TbD competitive again? \jenny{MAKE TbD GREAT AGAIN!! :D}  \gui{Wasn't it also part of the story that we show 'the right way' to exploit ReID? Now it seems like the entire weight is on combining reid and motion, which is not that strong results/methodology wise...}
%\lau{Yes, I have always been a fan of the whole reid and not the motion, maybe i need to be more authoritative about this ahahah :D}
%
%We investigate on how to improve basic appearance-based cues as well as
%
%how to best combine motion and appearance within the online TbD framework, obtaining a strong tracker.
%: \textit{do we really need to use sophisticated learning-based frameworks for data association?}
%
%We revisit the association step, showing that it can significantly improve over state-of-the-art models in several datasets.
%
%We do so by exploiting two standard cues, \textit{appearance} and \textit{motion}, within the online TbD framework, obtaining a strong tracker.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/teaser.jpg}
    \caption{IDF1/Rank-1 of different state-of-the-art re-ID approaches. R50-TR \cite{torchreid}, BOT \cite{DBLP:conf/cvpr/0004GLL019}, BDB \cite{DBLP:conf/iccv/DaiCGZT19}, ABD \cite{DBLP:conf/iccv/ChenDXYCYRW19}. \textit{Basic} is our baseline, \textit{Ours} is our appearance model.}
    \label{fig:teaser}
\end{figure}

%\jenny{Maybe in line with the above comment: we should add here that a well trained detector + simple cues is enough maybe? Would be in line with what the positive reviewer said.} \lau{We are also sota on public detections, no? i do not see the problem then.}
We argue that if the appearance and motion cues are strong \jenny{our motion is actually not pretty strong/fancey?}, we do not need a complex tracker, and a simple frame-by-frame tracking-by-detection will suffice. %\jenny{Are our motion and reid cues strong? Actually they are quite basic, right? And also the detector we utilize was trained on many datasets which I think we cannot just leave our here right?} \lau{Detector is another thing, and we are actually sota with public dets, so I think we dont need to go deep into this in the intro. also strong and simple/basic are not antagonists :)}
%
We therefore propose to revist the roles of the appearance and motion cues for MOT.
%
Our first observation is that simply using state-of-the-art re-identification (reID) networks for appearance matching is not enough for the real scenarios of MOT. In Figure~\ref{fig:teaser}, we visualize the performance of several state-of-the-art reID approaches on Market-1501 dataset \cite{DBLP:conf/iccv/ZhengSTWWT15} (x-axis), as well as the models performance when used in a simple matching-based tracker (y-axis). It shows that the reID performance does not necessarily translate to MOT performance. %\jenny{Please check.} \lau{awesome}
%\jenny{Our model is far from SOTA in person ReID. We achieve 85 Rank-1 while there is currently stuff our there that reaches 97 Rank-1 or so. We had an analysis in the CVPR version though showing that SOTA ReID does not nessecarity work good. We could show this if we want to keep this message.}
%


We identify two problems causing the weak performance of reID models on MOT: (i) reID models need to account for the different challenges expected at different time horizons, \ie, while in nearby frames appearance of objects will vary minimally, in longer time gaps more severe changes are expected, and
%We identify two problems: (i) re-identification in nearby frames is different \lau{i feel my wording here is a tad weak, another for that is not just "different"?} from re-identification in far away frames, where the appearance of the object has potentially changed \gui{models need to account for the different challenges expected at different time horizons: while in nearby frames appearance of objects will vary minimally, in longer time gaps, more severe changes are expected.}. 
(ii) reID performance tends to be inconsistent across MOT sequences because of their varying image statistics, which in turn differ from the relatively stable conditions of the corresponding reID training dataset.
%training and test distributions will be different to the point of making reID methods weak on new sequences. \lau{too sexy?} \gui{I'd word it differently, bc 'all sequences are new sequences in MOT' (if u follow the common practice of not training on MOT seqs), and I'm not sure if this is clear?. Maybe I'd rephrase for smth like?: reid performance tends to be inconsistent across tracking sequences because of their varying image statistics, which in turn differ from the relatively stable conditions of their reid training dataset.'} \jenny{I'm with you Guillem, but I think we should still say sth that they are 'weak' because that's what we are also showing in the teaser. 'training and test distributions will be different and also across tracking sequences image statistics vary heavily. Compared to the relatively stable conditions of the reid training dataset this leads to surprisingly low performance of reID methods in MOT.'}
%
%
We propose two simple but key design choices to overcome the aforementioned problems, \ie, on-the-fly domain adaptation, and different policies for active and inactive tracks.

%We propose to enhance our reID algorithm with two key design choices: (i) different policies for active and inactive tracks, and (ii) on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracks, while the latter helps to close the dataset statistics gap between train data and MOT sequences. \lau{I would change the order and first mention the problem and then the solution.} \gui{I agree}
%
We then do an extensive analysis under different conditions of visibility, occlusion time, and camera movement, to determine in which situations reID is not enough and we are in need of a motion model.
%
%\lau{Ok here I think we should say nothing about the motion model. The sentence before and after already match, so I think we can leave it as is and not speculate here about motion. What do you think?}
%Maybe surprisingly, a linear motion model over the past tracks works incredibly well. \gui{I'd rewrite these two sentences but I like the overall approach of how motion is introduced into the conversation} \lau{I might delete the second sentence and just leave the first, and go from "we need a motion model" to the simple combo that reaches sota.} \gui{proposal (not sure if we wanna go there though): we find that while ReID might struggle under occlusions in some situations, a simple motion model can compensate for most its failures.}\lau{risky}\jenny{Maybe surprisingly, a linear motion model over the past tracks complements reID incredibly well.}
%
Our experiments show that combining our ReID with a linear motion model suffices to obtain a tracking-by-detection tracker without any bells and whistles that significantly outperforms state-of-the-art \jenny{to be adapted}.
%
Most notably, \textit{our reID model is never trained on any tracking dataset, showing good generalization.} %\ili{put this sentence in bold/italic!}
%\jenny{I'm still not sure if we can say it like this because our detections are. But I think this is just because recently detectors and trackers are more and more entangled :)}
%\lau{Yes but that is their problem, right? I mean detection datasets you have a million, tracking not so much, so training a strong detector is arguably easier. We dont really lie here, we jus say our tracker does not need much data, plus we are also strong in public detections, so its not only when detector is strong.} \jenny{Convinced :)}


% go a bit more precise

%Our approach consists of a matching-based tracker that performs association in one single step utilizing an affinity score based on the appearance and motion cues between past \gui{tracks} and current detections at every frame.
%
%We obtain our appearance information from a standard re-identification (ReID) network, whose performance we enhance with two design choices: different handling of active and inactive tracklets and on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracklets while the latter helps to close the dataset statistics gap between train data and MOT sequences. 
%
%Our motion term relies on the predictions of a linear motion model over past tracks. \gui{Maybe comment that we find it works incredibly well?
%}
% 
%We do an extensive analysis, determining that visibility, occlusion time, and camera movement heavily influence the performance of ReID and motion systems.
%
%Following that, we introduce a probabilistic policy to determine in which scenarios motion and ReID give more trustworthy similarity predictions given the underlying conditions and combine both appropriately.
%
%, and we demonstrate with our experimental analysis that our strong performance originates from improved data association.


% not sure if this goes here
\iffalse
Our work serves three main purposes. We demonstrate that using a strong, yet conceptually simple data association scheme can further revive the TbD paradigm.
%
We believe this is valuable by itself, and expect to make future work question the need for sophisticated learning-based approaches.
%
Furthermore, we demonstrate how to improve appearance cues following our simple design choices.
%Furthermore, our tracking analysis sheds light on what are the pressing challenges of tracking that both our method as well as previous top-performing ones still struggle to address.
Finally, based on a tracking analysis we shed light on how to combine motion and ReID in way to best exploit both cues.
%
We expect that the insights presented in this paper will encourage subsequent methods to target their effort towards solving them.

\fi 

\vspace{0.3cm}
%\lau{Contributions: 1. We propose key changes to reid so that it works. 2. We analyze where appearance and motion have the potential to be useful to increase performance wrt current trackers. 3. We show SOTA with a simple tracker cos we are awesome.}

\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We provide key design choices that significantly boost the performance of reID models for the MOT task.
    \item We extensively analyze in which cases appearance and motion have the potential to increase performance with respect to current trackers.
    \item We obtain state-of-the-art results on several benchmarks with a simple tracking-by-detection online tracker.
\end{itemize}
%All code and models will be made publicly available upon acceptance.

%\gui{I know this is not easy, but since we have a relatively 'exotic' paper, questioning current trends, I think it'd be nice if we were a bit more specific on how  we expect our results to impact future research. What should our paper make future tracking research change based on what we show, exactly? What is the main takeaway ? Example: people should think about Domain adaptation and appearance (ReID performance across diff sequences), the different challenges of short/long term association (e.g. we use two thresholds/proxies), people should think about interplay of motion and appearance in different circumstances. We showed a simple but strong version of how to operationalize these insights, people should look for fancier models while keeping these important tracking aspects in mind, not simply going all in on transformers. What do you think? Something along these lines could be placed either here in intro/conclusions, or at the experiments, after analysis, to make it look a bit more relevant for the overall paper.} \jenny{Really good idea/comment!! Tried to make a paragraph out of your thoughts, can you check? (below). We could acutally have the big paragraph here and then refer to it / repeat parts of it over the paper again at the corresponding sections.}

%\ili{is the part after the bullet points legit for this version of the paper?}

The current simplistic usage of of-the-shelf pre-trained ReID networks does not leverage the full potential appearance as networks only perform well on data that is highly similar to the train set. This leads to less stable results in tracking. Our work highlights the need of more robust models and domain adaptation which we hope inspires future works. 
%
Moreover, our analysis shows that the interplay between motion and appearance holds high potential. While our simple but strong version already achieves state-of-the-art performance, we hope future work to investigate this interplay even more. 
%
Consequently, we propose to rethink recent developments of ever increasing data-hungry trackers towards learning more from well-known concepts. Without much adaption between highly differing datasets, they still can achieve state-of-the-art performance.

%Overlooked by the community until now, we hope our work inspires future approaches to overthink the current usage of reID and the integration of domain adaption as well as how approach the differences between short and long term association, \textit{e.g.}, with different appearance proxies for active and inactive tracks. Moreover, our analysis shows the interplay between motion and appearance in different circumstances. Introducing a simple but strong version of how to utilize those insights, we hope to inspire future work to integrate this interplay into novel, sophisticated models further improving the state of the art.


%\lau{Totally agree with guillem, but i think the above paragraph is still not there yet. Things i would highlight: 1. We show that the previous idea of reid was far too simplistic, it only works if u train on extremely similar data as test. Current reid models do not work out of the box and the transfer to tracking is much less stable that previously thought --> adaptation is needed as we show or maybe more robust models --> future work. 2. analysis of the interplay between reid and motion, here again, it seems a simple combination is not the way to go but rather an analysis of when what can be used. 3. Overall, maybe learn-all transformers outperformed more classic models because classic models were not being used properly.  We should rethink the "let us throw data at the problem" for tracking because the "old" knowledge is still very much SOA. }

\iffalse
\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We do an extensive analysis, determining the most important factors that determine the performance of ReID and motion systems.
    \item Based on our analysis, we provide a strong probabilistic scheme for data association that combines appearance and motion cues using a derived policy.
    \item We obtain state-of-the art results on several benchmarks, etc. \ili{more precise, give numbers already}
\end{itemize}
\fi

==> cvpr2023-author_kit-v1_1-1/latex/chapters/Conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}
\vspace{-0.15cm}
\label{sec:conclusion}
In this paper, we show that good old TbD trackers are able to generalize to various highly differing datasets incorporating domain-specific knowledge. 
%
For our general simple Hungarian tracker \textbf{GHOST}, we introduce a spiced-up appearance model that handles active and inactive trajectories differently.
%
Moreover, it adapts itself to the test sequences by applying an on-the-fly domain adaptation. 
%
We analyze where our appearance and simple linear motion model struggle with respect to visibility, occlusion time, and camera movement. 
%
Based on this analysis, we decide to use a weighted sum that gives more weight to either cue when needed, depending on the situations in the datasets.
%
Despite being straightforward, our insights have been largely overlooked by the tracking community. 
%
We hope to inspire future research to further investigate on, extend, and integrate these ideas into novel and more sophisticated trackers.




==> cvpr2023-author_kit-v1_1-1/latex/chapters/Experiments.tex <==
\section{Experiments}

\label{sec:experiments}
% In this section, we first give implementation (Section \ref{subsec:implementation_details}) as well as dataset and metric details (Section \ref{subsec:datasets}). We then ablate GHOST with respect to the appearance design choices (Section \ref{subsec:reid_ablation}). Afterwards, we analyse the strengths of ReID and motion and ablate the performance of single cues (Section \ref{subsec:analysis}) to show the potential of GHOST (Section \ref{subsec:potential}). Finally, we demonstrate that GHOST generalizes to four public datasets (Sections \ref{subsec:MOT17}, \ref{subsec:MOT20}, \ref{subsec:dance}, \ref{subsec:BDD}).

\subsection{Implementation Details}
\label{subsec:implementation_details}
Our appearance model follows common practice~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/BrasoL20,DBLP:conf/cvpr/DaiWCZHD21}, with a ResNet50 \cite{DBLP:conf/cvpr/HeZRS16} model %\gui{question that just came to mind: why a ResNet50? would we be better with a larger CNN / transformer backbone?} \jenny{Cos R50 the default backbone in person reid and otherwise revs could also be like 'but you use a bigger backbone, thats why you are better' no?}\ili{agree with jenny, as a non tracking guy, that would have been my first comment as a reviewer...cause I am superficial like that :D} \jenny{ahahaha} 
with one additional fully-connected layer at the end to downsample the feature vectors. We train our model on the Market-1501 dataset~\cite{DBLP:conf/iccv/ZhengSTWWT15} using label-smoothed cross-entropy loss with temperature for $70$ epochs, with an initial learning rate of $0.0001$, and decay the learning rate by $10$ after $30$ and $50$ epochs. For optimization, we utilize the RAdam optimizer~\cite{DBLP:conf/iclr/LiuJHCLG020}. Moreover, we add a BN layer before the final classification layer 
%\ili{why?} \jenny{ReID tricks ;) bag of tricks rules } 
during training and utilize class balanced sampling as in~\cite{DBLP:conf/cvpr/0004GLL019}.
%
We resize the input images to $384 \times 128$ and apply random cropping as well as horizontal flipping during training \cite{DBLP:conf/cvpr/0004GLL019}.
%
Evaluated on Market-1501 dataset this model achieves $85.2$ rank-1, which is far below the current state-of-the-art performance~\cite{DBLP:conf/cvpr/0004GLL019,DBLP:journals/corr/HermansBL17,DBLP:conf/iccv/QuanDWZY19,DBLP:conf/cvpr/ChengGZWZ16,DBLP:conf/eccv/SunZYTW18,DBLP:conf/eccv/VariorHW16,DBLP:conf/cvpr/ZhangLZ019}.
%
For tracking, we define the appearance distance between $i$ and $j$ as the cosine distance between appearance embeddings $d_a(i, j) = 1 - \frac{f_i \cdot f_j}{||f_i||\cdot||f_j||}$. As motion distance we use the intersection over union (IoU) between two bounding boxes $d_m(i, j) = IoU(p_i , p_j) = \frac{|p_i \cap p_j|}{|p_i \cup p_j|}$. %\ili{oh nooooo, passive tense again :S}
%
%We compare GHOST to state-of-the-art approaches mainly under the focus of IDF1 and HOTA metrics. Considering MOTA is mostly dependent on detection performance, while our work focuses on the association step.
\input{tables/reid_balation}

\subsection{Datasets and Metrics}
\label{subsec:datasets}
In this section we introduce the datasets we evaluate GHOST on. MOT17 and MOT20 can be evaluated in public and private detection setting. For the private detection settings, BDD and DanceTrack we use detections generated by YOLOX-X~\cite{DBLP:journals/corr/abs-2107-08430} following the training procedure of \cite{DBLP:journals/corr/abs-2110-06864}.

\noindent\textbf{MOT17.} The dataset \cite{DBLP:journals/corr/MilanL0RS16} consists of seven train and test sequences of moving and static cameras. As common practice, for public detections we utilize bounding boxes refined by CenterTrack \cite{DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/SalehARSG21,DBLP:journals/corr/abs-2006-02609} as well as Tracktor \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/cvpr/YinWMYS20,DBLP:journals/pr/PengWLWSWD20,DBLP:conf/ijcai/LiuC0Y20,DBLP:conf/cvpr/SalehARSG21,DBLP:conf/cvpr/KimLAR21} for MOT17. For our ablation studies, we split MOT17 train sequences along the temporal dimension and use the first half of each sequence as train and the second half as evaluation set ~\cite{DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/WuCS00Y21}.

\noindent\textbf{MOT20.} Different from MOT17, MOT20 \cite{DBLP:journals/corr/abs-2003-09003} consists of four train and test sequences being heavily crowded with over $100$ pedestrians per frame. For the public setting, we utilize bounding boxes pre-processed by Tracktor \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/SalehARSG21,DBLP:conf/cvpr/BrasoL20}.
%

\noindent\textbf{DanceTrack.}
The dataset \cite{sun2022dance} significantly differs from MOT17 and MOT20 datasets in only containing videos of dancing humans having highly similar appearance, diverse motion, and extreme articulation. It contains 40, 25 and 35 videos for training, validation and testing.

\noindent\textbf{BDD.}
The MOT datasets of BDD 100k \cite{DBLP:conf/cvpr/YuCWXCLMD20} consists of 1400, 200 and 400 train, validation and test sequences with eight different classes with highly differing frequencies of the different classes. Note that our appearance model was \textit{never} trained on classes other than pedestrians.

\noindent\textbf{Metrics.} 
The benchmarks provide several evaluation metrics among which HOTA metric \cite{DBLP:journals/ijcv/LuitenODTGLL21}, IDF1 score \cite{DBLP:conf/eccv/RistaniSZCT16} and MOTA \cite{DBLP:journals/pami/KasturiGSMGBBKZ09} are the most common. While MOTA metric mainly is determined by object coverage and IDF1 mostly focus on identity preservation, HOTA balances both.

\input{tables/da_ablation}

\subsection{Appearance Ablation}
\label{subsec:reid_ablation}
In this section, we investigate the impact of the design choices of our appearance model on tracking performance. To this end, we do not utilize motion. In Table~\ref{tab:reid_blation}, we report our results on public detection bounding boxes of MOT17 as well as on BDD. %\lau{I removed the CT reference here on purpose, we said it already, lets not repeat too much since this i still find fishy.} 
%
% Note, that we do not use the same matching thresholds for the different settings as the distance histograms significantly change between them. \lau{What do you mean by these matching thresholds? I think this can easily go into suppl. otherwise it gets quite confusing here.}
%
The first row shows the performance of our basic appearance model. % It uses ResNet50 \cite{DBLP:conf/cvpr/HeZRS16} trained on Market-1501 dataset \cite{DBLP:conf/iccv/ZhengSTWWT15}, the same network as used for our appearance model. 
%SHORTENED
%We then ablate the model by adding our contributions: (i) different thresholds for active and inactive tracks (diff $\tau$), (ii) the usage of the proxy distance for inactive tracks (IP), and (iii) on-the-fly domain adaptation, \ie, target domain statistics for the batch-norm layers (DA). As shown, every module significantly improves the results in both IDF1 and HOTA scores. \jenny{Can be shortened for space issues}



\noindent\textbf{Different Handling of Active and Inactive Tracks.} As introduced in subsection~\ref{subsec:ReID}, the distance histograms for active and inactive tracks differ significantly. %Therefore, this calls for different matching thresholds $\tau_i$. 
In the second row in Table~\ref{tab:reid_blation}, we show that utilizing different thresholds for active and inactive tracks (diff $\tau$) improves our tracking performance by $0.5$ percentage points (pp) ($0.9pp$) in IDF1 and $0.2pp$ ($0.6pp$) in HOTA on MOT17 (BDD). Moreover, utilizing our proxy distance (IP) computation instead of the last detection for inactive tracks further adds $0.9pp$ ($1.8pp$) in IDF1 and $0.6pp$ ($1.0pp$) in HOTA.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[height=4.5cm]{figures/idf1_private_trackers.pdf}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.55\textwidth}   
        \centering 
        \includegraphics[height=4.5cm]{figures/hota_private_trackers.pdf}
    \end{subfigure}
    \vspace{-0.35cm}
    \caption{Analysis of contribution of appearance, motion and their combination upon private tracker bounding boxes \cite{DBLP:conf/eccv/WangZLLW20,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/cvpr/PangQLCLDY21,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20,DBLP:conf/eccv/PengWWWWTWLHF20}.}
    \label{fig:private}
    \vspace{-0.4cm}
\end{figure*}

\noindent\textbf{On-the-fly domain adaptation.} Additionally, we leverage our on-the-fly domain adaptation (DA) introduced in Subsection~\ref{subsec:ReID} that accounts for differences among the sequences, allowing us to have a well-suited threshold over all sequences. We gain another $1.7pp$ ($1.1pp$) in IDF1 and $0.9pp$ ($0.8pp$) in HOTA metrics. 
%
We also compare our on-the-fly DA to various different other domain adaptation approaches (see Table~\ref{tab:domain_adaptation_ablation}).
First, we ablate different versions of GHOST, \textit{i.e.}, utilizing random patches of a given frame instead of the pedestrian bounding boxes, utilizing the bounding boxes of the 10 frames before the current frame as well as feeding the whole sequence first to update the parameters. Except for the last, none of them leads to a performance improvement. We argue, that random patches do not represent the statistics of pedestrians well. Also, we fine-tune our reID network on MOT17. For this, we split the train sequences into three cross-validation splits and fine-tune one model for each split. This is necessary as the same identities are given if a sequence is split along the temporal domain. 
While the model is fine-tuned on tracking sequences, the sequences still differ in their distributions among each other. Hence, despite fine-tuning also significantly improving the performance it does not surpass DA. The same holds for using Instance-Batch Norm (IBN) \cite{DBLP:conf/eccv/PanLST18} instead of BN layers, which combine the advantages of Instance and Batch Normalization layers. %\jenny{maybe shorten here + struggeling to explain why 10 frames don't work. Not sure if we should go down the conditioned on the frame here.}

%We visualize the histograms for our Appearance with on-the-fly domain adaptation in  Fig~\ref{fig:dist_distribution_evalbb1} and without in Fig~\ref{fig:dist_distribution_evalbb0}. As can be observed, the distances of active tracklets and inactive tracklets to detections show varing means over the sequences. Although in Fig~\ref{fig:dist_distribution_evalbb0} the former still varies, the latter shows close to no variance. 

\subsection{Strengths of Motion and Appearance}
\label{subsec:analysis}
In this subsection, we analyze the performance of our appearance cues as introduced in Subsection~\ref{subsec:ReID} to find their strengths with respect to given tracking conditions, namely, visibility level of the detection, occlusion time of the track, and camera movement. We also analyze the complementary performance of our linear motion model that we introduce in the following. Here and in the following Subsection~\ref{subsec:potential}, we apply GHOST on the bounding boxes produced by several private trackers, treating them as raw object detections. We note that this is \textit{not} a state-of-the-art comparison, and emphasize that we solely use those experiments for analysis and to show the potential of our insights. %appearance and motion cues to improve current trackers.


\noindent\textbf{Linear Motion Model.} While many works apply more complex, motion models, \eg, Kalman Filters 
%\gui{as far as I know, Kalman filters are considered to be linear? Since they are applied with a constant velocity assumption}\jenny{Mhm in general you can add acceleration to a Kalman filter, but I guess in MOT it's normally not used? Therefore, removed the non-linear :) }
\cite{DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/eccv/WangZLLW20}, social motion models \cite{DBLP:conf/iccvw/Leal-TaixePR11}, or utilize detectors as motion model \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20}, we choose on purpose a simple linear model for our experiments.
%
Although the world does not move with constant velocity, many short-term movements, as in the case of two consecutive frames, can be approximated with linear models and assuming constant velocity.
%
Given detections of a track $j$, we compute the mean velocity $v_j$ between the last $k$ consecutive detections and predict the current position of a track by
\begin{equation}
    \hat{p}_j^{t} = p_j^{t-1} + v_j \cdot \Delta t,
\end{equation}

where $\Delta t$ is the time difference from one frame to another and $p_j^{t-1}$ is the position of the previous detection for active and the last predicted position for inactive tracks.

To obtain the motion distance between the new detections and the tracks, we compute the IoU between the position of a new detection $p_i$ and $\hat{p}_j^{t}$. We also visualize the corresponding distance histogram in Fig~\ref{fig:distributions}(c), showing that distance histograms between detections and tracks of the same and different identities are well separated for active tracks. In the following, we underline this observation by showing that this simple motion model is able to solve most situations. We set $k$ to use all previous positions in Subsections~\ref{subsec:analysis} and ~\ref{subsec:potential}. %\lau{I am a bit confused why we go back to fig 3 here?} \jenny{just because of spacing reasons. the three histograms fit nicely next to each other. I know not perfect.}


\noindent\textbf{Analysis Setup.} For our analysis, we investigate the rate of correct associations ($RCA$) on MOT17 validation set~\cite{DBLP:journals/ijcv/DendorferOMSCRR21}, which we define as:
\begin{equation}
    RCA = \frac{\text{TP-Ass}}{\text{FP-Ass} + \text{TP-Ass}},
\end{equation}
where $\text{TP-Ass}$ and $\text{FP-Ass}$ represents true positive and false positive association, respectively. We average RCA over the sets of pre-processed private detections from several trackers (see Section~\ref{subsec:potential}) to get less noisy statistics.  
\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/by_visibility_small.png}
    \caption{RCA with respect to different visibility levels for short-term vs. long-term associations.}
    \label{fig:by_visibility}
\end{figure}
\fi


% SHORTENED
% Intuitively, motion should perform well for short-term associations as pedestrians only undergo small displacements, while appearance should be able to correctly do long-term associations. 
%
%At the same time, motion should struggle to model long-term pedestrian behaviour, while appearance should be less robust with respect to occlusions as they highly influence appearance features. \jenny{maybe we can remove this paragraph?}

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/Sequence_analysis_occlusion_time_SMALL.png}
    \caption{RCA for static, moving, and all sequences with respect to short-term vs. long-term associations.}
    \label{fig:seq_analysis_occ}
\end{figure} 
\fi


\noindent\textbf{Observations.} %\jenny{Do you think we can put figure 4, 5 and 6 in supplementary? So rewriting this paragraph without see figure and so on and say in our supplementary we show visualizations? Just thinking about space issues}
We visualize RCA between detections and trajectories with increasing occlusion time for different visibility levels (Fig~\ref{fig:by_visibility}) as well as the performance of motion and appearance for static and moving sequences with respect to occlusion time and visibility (Fig~\ref{fig:seq_analysis_occ} and Fig~\ref{fig:seq_analysis_vis}). %For example, in Fig~\ref{fig:by_visibility}(a) we plot RCA for reappearing bounding boxes that are $0-33\%$ visible.
%
For highly visible bounding boxes (Fig~\ref{fig:by_visibility}(c)) appearance performs better than motion with respect to long- \textit{and} short-term associations.
%
While intuitively motion should perform especially well on short-therm associations independent of the visibility, Fig~\ref{fig:seq_analysis_vis} reveals that it struggles in moving sequences. This is due to the combination of the camera
movement and the bounding box movement which turns motion into being more non-linear.
On the other hand, in static sequences, the linear motion model performs better with respect to long-term associations than appearance (see Fig~\ref{fig:seq_analysis_occ}). 
%
This is caused by the fact that the lower the visibility (see Fig~\ref{fig:by_visibility}(a)), the higher the tendency of motion to perform better for long-term occlusions since motion is a strong cue in low visibility, \ie, occluded scenarios, (see Fig~\ref{fig:seq_analysis_vis}).
%
We show a more detailed analysis in the supplementary. %\jenny{Rewritten the above, comments please :)} \gui{I like it, I think it's clear and concise!!}

%\gui{I think we need to shorten this. Since I still think that we don't really use this that much for anything and I find it a bit hard to follow. I think that the overall content is good, we just need a little less detail.} 
%We visualize RCA between detections and trajectories with increasing occlusion time for different visibility levels (see Fig~\ref{fig:by_visibility}). For example, in Fig~\ref{fig:by_visibility}(a) we plot RCA for reappearing bounding boxes that are $0-33\%$ visible. 
%
%We observe that for highly visible bounding boxes appearance performs better with respect to long-term as well as short-term occlusions. On the other hand, the lower the visibility, the higher the tendency of motion performing better with respect to long-term occlusions.
%
%This raises the following question: Why does motion not perform as good as appearance for short-term associations on highly visible bounding boxes? The motion of non-occluded pedestrians should not exhibit highly non-linear motion. \gui{double negation is a bit hard to parse} Moreover, it is questionable why motion is able to perform long-term associations correctly. Therefore, we analyze the performance of motion and appearance for static and moving sequences with respect to short-term vs. long-term associations as well as visibility (see Fig~\ref{fig:seq_analysis_occ} and Fig~\ref{fig:seq_analysis_vis}).
%
%We observe that motion is a strong cue in low visibility, \ie, occluded scenarios, however struggles in moving sequences. Especially for static sequences, the linear motion model performs better with respect to long-term associations than appearance. We show a more detailed analysis in supplementary.


\noindent\textbf{Conclusion.} In conclusion, the interplay of three factors mainly influences the performance of motion and appearance: visibility, occlusion time, and camera motion. However, we saw that appearance and motion complement each other well with respect to those factors.
Hence, we now move on to creating a strong tracker that combines our appearance and a simple linear motion model.


\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/binned_frame_dist0.33-0.0_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=0.99\textwidth]{figures/binned_frame_dist0.6666666666666666-0.3333333333333333_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=0.99\textwidth]{figures/binned_frame_dist1.00001-0.6666766666666668_plot.png}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{RCA with respect to different visibility levels for short-term vs. long-term associations.}
    \label{fig:by_visibility}
    \vspace{-0.1cm}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/binned_frame_distS_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/binned_frame_distM_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/binned_frame_distno_mask_plot.png}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{RCA for static, moving, and all sequences with respect to short-term vs. long-term associations.}
    \label{fig:seq_analysis_occ}
    \vspace{-0.1cm}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/binned_visS_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/binned_visM_plot.png}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/binned_visno_mask_plot.png}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{RCA for static, moving, and all sequences with respect to different visibility levels.}
    \label{fig:seq_analysis_vis}
    \vspace{-0.3cm}
\end{figure*} 


\subsection{Simple cues lead to a strong tracker}
\label{subsec:potential}
%As can be seen, we improve the performance of all original trackers significantly by up to $10.2pp$ in IDF1 and $5.1pp$ in HOTA metrics. On average we achieve a relative improvement of $6.1pp$ on IDF1 and $2.2pp$ on HOTA.
%\input{tables/private_detectors}
In this subsection, we ablate the combination of appearance and motion into a simple Hungarian-based online tracker.
%
%our design choices with respect to appearance and motion and underline the potential lying in revising the TbD paradigm. 
%
We use the same setting as in Subsection~\ref{subsec:analysis}, \ie, we apply GHOST upon other trackers. Hence, we only report metrics related to the association performance, \ie, IDF1, and HOTA in Subsection~\ref{subsec:potential}, as our goal is not to improve on the MOTA metric, which is heavily dependent on detection performance.
%
We visualize the results in Fig~\ref{fig:private}, where markers and colors define which motion and appearance model is used, respectively. The blue bars represent the average occlusion level of detection bounding boxes of the different trackers.
%\lau{explain blue bars here, otherwise its too confusing}



\noindent\textbf{Appearance.} 
%We analyze the performance of the basic appearance model from Section~\ref{subsec:reid_ablation}. As can be seen in Fig~\ref{fig:private}, basic appearance mostly performs worse than the original trackers. Exchanging the basic appearance application by our appearance gives a significant performance boost for most trackers. 
Compared to the performance of the original trackers, our appearance model improves the performance by up to 8.2pp in IDF1 and 4pp in HOTA for detection sets with lower average occlusion levels. In detection sets with high occlusion, pure appearance struggles, confirming that it is not suited for associations in those scenarios. %\ili{some numbers, e.g., by up to x pp instead of just significantly?}
%\lau{We also need to say our appearance is better! red>green}\jenny{nonono green os not basic it is NO appearance haha, we removed no basic appearance :) }
%Compared to the performance of the original trackers our appearance does not show a consistent behaviour: in some cases our appearance outperforms the original performance while in others our appearance worsens it \ili{this is a really bad sentence, our method at times works better, at times worst screams reject this paper. Reformulate in a way to emphasise the 'wins' and diminish the 'losses'}. 
%Investigating the average occlusion level of the trackers bounding boxes (blue bars in Fig~\ref{fig:private}) reveals that the performance of our appearance drops if the occlusion level is high confirming that appearance is not suited for associations in those scenarios.


\noindent\textbf{Motion.} Interestingly, applying only the simple linear motion model without appearance %, \ie, $d^m$ 
always improves or performs on par with the original trackers. Utilizing a Kalman filter instead of the linear motion model does not impact the performance significantly. This further highlights the strength of the simple linear motion model. %Those observations indicate that a simple motion model suffice to perform tracking in most cases. 
While setting the number of previous positions to use to approximate a tracks current velocity $k$ to use all previous positions in this section, we generally found that moving camera sequences profit from a lower $k$ value due to the combination of the camera movement and the bounding box movement leading to less stable motion. The same holds for extreme movements, \textit{e.g.} as in the DanceTrack dataset.

\noindent\textbf{Combination.} We also visualize our appearance combined with linear motion or a Kalman Filter. Although we find that sequences with a moving camera profit from a lower motion weight while detections with high occlusion level profit from a higher motion weight, we fix the motion weight to $0.5$ in this experiment. Moreover, we visualize the performance of our appearance model combined with a Kalman filter. %, and utilize the same setup as when combining our appearance model and the linear motion model.
Fig~\ref{fig:private} shows that using a Kalman filter instead of the linear motion model does not impact the performance notably. %While showing that our appearance and both motion models complement each other, we chose the simpler model, \ie, the linear model.
%\input{tables/ablations} 
However, both combinations improve significantly over using motion or our appearance alone.
%\lau{Again, talk about how awesome our method with our appearance is!}

\subsection{Comparison to State of the Art}
We compare GHOST to current state-of-the-art approaches. In all tables \textbf{bold} represents the best results, \textcolor{red}{red} the second best, and \textcolor{blue}{blue} the third best. 

\iffalse
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/NoLeg_idf1_private_trackers_no_trans.jpg}
        \caption{IDF1}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.57\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures/hota_private_trackers_wo_trans.jpg}
        \caption{HOTA}
    \end{subfigure}
    \caption{Analysis of the contribution of Appearance and motion cues as well as their combination upon JDE \cite{DBLP:conf/eccv/WangZLLW20}
, FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21}, QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21}, TraDeS \cite{DBLP:conf/cvpr/WuCS00Y21}, CenterTrack \cite{DBLP:conf/eccv/ZhouKK20}, CTracker \cite{DBLP:conf/eccv/PengWWWWTWLHF20}}
    \label{fig:private}
    \vspace{0.2cm}
\end{figure*}
\fi

% \subsection{The Interplay of Motion and Appearance}
% We now also analyze the influence of the combination parameters used in our model, \ie, the $h$ values in the hill functions as well as the mixture weights $\lambda_i$. Rest tbd :)
\input{tables/public_detections}

\noindent\textbf{MOT17 Dataset.}
%\noindent\textit{Public Detections.} 
%We compare our method with several state-of-the-art methods \cite{DBLP:journals/isci/YoonKSYJ21,DBLP:conf/icmcs/ChenAZS18,DBLP:journals/pr/PengWLWSWD20,DBLP:journals/access/YoonGSYJ20,DBLP:conf/iccv/Xu0ZH19,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/ijcai/LiuC0Y20,DBLP:conf/cvpr/YinWMYS20,DBLP:journals/corr/abs-2111-05943,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/SalehARSG21,DBLP:conf/cvpr/KimLAR21} in public detections. 
%
On \textit{public detections}, GHOST improves over the best previous methods, \textit{e.g.}, we improve over %TrackPool-T \cite{DBLP:conf/cvpr/KimLAR21} by $3.8pp$ in IDF1 \gui{If I'm not wrong, we are comparing our centertrack-preprocessed numbers to their tracktor-preprocessed numbers. With a fair comparison we are actually slightly worse!?} \jenny{I've seen this stuff in general several times, but you are right, how should we do this, just not compare to them but just to ArTIST-C?} and 
ArTIST-C \cite{DBLP:conf/cvpr/SalehARSG21} $1.8pp$ in HOTA (see Table~\ref{tab:sota}). As expected, we do not improve in MOTA, as it is mostly dependent on the detection performance. %, and we do not add new detection bounding boxes.
%
%We also utilize pre-processed bounding boxes the current state-of-the-art TMOH \cite{DBLP:conf/cvpr/StadlerB21} which adds occluded bounding boxes to the public detection set. As can be seen, MOTA, IDF1 as well as HOTA performance improves over previous state-of-the-art Trackers.
%
%\noindent\textit{Private Detections.} %In the private detection setting, compare to MOT17 state-of-the-art approaches~\cite{DBLP:journals/pami/SunASMS21,DBLP:conf/eccv/PengWWWWTWLHF20,DBLP:conf/cvpr/PangLZLL20,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/PangQLCLDY21,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/cvpr/WangZPX21,DBLP:conf/avss/StadlerB21a,DBLP:conf/icra/0002KW21}. 
In the \textit{private detection setting} we perform on par with ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} in HOTA and IDF1 outperforming second-best approaches by $3.7pp$ and $4.6pp$.


\noindent\textbf{MOT20 Dataset.}
%\noindent\textit{Public Detections.} 
%Next, we compare to state-of-the-art approaches on the \textit{public detection setting} of MOT20 %\cite{DBLP:conf/icip/BewleyGORU16,DBLP:conf/icpram/Lohn-JaramilloJ21,DBLP:journals/jvcir/Baisa21a,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/SalehARSG21}. 
Despite the complexity of the sequences being heavily crowded and exhibiting difficult lightning conditions, GHOST improves state-of-the-art \cite{DBLP:conf/iccv/BergmannML19} on \textit{public detection setting} of MOT20 by $2.6pp$ in IDF1 and $1.3pp$ in HOTA metric (see Table~\ref{tab:sota}).
%
This shows that the combination of our strong appearance cues and the linear motion adapts to the underlying conditions of higher occlusion levels.
%
%Recall, we never train our appearance model on any of these sequences.
%
%\noindent\textit{Private Detections.} 
In the \textit{private detection setting} of MOT20, we %compare to~\cite{DBLP:journals/iotj/ZhangSWWKX20,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/avss/StadlerB21a,DBLP:conf/icra/0002KW21} and 
 outperform all other methods by up to $0.8pp$ on HOTA and $0.7pp$ on IDF1. %This again shows the adaptability of GHOST to highly varying sequences. 
%
GHOST is able to fully leverage the additional available bounding boxes in the private detection setting, substantially increasing identity preservation compared to the private setting.


\noindent\textbf{DanceTrack Dataset.}
Despite the claim of the corresponding paper \cite{sun2022dance} that reID and linear motions models are not suitable for DanceTrack, GHOST outperforms all other methods on the test set (see Table~\ref{tab:dance}). Surprisingly, Transformer-based methods like GTR \cite{DBLP:conf/cvpr/ZhouYKK22} and MOTR \cite{DBLP:journals/corr/abs-2105-03247} that are said to be general cannot transfer their performance from MOT17 and MOT20. We improve over prior state-of-the-art by \textit{2.5pp} on HOTA, \textit{3.8pp} on IDF1 and even \textit{0.7pp} on MOTA.
\input{tables/dancetrack}

\noindent\textbf{BDD100k Dataset.}
Despite our appearance model \textit{never} being trained on more than pedestrian images, it is able to generalize well to the novel classes. GHOST outperforms state-of-the-art in mHOTA and mIDF1 on the validation set by $0.3pp$ and $2pp$ and in mIDF1 on the test set by $1.2pp$ (see Table~\ref{tab:bdd_short}). In IDF1 metrics, QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} outperforms GHOST. Since mHOTA and mIDF1 are obtained by averaging per-class IDF1 and HOTA while IDF1 and HOTA are achieved by averaging over detections, the results show that GHOST generalizes well to less frequent classes while other approaches like QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} overfit to more frequent classes, \textit{e.g.}, car (see also per-class validation set results in the supplementary).

\input{tables/bdd_short}


==> cvpr2023-author_kit-v1_1-1/latex/chapters/Intro.tex <==
\section{Introduction}
\label{sec:intro}
\iffalse
\begin{itemize}
    \item Multi-object tracking (MOT) aims to track multiple objects over video sequences
    \item classic paradigm tracking-by-detection
    \item nowadays also joint detection and tracking
    \item trackers use location, motion and appearance cues
    \item Recently trackers leverage sophisticated motion models as well as embedded ReID
    \item We provide a strong baseline for Multi-Object Tracking
    \item We claim depsite its simplicity a mixture of a simple ReID and a simple motion model is enough to achieve state of the art
    \item Contributions: Analysis when motion and when ReID, show that simple motion model and ReID complement each other, achieve state of the art.
\end{itemize}
\fi

% MOT and TbD
We revise Multi-Object Tracking (MOT) which aims at finding the trajectories of all moving objects in a video. The dominant paradigm in the field is Tracking by Detection (TbD), which consists in first detecting objects across video frames, and then linking them into temporally coherent trajectories, i.e., performing \textit{data association}. While the performance of approaches following the TbD paradigm can be significantly improved by the underlying detections, we focus on the less studied yet profoundly important association step. \ili{do we need the last sentence? every tracking paper focuses on the association step.}

% Criticism of field/motivation
\ili{agree that it is too long, and needs to be more conciser}
\alj{This section is too verbose. Also, unsure about the message. The message appears as “do we need complex frameworks for data assoc”, but I think this has been questioned and answered over and over: turns out that with good detectors and ReID models, once can get away with the most simplistic association techniques (Hungarian, greedy based on regressed offset as in centertrack, etc)} \jenny{I'm not 100\% sure about what would be the optimal message here then.}
Advances in learning-based object detectors have benefited the field, as evidenced by the widespread adoption of Faster R-CNN variants among top-performing approaches \REF. In contrast, progress in data association has been \textcolor{red}{more difficult to observe}, as current state-of-the-art methods have taken seemingly divergent paths. However, there is a common theme among them: a strong focus on sophisticated learning-based pipelines. Some examples are attention-based networks \REF, graph neural networks \REF or end-to-end joint detection and embedding frameworks \REF, as well as the trend of using increased amounts of labelled data such as single-image training \REF. %As a consequence of their focus on learning, recent methods also tend to have increased needs for training data. 
Given the significant differences and increasing complexity of these approaches, comparisons among them are notoriously difficult. Moreover, it is unclear which advances are driving progress in the field. These issues make the following question arise: \textit{do we really need to use sophisticated learning-based frameworks for data association?}

\jenny{Ideas for the upper paragraph: we show how much we can improve the performance by taking a step back and re-visting morion and ReID cues.}


% Overview of our approach
In this work, we address this question by showing that taking a step back and re-visting the association step can significantly improve upon complex state-of-the-art methods on \textcolor{red}{several} datasets. We show that by exploiting motion and appearance, which are standard cues, within a well-known online TbD framework, we can obtain a strong tracker. Our tracker, without bells and whistles, outperforms state-of-the-art trackers, and we demonstrate with our experimental analysis that our strong performance originates from improved data association.
\jenny{can we say this? If we would use purely the detections of QDTrack for example it would not be as good as it is now}, 


% More detailed explanation of our appraoch
% \alj{Also this section, rephrase. Bi-partite matching is probably irrelevant at this stage. Seems to me that at the core of your method are the appearance and motion model, and “a policy” on how/when trust whom, or how to combine them? Dont use words such as “simple tricks”!}
Our approach consists of a matching-based tracker that leverages a single affinity score taking appearance and motion cues between past tracks and current detections, at every frame into account.
%
We obtain our appearance term from a standard re-identification (ReID) network, whose performance we enhance with two design choices: different handling of active and inactive tracklets and on-the-fly domain adaptation.
%
Our motion term relies on the predictions of a linear motion model over past tracks. 
%
Undertaking an extensive analysis we determine three factors, namely, visibility, occlusion time, and camera movement, that heavily influence the performance of ReID and motion, respectively. \ili{i think that the previous sentence should not be here, but somewhere in methodology.} Based on those three factors we introduce a policy to determine in which scenarios motion and ReID give a more trustworthy similarity predictions and combine the appropriately.
%
%Overall, we show how to design a strong prior on tracking behavior combining simple features that outperforms sophisticated learning-based predictions.  

% Our message
We expect our work to serve two main purposes. First, to demonstrate that given good detections, data association can be mostly solved with a strong yet simple association scheme. We believe that this is valuable by itself, and expect it to make future work question the need for sophisticated learning-based approaches. Second, the analysis we conduct to derive our tracking policy sheds light on what are the pressing challenges of tracking that both our method as well as previous top-performing ones still struggle to address. We hope that the insights we derive will encourage subsequent methods to target their effort towards solving them.
%
Overall, we make the following contributions:
\begin{itemize}
    \item We provide a strong scheme for data association combining simple appearance and motion cues with a policy derived from an analysis of their applicability under different tracking conditions.
    \item We obtain state-of-the art results on several benchmarks, etc. \ili{more precise, give numbers already}
\end{itemize}




\ili{too much mentioning of the simple, also we should add another contribution, maybe something with respect to analysis.}

%In this work, we take a step back and address show that a simple baseline with minimal learning involved
\iffalse
Rough structure:
\noindent{\textbf{1) Background + Motivation}}
\begin{itemize}
\item[$\bullet$]   MOT definition, TbD=det + data association,  it's still the dominant paradigm.
\item[$\bullet$]  Progress in detection has clearly benefited tracking (cite MOTCha paper), and most TbD approaches stick to standard FRCNN and variants.
\item[$\bullet$] (Criticism of status of field:) But progress in data association has been less clear, as different methods have taken seemingly completely different directions. Common trends:
\begin{itemize}
\item Strong focus on learning with ever increasing complexity in architectures (attention, GNNs, e2e detection+appearance)
\item Increase in data needs (e.g. extra datasets, single-image training) 
\item Generally, methods still exploiting classical appearance and motion cues, but possibly in fancy ways.
\end{itemize}
\item[$\bullet$] Comparisons among methods are hard, and it's overall unclear what's driving progress in the field. Do we really need all the fancy stuff?
\end{itemize}
\noindent{\textbf{2) Our solution}}
\begin{itemize}
\item[$\bullet$] High-level view of contribution: We take a step back, and show that appearance and motion cues can be exploited in a remarkably simple way, and without any complex learning scheme. Despite its simplicity, we demonstrate that when evaluated on the same detections of other trackers, our approach consistently outperforms sophisticated methods
\item[$\bullet$]Method overview: our approach consists of a simple bipartite-matching-based online tracker, that combines an appearance term with a motion term to obtain a single cost.
\begin{itemize}
	\item  Our appearance term comes from the embedding similarity produced by a standard ReID network, with some simple tricks. 
	\item Our motion term comes from the prediction of a simple linear motion model
	\item Our policy to combine them is derived from an extensive analysis of the performance of these two terms. 'We replace learning by 'analysis' and manually setting strong priors' kinda argument'.
\end{itemize}
\item[$\bullet$] (Wrap-up again? maybe skip) despite the simplicity of our features and (lack/simplicity) of our learning scheme, we show that our approach systematically outperforms SOTA methods when evaluated over the same set of detections --> We show superior association! 
\end{itemize}
\noindent{\textbf{3) General message and contributions}}
\begin{itemize}
\item[$\bullet$] Our message: given good detections, data association can be mostly solved with a simple scheme Future methods should make sure that
\begin{itemize}
\item[$\bullet$] They can surpass this baselines before resourcing to fancy learning-based approaches
\item[$\bullet$] They focus on the bits of tracking such as long-term association that, as showed in our analysis, remain unaddressed
\end{itemize}
\item[$\bullet$] Our contributions:
\begin{itemize}
\item[$\bullet$] Simple strong baseline
\item[$\bullet$] Analysis
\item[$\bullet$] SOTA results
\end{itemize}

\end{itemize}

\fi

==> cvpr2023-author_kit-v1_1-1/latex/chapters/Methodology.tex <==
\section{Methodology}
\label{sec:methodology}


%In this section we introduce our general yet simple online tracker GHOST. 
Based on the good old Hungarian TbD paradigm, GHOST combines design choices that have been overlooked by the community until now. 
%
We start by giving the general pipeline of GHOST (see Sec. \ref{subsec:pipeline}) and then build our strong appearance model (see Sec. \ref{subsec:ReID}).
%
%In Section~\ref{sec:experiments}, we analyse the performance of our appearance model with respect to visibility of a given detection, occlusion time of a tracklet, as well as camera movement.

%We combine a appearance model solely trained on a commonly used reID dataset with a heuristic linear motion model based on constant velocity assumption. 
%
%We analyze the scenarios where motion and appearance work best, and unify them to leverage their complementary strengths.
%Despite its simplicity our model outperforms current state-of-the-art trackers. 

\subsection{A simple tracking-by-detection tracker}
\label{subsec:pipeline}

%Visualized in Figure~\ref{fig:pipeline}
%We follow the commonly used tracking-by-detection paradigm. 
Our tracker takes as input a set of detections $\mathcal{O} = \{o_1, ..., o_M\}$, each represented by $o_i = (f_i, p_i)$. $f_i$ are appearance feature vectors generated from the raw detection pixels using a Convolutional Neural Network (CNN) and $p_i$ is the bounding box position in image coordinates.
%
A trajectory or track is defined as a set of time-ordered detections ${T}_j = \{o_{j_1}, ..., o_{j_{N_j}}\}$ where $N_j$ is the number of detections in trajectory $j$. Moreover, each trajectory has a corresponding predicted position $\hat{p}_j^t$ at time step $t$, produced by our linear motion model. During the tracking process, detections are assigned to trajectories. %based on appearance cues, motion cues or a combination of both. 
%
If no new detection is added to a trajectory at a given frame, we set its status to \textcolor{blue}{inactive} whereas it remains \textcolor{mygreen}{active} otherwise. We use a memory bank to keep inactive trajectories of up to 50 frames. %(see Figure~\ref{fig:pipeline}). %\ili{possible rewrite: We use a memory bank to keep inactive trajectories of up to 50 frames (see Figure~\ref{fig:pipeline}}.
%
The goal is to find the trajectories $\mathcal{T} = \{{T}_1, ..., {T}_M\}$ that best match the detections to the underlying ground truth trajectories.

Towards that end, we associate existing detections over consecutive frames utilizing bipartite matching via the Hungarian algorithm
as commonly done \cite{DBLP:conf/icip/WojkeBP17,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/eccv/WangZLLW20,DBLP:conf/ijcai/LiuC0Y20,DBLP:conf/icip/BewleyGORU16}. 
%
The assignment is driven by a cost matrix that compares new detections with the tracks already obtained in previous frames. To populate the cost matrix, we use appearance features, motion cues, or both. Our final tracker utilizes a simple weighted sum of both. We filter detection-trajectory pairs $(i, j)$ \textit{after} the matching using matching thresholds $\tau_i$.
%To restrict assignments to only contain sufficiently similar detection-trajectory pairs $(i, j)$, we filter the matchings using matching thresholds $\tau_i$. \gui{maybe reword}

\subsection{Strong appearance model for MOT}
\label{subsec:ReID}

Our appearance model is based on ResNet50 \cite{DBLP:conf/cvpr/HeZRS16} with one additional fully-connected layer at the end for downsampling, and trained on a common person reID dataset \cite{DBLP:conf/iccv/ZhengSTWWT15}.
It is important to note that we \textit{do not train any part of our reID model on any MOT dataset}.  %\gui{Might need to update depending on BDD}
%
As we will show in experiments, this basic reID model does not perform well on the MOT task. We, therefore, propose two design choices to make our appearance model stronger: (i) we handle active and inactive tracks differently; (ii) we add on-the-fly domain adaption. For this, we analyze distances between detections and tracks in given MOT sequences.

\noindent\textbf{Appearance distance histograms.} In Fig~\ref{fig:distributions} we analyze the histograms of distances between new detections and \textcolor{mygreen}{active} or \textcolor{blue}{inactive} tracks on MOT17 validation set (please refer to Sec. 8 supplementary for details) utilizing different distance measures.
%
In dark and light colors we show the distance of a track to a new detection of the same (positive match) and different (negative match) identity, respectively.

\noindent\textbf{Different handling of active and inactive tracks.} 
%
% We consider a track to be inactive when the method can no longer track \gui{reword} it in the current frame. All other tracks are considered active. 
%
%
% MAYBE RE-ADD / RE-FORMULATE
%Typically trackers only keep inactive tracks for several frames in their memory-bank \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/StadlerB21,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/nips/RenHGS15,DBLP:conf/ijcai/LiuC0Y20}, which means they will only be able to re-identify the target after a short occlusion. With our strong appearance model, we are able to keep \textit{all} \gui{might need to update} inactive tracks in the memory bank for association, hence, we are theoretically able to recover the identity after an occlusion of arbitrary length. \jenny{Yes commented out for now}
While the appearance embeddings of one identity barely vary between two consecutive frames, the embeddings of the same identity before and after occlusion can show larger distances due to, \eg, partial occlusion or varying poses.
%
%
This pattern can be observed in Fig~\ref{fig:distributions}(a) where we visualize the distance between new detections and the last detection of \textcolor{mygreen}{active} or \textcolor{blue}{inactive} tracks. The two dark-coloured histograms vary significantly, which suggestis that a different treatment of \textcolor{mygreen}{active} or \textcolor{blue}{inactive} tracks is necessary. Furthermore, we can see the overlap between both negative and positive matches for \textcolor{blue}{inactive}  tracks showing the inherent difficulty of matching after occlusion.


%to new detections of the same identity (dark colors) and different identities (light colors) are given, respectively. To account for those differences between active and inactive tracks we process both differently. 
% proxy distance
Hence, for \textcolor{mygreen}{active} tracks, we leverage the appearance features of the detection assigned to track $j$ at frame $t-1$ $f_j^{t-1}$ for the distance computation to detection $i$ at frame $t$ $d_{i,j} = d(f_i,f_j^{t-1})$.
For the \textcolor{blue}{inactive} tracks we compute the distance between the appearance feature vectors of all $N_k$ detections in the \textcolor{blue}{inactive} track $k$ and the new detection $i$ and utilize the mean of those distances as a \textit{proxy distance}:
\begin{equation}
    d_{i, k} = \frac{1}{N_k} \sum_{n=1}^{N_k} d(f_i,f_k^n)
\end{equation}
The resulting distance histograms are as visualized in Fig~\ref{fig:distributions}(b). This proxy distance leads to a more robust estimate of the true underlying distance between a detection and an \textcolor{blue}{inactive} track. Hence, in contrast to when using a single feature vector of the \textcolor{blue}{inactive} track (see  Fig~\ref{fig:distributions}(a)) utilizing the proxy distance leads to better-separated histograms (see  Fig~\ref{fig:distributions}(b)).

% 2 thresholds

Moreover, the different histograms of \textcolor{mygreen}{active} and \textcolor{blue}{inactive} trajectories call for different handling during the bipartite matching. To be specific, thresholds typically determine up to which cost a matching should be allowed.
Looking at Fig~\ref{fig:distributions}(b), different thresholds $\tau_i$ divide the histograms of distances from \textcolor{mygreen}{active} and \textcolor{blue}{inactive} trajectories to detections of the same (dark colors) and different (pale colors) identities. Utilizing \textit{different matching thresholds} $\tau_{act}$ and $\tau_{inact}$ for active and inactive trajectories allows us to keep one single matching. In contrast to cascaded matching \cite{DBLP:conf/icip/BewleyGORU16}, our assignment is simpler and avoids applying bipartite matching several times at each frame.




\iffalse
\begin{figure*}{\textwidth}
  \begin{minipage}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures/both.png}
    \captionof{figure}{Analysis of contribution of appearance, motion cues and their combination upon bounding boxes of several private trackers \cite{DBLP:conf/eccv/WangZLLW20,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/cvpr/PangQLCLDY21,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20,DBLP:conf/eccv/PengWWWWTWLHF20}}
    \label{fig:private}
    \vspace{-0.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.38\textwidth}
    \centering
    \input{tables/da_ablation}
    \vspace{0.5cm}    
    \captionof{table}{Ablation of different domain adaptation approaches.}
    \label{tab:domain_adaptation_ablation}
  \end{minipage}
  \vspace{-0.3cm}
\end{figure*}
\fi

% domain adaptation
\noindent\textbf{On-the-fly Domain Adaptation.} As introduced in Section~\ref{sec:related_work}, recent developments in the field of person reID propose to apply domain adaptation (DA) techniques as the source dataset statistics may not match the target ones \cite{DBLP:conf/cvpr/ChoiKJPK21,DBLP:conf/cvpr/ZhaoZYLLLS21,DBLP:conf/eccv/ZhuangWXZZWAT20}. 
%
For MOT this is even more severe since each sequence follows different statistics and represents a new target domain. 
%
We, therefore, propose to apply an on-the-fly DA in order to prevent performance degradation of reID models when applied to varied MOT sequences. This allows us to capitalize on a strong reID over all sequences.


% SHORTEN 
%Recently, several works on person reID introduced approaches utilizing ideas from DA to achieve cross-dataset generalization. MetaBIN \cite{DBLP:conf/cvpr/ChoiKJPK21} utilizes a meta learned mixture of Instance and BN. This prevents filtering out all style information as Instance Normalization would do and failing at generalizing to new styles as BN would do. $M^3L$ \cite{DBLP:conf/cvpr/ZhaoZYLLLS21} utilizes multiple source domains to train a Meta Batch Normalization layer to diversify the features, while CBN \cite{DBLP:conf/eccv/ZhuangWXZZWAT20} utilizes a camera-based BN layer where BN statistics are pre-collected for each camera during test time.
Recently, several works on person reID introduced approaches utilizing ideas from DA to achieve cross-dataset generalization by adapting normalization layers to Instance-Batch, Meta Batch, or Camera-Batch Normalization layers \cite{DBLP:conf/cvpr/ChoiKJPK21,DBLP:conf/cvpr/ZhaoZYLLLS21,DBLP:conf/eccv/ZhuangWXZZWAT20}. 
%\gui{Just saw this comment from ili, and I agree, this seems like a bit too much detail about other methods IMO. I think that the goal of this is to justify that we use a BN-based approach. right?. Could we have instead 1-2 more high level sentences instead? Proposal: Recently, several works on person reID introduced approaches utilizing ideas from DA to achieve cross-dataset generalization by utilizing normalization layers [citations]. While promising, these  approaches either fail to [main reason why they are not great] or require [main reason why they are not easily applicable]}. 
%\ili{this paragraph seems like something that should have been in the related work}\jenny{Yes we were discussion if we leave it here or put it in related work but decided to put it here to make BN-based DA more accessible to revs :)}
%
Contrary to the above-mentioned approaches, we utilize the mean and variance of the features of the current batch, which corresponds to the detections in one frame during test time, in the BN layers of our architecture:

\begin{equation}
    \hat{x_i} = \gamma \frac{x_i - \mu_b}{\sqrt{\sigma_b + \epsilon}} + \beta
\end{equation}

where $x_i$ are features of sample $i$, $\mu_b$ and $\sigma_b$ are the mean and variance of the current batch, $\epsilon$ is a small value that ensures numerical stability, and $\gamma$ and $\beta$ are learned during training. While not requiring any sophisticated training procedure or test time adaptions nor several BN layers, this approximates the statistics of the sequences reasonably well as all images of one sequence have highly similar underlying distributions and leads to more similar distance histograms across tracking sequences. This in turn allows us to define matching thresholds $\tau_i$ that are well suited for all sequences, \textit{i.e.}, that separate all histograms well. For a more detailed analysis please refer to the supplementary material.
%

% SHORTEN
% definition intersection points
%Given two distributions $f_1(x)$ and $f_1(x)$, they intersect at the intersection point $x_{1,2}$ where $f_1(x_{1,2}) = f_2(x_{1,2})$. Intuitively, this intersection point divides positive from negative matches. To find this intersection point we utilize the distribution percentiles (please refer to supplementary material).
% Use it
%Similar intersection points $x_{s, d}^{act}$ between distributions of distances from detections to active tracks of same and different identities $f_{act,s}$ and $f_{act,d}$ across sequences allow to choose one single well suited threshold $\tau_{act}$ for all sequences that separates positive from negative matches. The same holds for the inactive track distributions $f_{inact,s}$ and $f_{inact,d}$ their corresponding threshold $\tau_{inact}$. $x_{s, d}^{inact}$ varies significantly less across tracking sequences when using our on-the-fly DA compared to when not using it (see Figure~\ref{fig:intersection_2}). 
%
%While the $x_{s, d}^{act}$ has a higher variance for both settings, \textit{i.e.}, with and without the on-the-fly DA, the distributions are generally more separated when using DA compared to when not using it (see supplementary material). \jenny{add section with percentile plots in supp}
%This allows to find thresholds $\tau_i$ that are well suited for all tracking sequences when using our DA and directly affects the parameter choices of our appearance model. \jenny{Proposal: Should we move this paragraph and the intersection points figure to supplementary? Feel like we need a bit more space to explain this in detail and we already have ablation experiments on this. if so, we can also switch this and the prior section}


We empirically show that applying these design choices to our appearance model, makes it more robust towards occlusions and better suited for different sequences.

==> cvpr2023-author_kit-v1_1-1/latex/chapters/Realted_Work.tex <==
\section{Related Work}
\label{sec:related_work}
\iffalse
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/pipeline_small1.png}
    \caption{Overview over GHOST where DA represents the domain adaptation. The memory bank contains all \textcolor{blue}{inactive} and \textcolor{green}{active} trajectories but we process both differently. Each tracklet consists of its feature vector and bounding box positions. We utilize the sum of motion and appearance cues for bipartite matching as well as different thresholds for active and inactive trajectories.}
    \label{fig:pipeline}
\end{figure*}
\fi

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \vspace{-0.8cm}
        \includegraphics[width=\textwidth]{figures/last.pdf}
        \vspace{-0.8cm}
        \caption{Appearance}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.27\textwidth}   
        \centering 
        \vspace{-0.8cm}
        \includegraphics[width=\textwidth]{figures/on_the_fly.pdf}
        \vspace{-0.8cm}
        \caption{Proxy Appearance}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.27\textwidth}   
        \centering 
        \vspace{-0.8cm}
        \includegraphics[width=\textwidth]{figures/iou.pdf}
        \vspace{-0.8cm}
        \caption{Motion}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Distance histograms when utilizing (a) the appearance features of the last detection for active and inactive trajectories, (b) the appearance features of the last detection for active and the proxy distance for appearance features of inactive trajectories, (d) the motion distance using IoU measure for active and inactive trajectories.}
    \label{fig:distributions}
    \vspace{-0.5cm}
\end{figure*}


%\jenny{Currently not sure where to best put OUR stuff such that everything is readable in a smooth way here. Also not sure about if we evenn should put the reID paragraph here?}\ili{best way is to position our work in context of others after each paragraph, check my Nvidia paper or any of Aljosa's papers}
In the last years, TbD was the most common paradigm used in MOT %\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20}.
\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/eccv/WangZLLW20,DBLP:journals/ijcv/ZhangWWZL21,DBLP:journals/corr/abs-2103-14258,DBLP:conf/cvpr/PangLZLL20,DBLP:conf/cvpr/PangQLCLDY21,DBLP:conf/cvpr/BrasoL20,DBLP:conf/icml/HornakovaHRS20}. 
Pedestrians are first detected using object detectors \cite{DBLP:conf/nips/RenHGS15,DBLP:conf/cvpr/RedmonF17,DBLP:conf/cvpr/YangCL16}. %which makes the tracking performance heavily dependent on the detection performance. 
Then, detections are associated across frames to form trajectories corresponding to a certain identity utilizing motion, location, appearance cues, or a combination of them. The association can either be solved frame-by-frame for online applications or offline in a track-wise manner over the sequence.

\noindent\textbf{Graph-Based Approaches.}
One common formalism to perform data association following the TbD paradigm is viewing each detection as a node in a graph with edges linking several nodes over the temporal domain to form trajectories. Determining which nodes are connected can then be solved using maximum flow \cite{DBLP:journals/pami/BerclazFTF11} or minimum cost approaches \cite{DBLP:conf/cvpr/JiangFL07,DBLP:conf/cvpr/PirsiavashRF11,DBLP:conf/cvpr/ZhangLN08} by, \textit{e.g}, taking motion models into account \cite{DBLP:conf/iccvw/Leal-TaixePR11}. Recent advances combined track-wise graph-based models with neural networks \cite{DBLP:conf/cvpr/BrasoL20}.
%
%\alj{I would also suggest phrasing this differently! I would not call these architectures “complex”. I think they are nowadays fairly well understood and part of the standard toolbox. I would say instead: aforementioned may work well, but require large amounts of training data. In this work, we re-think this approach and show and we can train strong and light-weight models (with a possible punchline on what exactly drives your simple/data efficient model to work well). Also consider this argument: we can nowadays get lots of data for cars and peds, but what about the long tail? The tail is doomed to be in the “low data” regime. }
%
%The aforementioned approaches may work well, but are rather complex. 
We challenge those recent advances by showing that we can obtain strong TbD trackers without using a complex graph model combining our strong but simple cues. 

%common appearance model enhanced with two design choices trained solely on a commonly used person re-identification (reID) dataset with a linear motion model. 

%However, the recent developments require complex architectures and large amounts of training data. In our work we focus on a simplistic, strong baseline for MOT that challenges the necessity and the real drivers of those recent advances.

\noindent\textbf{Motion-Based Association.}
%\alj{Significantly too long.}
%\ili{why they are good/bad, last sentence should connect to our work}
% without reID
Different from the graph-based approaches, many TbD approaches perform frame-by-frame association directly using motion and location cues from detections and existing trajectories %rather than letting them communicate among each other to associate them
\cite{DBLP:conf/icip/BewleyGORU16,DBLP:conf/avss/BochinskiES17,DBLP:conf/eccv/ZhouKK20,DBLP:conf/eccv/PengWWWWTWLHF20,DBLP:conf/cvpr/PangLZLL20}. For short term preservation, those trackers exploit that given two nearby frames object displacements tend to be small. This allows them to utilize spatial proximity for matching by exploiting, \eg, Kalman filters \cite{DBLP:conf/icip/BewleyGORU16}. Taking this idea further, approaches following the tracking-by-regression paradigm utilize object detectors \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20} to regress bounding box positions. Recent advances introduced Transformer-based approaches \cite{DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2105-03247} that perform tracking following the tracking-by-attention paradigm. 
%
%Some works, \eg, \cite{DBLP:conf/icip/BewleyGORU16}  utilize Kalman filters to predict bounding box position and motion states in the next frame while
% Tracktor
%Tracktor \cite{DBLP:conf/iccv/BergmannML19} leverages the regression head of Faster RCNN detector to predict bounding box positions and drops low confidence boxes.
% CT
%Similarly, CenterTrack \cite{DBLP:conf/eccv/ZhouKK20} propagates bounding box center locations in a frame-wise manner and leverages a greedy matching algorithm to perform association.
%
%It outputs the center heat map of the second, the size of the bounding boxes and the bounding box offset while performing association by greedy matching.
%
%In contrast, Chained-Tracker \cite{DBLP:conf/eccv/PengWWWWTWLHF20} takes two frames chained together as input and predicts the bounding boxes for both at the same time. Pairs of bounding boxes are matched using IoU.
%
%This is further extended in TubeTK \cite{DBLP:conf/cvpr/PangLZLL20} where not only pairs of bounding boxes are matched but bounding-tubes are generated to combine three bounding boxes.
% problem: occlusions
%Using sophisticated motion models, those approaches reach outstanding performance with respect to short-term associations in most scenarios.  However, especially the Transformer-based approaches require sophisticated training strategies and a large amount of data. \jenny{if we don't go the path of data-hungry maybe remove the large abount of data part}
Using sophisticated motion models, those approaches reach outstanding performance on several datasets, especially in short-term associations.  However, especially the Transformer-based approaches require sophisticated training strategies. %and a large amount of data. \jenny{if we don't go the path of data-hungry maybe remove the large abount of data part}
%
Contrary to all those approaches, we show that a simple linear motion model suffices to model short-term associations in most scenarios. 
%
In scenes with moving cameras or scenarios requiring non-trivial long-term associations, \textit{e.g.}, scenarios with many occlusions, purely motion-based trackers struggle which calls for a combination with appearance-based cues.

\noindent\textbf{Appearance-Based Association.}
% \alj{This is also too long and verbose}
To achieve better performance in long-term association scenarios, numerous approaches use additional appearance-based re-identification networks that encode appearance cues to re-identify persons after occlusions \cite{DBLP:conf/eccv/YuLLLSY16,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/BrasoL20,DBLP:conf/cvpr/KimLAR21,DBLP:conf/icip/WojkeBP17,DBLP:conf/cvpr/Leal-TaixeCS16,DBLP:conf/iccv/SadeghianAS17,DBLP:conf/cvpr/SonBCH17}.
%
%To be specific, \cite{DBLP:conf/iccv/BergmannML19} utilizes ResNet50 trained on the task of person reID to generate appearance embeddings. \ili{I do not think the specific backbone has any importance at this stage}
% A recent work \cite{DBLP:conf/cvpr/PangQLCLDY21} introduces an approach that during training leverages the proposals generated by the Faster-RCNN detection backbone and matches them to proposals of the previous frame utilizing appearance embeddings generated by an additional embedding head and a bi-directional softmax. However, it requires an advanced matching scheme during inference to prevent false positive detections to be entangled into the tracklets.
Further exploring this direction, a recent work \cite{DBLP:conf/cvpr/PangQLCLDY21} proposed to train a detection network solely utilizing embedding information during the training process. % However, this requires an advanced matching scheme during inference to prevent false positive detections to be entangled into the tracklets.
%
Enhancing MOT towards real-time, several works proposed to jointly compute detections and embeddings in a multi-task setting \cite{DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/cvpr/GuoWWT21,DBLP:conf/eccv/WangZLLW20,DBLP:conf/cvpr/LuRVH20,DBLP:journals/ijcv/ZhangWWZL21}. Some of them introduce more balanced training schemes \cite{DBLP:conf/cvpr/GuoWWT21,DBLP:conf/cvpr/XuOBHLA20} to better leverage the synergies between both cues.
%However, it is not trivial to achieve the same performance compared to when using a separate reID network \cite{DBLP:conf/cvpr/XuOBHLA20}.
%This is due to the fact that a simple multi-task training is biased towards detection performance and, therefore, a fair, sophisticated training procedure has to be introduced \cite{DBLP:conf/cvpr/XuOBHLA20}.
%However, as multi-task training not fully leverages the full synergies between the detection and embedding head, lately a complex attention-based architecture was introduced \cite{DBLP:conf/cvpr/GuoWWT21}.
%
%
While promising, approaches using appearance additionally to motion cues require rather complex association schemes with several steps \cite{DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/icip/BewleyGORU16}.
%Instead they just combine them in a trivial manner as, \eg, in Tracktor where reID is only used for long-term while motion cues are solely used for short-term associations. 
Also, complex and highly differing training schedules or differing inference strategies make it hard to draw conclusions about what really is driving the progress in the field. 
%
In contrast, GHOST does not rely on complex procedures but combines lightweight motion and spiced-up appearance cues in a simple yet strong TbD tracker that only requires little training data. %\ili{kudos to whomever came with light-weight and spiced-up} %\gui{This looks good! Maybe further add that we use little training data? (since this seems to be a significant part of the story now}
% Our work aims at introducing a strong baseline allowing fair comparisons among the different approaches. It is inspired by the joint usage of reID and motion cues, but differs in several ways from existing works. Unlike the other methods who use reID to boost their performance handling long-term occlusions, \eg, \cite{DBLP:conf/iccv/BergmannML19}, we combine simple reID and motion models in a complementary way for association. To this end, we discover policies to leverage the strengths of both and, therefore, the resulting synergies.

\noindent\textbf{Person Re-Identification and Domain Adaptation.}
In contrast to the tracking domain, the goal of person reID is to retrieve person bounding boxes from a large gallery set that show the same person as a given query image based on appearance cues. %Those query and gallery image sets mostly contain fully visible bounding boxes, which is different to MOT scenario where pedestrians are often occluded.
% domain-adaptation / cross-dataset evaluation
However, state-of-the-art reID models tend to significantly drop in performance when evaluated on out-of-domain samples, \textit{i.e.}, samples coming from other datasets \cite{DBLP:conf/cvpr/ChoiKJPK21,DBLP:conf/cvpr/ZhaoZYLLLS21,DBLP:conf/eccv/ZhuangWXZZWAT20}. As during application, person reID models are applied to different cameras, several approaches on cross-dataset evaluation emerged that transfer the knowledge from a given source, \textit{i.e.}, training to a given target, \textit{i.e.}, test domain utilizing domain adaptation (DA) \cite{DBLP:conf/cvpr/ChoiKJPK21,DBLP:conf/cvpr/ZhaoZYLLLS21,DBLP:conf/eccv/ZhuangWXZZWAT20}. %This is also of major importance for MOT. 
%However, those approaches either are trained using meta-learning and therefore not directly adapted to the target domain \cite{DBLP:conf/cvpr/ChoiKJPK21,DBLP:conf/cvpr/ZhaoZYLLLS21} or use a mixture of BN layers trained on several datasets. \jenny{REF}
%
DA often relies on adapting Batch Normalization (BN) statistics to account for distribution shifts between different domains.
The weight matrix and the BN statistics store label and domain-related knowledge, respectively \cite{DBLP:conf/iclr/LiWS0H17}. 
% OLD
%The misalignment between the shifted features and the weights leads to corrupted predictions. 
%To update the latter, the statistics of BN layers can be updated, \textit{e.g.}, by taking the mean and variance of all target domain images \cite{DBLP:conf/iclr/LiWS0H17}. Similarly, pseudo-labels can be generated using a domain-specific batch normalization to re-train the model using source and target data \cite{DBLP:conf/cvpr/ChangYSKH19}. An approach similar to ours but for classification \cite{DBLP:journals/corr/abs-2006-10963} updates BN statistics during test time but in a batch-wise manner while another work combines train and test datatset statistics in the BN layers \cite{DBLP:conf/nips/SchneiderRE0BB20}. Apart from the statistics, the learned parameters $\beta$ and $\gamma$ can also be updated using entropy minimization \cite{DBLP:conf/iclr/WangSLOD21}. 
% Shortened
To update the latter, the statistics of BN layers can be updated, \textit{e.g.}, by taking the mean and variance of all target domain images \cite{DBLP:conf/iclr/LiWS0H17}, by re-training using pseudo labels \cite{DBLP:conf/cvpr/ChangYSKH19} or combining train and test datatset statistics \cite{DBLP:conf/nips/SchneiderRE0BB20}.
Apart from the statistics, the learned parameters $\beta$ and $\gamma$ can also be updated \cite{DBLP:conf/iclr/WangSLOD21}. 
An approach similar to ours but for classification \cite{DBLP:journals/corr/abs-2006-10963} updates BN statistics during test time in a batch-wise manner.
%
Inspired by those recent advances, we enhance our appearance model to be better suited for MOT using a simple on-the-fly domain adaptation approach. This directly adapts the model's learned training dataset statistics (source) to the sequences (targets).

% Despite its simplicity, our model approach introduces a strong baseline and achieves state-of-the-art performance on MOT17 dataset. 




==> cvpr2023-author_kit-v1_1-1/latex/chapters/acknowledgement.tex <==
\noindent\textbf{Acknowledgements}
This work was partially funded by the Sofja Kovalevskaja Award of the Humboldt Foundation.

==> cvpr2023-author_kit-v1_1-1/latex/chapters/intro_alt.tex <==
\section{Introduction}

% intro to tracking and TBD
Multi-Object Tracking (MOT) aims at finding the trajectories of all moving objects in a video. The dominant paradigm in the field has long been tracking-by-detection, which divides tracking into two steps: (i) frame-wise object detection, (ii) data association to link the detections and form trajectories. 
%
One of the simplest forms of data association for online trackers is frame-by-frame matching using the Hungarian algorithm~\cite{hungarian}. %\lau{Unsure whether to mention offline trackers, maybe not, only at related work we do LP, MPN, etc)}.
%
Matching is often driven by cues such as appearance, \eg, re-identification (reID) features \cite{DBLP:conf/cvpr/0004GLL019,DBLP:journals/corr/HermansBL17,DBLP:conf/iccv/QuanDWZY19,DBLP:conf/cvpr/ChengGZWZ16,DBLP:conf/eccv/SunZYTW18,DBLP:conf/eccv/VariorHW16,DBLP:conf/cvpr/ZhangLZ019}, or motion cues \cite{DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/nips/RenHGS15,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/eccv/PengWWWWTWLHF20}.
%
%Obtaining robust appearance and motion cues even evolved as tasks on their own, namely, re-identification and trajectory prediction. \lau{cite,cite} \gui{Is this true? I see ReID as a task on its own: e.g. chinese government wants to fine you --> it needs to retrieve you from database, doesn't care about your trajectory. Or trajectory prediction is needed for action planning in autonomous driving, regardless of tracking. no?}
%
%Even new learning-based trackers are in need of motion and appearance cues, \eg, Tracktor \cite{DBLP:conf/iccv/BergmannML19} uses external reID and motion priors.
%
Even recent trackers propose data-driven motion priors~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20} or appearance cues, which may include external reID models~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/WuCS00Y21}. 
%

Most recent trackers based on Transformers \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}  learn all necessary cues from data through self- and cross-attention between frames and tracked objects.
%
While this implicitly gets rid of any heuristic typically embedded in the handcrafted appearance and motion cues, and could be the path to more general trackers, the training strategies are highly complex and the amount of data needed to train such models is very large, to the point where MOT datasets \cite{DBLP:journals/ijcv/DendorferOMSCRR21} are not enough and methods rely on pre-training on detection datasets such as CrowdHuman~\cite{crowdhuman}.
%

%Without any prior knowledge, these methods must extract all the information from data, and hence rely on very large amounts of training data, e.g., pre-training on the large scale CrowdHuman~\cite{crowdhuman} has become a necessity to obtain state-of-the-art results in tracking. 
%
%\jenny{actually just realized that this is also done for Byte detections. Maybe we can change it somehow that using an off the shelf object detector pretrained also on several datasets is way easier / that the pre-trainig is a game changer / performance boost for the methods.} \lau{I think the main difference here is that you need to train the whole tracker with these extra datasets, which we do not do, so i think the message can still be said this way. Ofc we use strong private detections, but that is beyond the point here.}

%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects.


%
%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects. 
%
% In a third line, joint-detection-and-embedding approaches emerged that take appearance features directly from the detection backbone. 
%
%While powerful, these methods rely more and more on large amounts of training data, e.g., pre-training on the detection dataset CrowdHuman \lau{cite} has become a necessity to obtain state-of-the-art results. 
%




%\lau{Next is just the spirit of what we want to say, need to find better words.}

%In our view, it would make sense to revisit TbD to see if we can obtain a strong tracker that does not heavily depend on training data.

%\lau{Alternative, you know what i mean...}

%We believe tracking-by-detection should not be discarded just yet, as it shows the clear advantage of being a simple tracker that can be built without large amounts of data. Our question is then: \textit{Can we bring the performance of TbD closer to new paradigms?} \gui{I like this! I don't yet have solid proposal, but I'd like to have an additional motivation for TbD. Do we have any other options? (e.g. long history of research that can be exploited). I think that the link TbD $\approx$ small amounts of data is not super obvious. Another thing that comes to mind (going too deep maybe) is that I believe that the reason why our simple TbD method works so well is partly bc detections are now so good. And detections are so good bc of large amounts of training data... so not sure how solid it is to sell (overall) TbD as good in the low-data regime.}



%While they both differ with respect to their detailed pipeline, they have a strong focus on complex learning-based pipelines. \gui{Not sure that this applies to tracktor/centertrack.}.\lau{Def not, I would say that they do needs large amounts of data to be trained, that is actually true. CT was the first to introduce CH pretraining, so that shows you how much data they need. Trackformer same... tracktor a bit less, but we can generalize here.} Moreover, approaches based on the tracking-by-attention paradigm as well as joint-detection-and-embedding approaches require a large amount of training data. \gui{talking about joint-detection-and-embeddings but they have not yet been introduced }


%A recent work \cite{DBLP:journals/corr/abs-2110-06864} showed that in the presence of high quality object detections, a simple Kalman filter suffices to achieve state-of-the-art performance in MOT. This rises the question which advances are driving the progress in the field. \gui{This last sentence now feels a bit detached from what we've been saying} \lau{I do not know either. I would say, this motivates us to restudy TbD with the new knowledge in machine learning, detectors and architectures.}


% Introducing our approach
%In this work, we follow the spirit of revisiting the TbD paradigm but take the thought further. Instead of solely relying on motion cues which are said to perform bad with respect to long-term associations \textcolor{red}{REF} \gui{I don't like how 'are said to perform bad' sounds, it seems like a weakly presented 'argument from authority'. We need something more powerful as we'are about to motivate what we do differently}, we also utilize appearance features which are often used to overcome those shortcomings. Therefore, we ask the question: How can we leverage synergies between motion and appearance features to further make TbD competitive again? \jenny{MAKE TbD GREAT AGAIN!! :D}  \gui{Wasn't it also part of the story that we show 'the right way' to exploit ReID? Now it seems like the entire weight is on combining reid and motion, which is not that strong results/methodology wise...}
%\lau{Yes, I have always been a fan of the whole reid and not the motion, maybe i need to be more authoritative about this ahahah :D}
%
%We investigate on how to improve basic appearance-based cues as well as
%
%how to best combine motion and appearance within the online TbD framework, obtaining a strong tracker.
%: \textit{do we really need to use sophisticated learning-based frameworks for data association?}
%
%We revisit the association step, showing that it can significantly improve over state-of-the-art models in several datasets.
%
%We do so by exploiting two standard cues, \textit{appearance} and \textit{motion}, within the online TbD framework, obtaining a strong tracker.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/teaser.pdf}
    \vspace{-0.3cm}
    \caption{IDF1/Rank-1 of different state-of-the-art re-ID approaches. R50-TR \cite{torchreid}, BOT \cite{DBLP:conf/cvpr/0004GLL019}, BDB \cite{DBLP:conf/iccv/DaiCGZT19}, ABD \cite{DBLP:conf/iccv/ChenDXYCYRW19}. \textit{Basic} is our baseline, \textit{Ours} is our appearance model.}
    \label{fig:teaser}
    \vspace{-0.6cm}
\end{figure}

%\jenny{Maybe in line with the above comment: we should add here that a well trained detector + simple cues is enough maybe? Would be in line with what the positive reviewer said.} \lau{We are also sota on public detections, no? i do not see the problem then.} We argue that if the appearance and motion cues are strong, we do not need a complex tracker, and a simple frame-by-frame tracking-by-detection will suffice. %\jenny{Are our motion and reid cues strong? Actually they are quite basic, right? And also the detector we utilize was trained on many datasets which I think we cannot just leave our here right?} \lau{Detector is another thing, and we are actually sota with public dets, so I think we dont need to go deep into this in the intro. also strong and simple/basic are not antagonists :)}
%

While interesting and challenging from a research point of view, it is questionable whether we should also follow the path of \textit{learning everything} in multi-object tracking, when there are strong priors that we know how to define and leverage, such as the good old appearance and motion cues. 
%
As we show in this paper, there are key observations that need to be made in order to properly leverage such cues. These observations might seem simple and obvious but have been largely overlooked by the community. If we spend as much time in properly understanding and implementing such cues as we do in training Transformers, we will be rewarded with a simple Hungarian tracker with appearance and motion cues that still dominates state-of-the-art on multiple benchmarks, and does not even need to be trained on any tracking data.


%\jenny{and can be applied to various highly different datasets without much adaption.} \jenny{What if we just drop the requires minimal training data? Then we don't get in the data-hungy confilt and we have the 'never trained on any tracking dataset' later. (not sure about this tho)}


%We therefore propose to revist the roles of the appearance and motion cues for MOT.
%
Our first observation is that simply using state-of-the-art re-identification (reID) networks for appearance matching is not enough for the real scenarios of MOT. In Figure~\ref{fig:teaser}, we visualize the performance of several state-of-the-art reID approaches on Market-1501 dataset \cite{DBLP:conf/iccv/ZhengSTWWT15} (x-axis), as well as the model's performance when used in a simple matching-based tracker (y-axis). It shows that the reID performance does not necessarily translate to MOT performance. %\jenny{Please check.} \lau{awesome}
%\jenny{Our model is far from SOTA in person ReID. We achieve 85 Rank-1 while there is currently stuff our there that reaches 97 Rank-1 or so. We had an analysis in the CVPR version though showing that SOTA ReID does not nessecarity work good. We could show this if we want to keep this message.}
%
%
%
We identify two problems causing the weak performance of reID models on MOT: (i) reID models need to account for the different challenges expected at different time horizons, \ie, while in nearby frames appearance of objects will vary minimally, in longer time gaps more severe changes are expected, \textit{e.g.}, caused by (partial-) occlusions and
%We identify two problems: (i) re-identification in nearby frames is different \lau{i feel my wording here is a tad weak, another for that is not just "different"?} from re-identification in far away frames, where the appearance of the object has potentially changed \gui{models need to account for the different challenges expected at different time horizons: while in nearby frames appearance of objects will vary minimally, in longer time gaps, more severe changes are expected.}. 
(ii) reID performance tends to be inconsistent across MOT sequences because of their varying image statistics, which in turn differs from the relatively stable conditions of the corresponding reID training dataset.
%training and test distributions will be different to the point of making reID methods weak on new sequences. \lau{too sexy?} \gui{I'd word it differently, bc 'all sequences are new sequences in MOT' (if u follow the common practice of not training on MOT seqs), and I'm not sure if this is clear?. Maybe I'd rephrase for smth like?: reid performance tends to be inconsistent across tracking sequences because of their varying image statistics, which in turn differ from the relatively stable conditions of their reid training dataset.'} \jenny{I'm with you Guillem, but I think we should still say sth that they are 'weak' because that's what we are also showing in the teaser. 'training and test distributions will be different and also across tracking sequences image statistics vary heavily. Compared to the relatively stable conditions of the reid training dataset this leads to surprisingly low performance of reID methods in MOT.'}
%
%
We propose two simple but key design choices to overcome the aforementioned problems, \ie, on-the-fly domain adaptation, and different policies for \textcolor{mygreen}{active} and \textcolor{blue}{inactive} tracks.
%
%We propose to enhance our reID algorithm with two key design choices: (i) different policies for active and inactive tracks, and (ii) on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracks, while the latter helps to close the dataset statistics gap between train data and MOT sequences. \lau{I would change the order and first mention the problem and then the solution.} \gui{I agree}
%
% OLD AND NEW
%Our second observation is that often the combination of appearance and motion cues is suboptimal. We therefore conduct an extensive analysis under different conditions of visibility, occlusion time, and camera movement, to determine in which situations reID is not enough and we are in need of a motion model.
Moreover, we conduct an extensive analysis under different conditions of visibility, occlusion time, and camera movement, to determine in which situations reID is not enough and we are in need of a motion model.
%
% OLD AND NEW
%This allows us to determine an intuitive way to combine our reID with a linear motion model, so that each cue can be leveraged in the situation when it is most needed.  
We combine our reID with a simple linear motion model using a weighted sum so that each cue can be given more weight when needed for different datasets. 
%\gui{I'm not sure that what we do is consistent with this paragraph: we combine motion and appearance just like other methods (by summing, them, no?. Maybe I'd just change the first line, and refer to the limitations of ReID (not how other methods use it)}
%

Our findings culminate in our proposed \textbf{G}ood \textbf{O}ld \textbf{H}ungarian \textbf{S}imple \textbf{T}racker 
 or \textbf{GHOST} (the order of the letters of the acronym does not change the product) that generalizes to four different datasets, remarkably outperforming the state-of-the-art while, most notably, \textit{never being trained on any tracking dataset}. %showing good generalization. 
%\jenny{I'm still not sure if we can say it like this because our detections are. But I think this is just because recently detectors and trackers are more and more entangled :)}
%\lau{Yes but that is their problem, right? I mean detection datasets you have a million, tracking not so much, so training a strong detector is arguably easier. We dont really lie here, we jus say our tracker does not need much data, plus we are also strong in public detections, so its not only when detector is strong.} \jenny{Convinced :)}


% go a bit more precise

%Our approach consists of a matching-based tracker that performs association in one single step utilizing an affinity score based on the appearance and motion cues between past \gui{tracks} and current detections at every frame.
%
%We obtain our appearance information from a standard re-identification (ReID) network, whose performance we enhance with two design choices: different handling of active and inactive tracklets and on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracklets while the latter helps to close the dataset statistics gap between train data and MOT sequences. 
%
%Our motion term relies on the predictions of a linear motion model over past tracks. \gui{Maybe comment that we find it works incredibly well?
%}
% 
%We do an extensive analysis, determining that visibility, occlusion time, and camera movement heavily influence the performance of ReID and motion systems.
%
%Following that, we introduce a probabilistic policy to determine in which scenarios motion and ReID give more trustworthy similarity predictions given the underlying conditions and combine both appropriately.
%
%, and we demonstrate with our experimental analysis that our strong performance originates from improved data association.


% not sure if this goes here
\iffalse
Our work serves three main purposes. We demonstrate that using a strong, yet conceptually simple data association scheme can further revive the TbD paradigm.
%
We believe this is valuable by itself and expect to make future work question the need for sophisticated learning-based approaches.
%
Furthermore, we demonstrate how to improve appearance cues following our simple design choices.
%Furthermore, our tracking analysis sheds light on what are the pressing challenges of tracking that both our method as well as previous top-performing ones still struggle to address.
Finally, based on a tracking analysis we shed light on how to combine motion and ReID in way to best exploit both cues.
%
We expect that the insights presented in this paper will encourage subsequent methods to target their effort towards solving them.

\fi 

\vspace{0.3cm}
%\lau{Contributions: 1. We propose key changes to reid so that it works. 2. We analyze where appearance and motion have the potential to be useful to increase performance wrt current trackers. 3. We show SOTA with a simple tracker cos we are awesome.}

\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We provide key design choices that significantly boost the performance of reID models for the MOT task.
    % \item We extensively analyze in which cases appearance and motion have the potential to increase performance with respect to current trackers.
    \item We extensively analyze in which underlying situations appearance is not sufficient and when it can be backed up by motion.
    %\item We achieve state-of-the-art performance on several benchmarks with our simple and general tracking-by-detection online tracker GHOST.
    \item We generalize to four datasets achieving state-of-the-art performance by combining appearance and motion in our simple and general TbD online tracker GHOST.
\end{itemize}
%All code and models will be made publicly available upon acceptance.

%\gui{I know this is not easy, but since we have a relatively 'exotic' paper, questioning current trends, I think it'd be nice if we were a bit more specific on how  we expect our results to impact future research. What should our paper make future tracking research change based on what we show, exactly? What is the main takeaway ? Example: people should think about Domain adaptation and appearance (ReID performance across diff sequences), the different challenges of short/long term association (e.g. we use two thresholds/proxies), people should think about interplay of motion and appearance in different circumstances. We showed a simple but strong version of how to operationalize these insights, people should look for fancier models while keeping these important tracking aspects in mind, not simply going all in on transformers. What do you think? Something along these lines could be placed either here in intro/conclusions, or at the experiments, after analysis, to make it look a bit more relevant for the overall paper.} \jenny{Really good idea/comment!! Tried to make a paragraph out of your thoughts, can you check? (below). We could acutally have the big paragraph here and then refer to it / repeat parts of it over the paper again at the corresponding sections.}


%\lau{Totally agree with guillem, but i think the above paragraph is still not there yet. Things i would highlight: 1. We show that the previous idea of reid was far too simplistic, it only works if u train on extremely similar data as test. Current reid models do not work out of the box and the transfer to tracking is much less stable that previously thought --> adaptation is needed as we show or maybe more robust models --> future work. 2. analysis of the interplay between reid and motion, here again, it seems a simple combination is not the way to go but rather an analysis of when what can be used. 3. Overall, maybe learn-all transformers outperformed more classic models because classic models were not being used properly.  We should rethink the "let us throw data at the problem" for tracking because the "old" knowledge is still very much SOA. }


% OPTION ONE
%Overlooked by the community until now, we hope our work inspires future approaches to overthink the current usage of reID and the integration of domain adaption as well as how approach the differences between short and long term association, \textit{e.g.}, with different appearance proxies for active and inactive tracks. Moreover, our analysis shows the interplay between motion and appearance in different circumstances. Introducing a simple but strong version of how to utilize those insights, we hope to inspire future work to integrate this interplay into novel, sophisticated models further improving the state of the art.

%\lau{maybe too poetic}

% OPTION TWO
With this paper, we hope to show the importance of domain-specific knowledge and the impact it can have, even on the simple good old models.
%
%While research on fully data-driven trackers is flourishing and should continue to do so, leveraging modern machine learning knowledge and domain-specific knowledge to create simple and data lean solutions should also get its share of attention.
%
Our observations, \textit{i.e.}, the importance of domain adaptation, the different handling of short- and long-term associations as well as the interplay between motion and appearance are straightforward, almost embedded into the subconscious of the tracking community, and yet they have largely been overlooked by recent methods. %. \gui{maybe let's say 'by recent methods'?} 
%
Introducing our simple but strong tracker, we hope our observations will inspire future work to integrate such observations into sophisticated models further improving the state of the art, in a solution where data and priors will gladly meet.

% \lau{I still do not like this paragraph.} \gui{I think it's good!} \ili{looks more like something that fits in broader impact rather than in intro}

\iffalse
\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We do an extensive analysis, determining the most important factors that determine the performance of ReID and motion systems.
    \item Based on our analysis, we provide a strong probabilistic scheme for data association that combines appearance and motion cues using a derived policy.
    \item We obtain state-of-the art results on several benchmarks, etc. \ili{more precise, give numbers already}
\end{itemize}
\fi

==> cvpr2023-author_kit-v1_1-1/latex/chapters/intro_shortened.tex <==
\section{Introduction}

% intro to tracking and TBD
Multi-Object Tracking (MOT) aims at finding the trajectories of all moving objects in a video. The dominant paradigm in the field has been tracking-by-detection, which divides tracking into two steps: (i) frame-wise object detection, (ii) data association to link the detections and form trajectories. 
%
In online tracking, where only the past is accessible, one of the simplest forms of data association is frame-by-frame matching using the Hungarian algorithm~\cite{hungarian} %\ili{should you define what are online trackers before mentioning them?}. %\lau{Unsure whether to mention offline trackers, maybe not, only at related work we do LP, MPN, etc)}.
%
Matching is then driven by cues such as appearance, \eg, re-identification (reID) features \cite{DBLP:conf/cvpr/0004GLL019,DBLP:journals/corr/HermansBL17,DBLP:conf/iccv/QuanDWZY19,DBLP:conf/cvpr/ChengGZWZ16,DBLP:conf/eccv/SunZYTW18,DBLP:conf/eccv/VariorHW16,DBLP:conf/cvpr/ZhangLZ019} or motion cues \cite{DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/nips/RenHGS15,DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/XuOBHLA20,DBLP:conf/eccv/PengWWWWTWLHF20}.
%

%Obtaining robust appearance and motion cues even evolved as tasks on their own, namely, re-identification and trajectory prediction. \lau{cite,cite} \gui{Is this true? I see ReID as a task on its own: e.g. chinese government wants to fine you --> it needs to retrieve you from database, doesn't care about your trajectory. Or trajectory prediction is needed for action planning in autonomous driving, regardless of tracking. no?}
%



%Even new learning-based trackers are in need of motion and appearance cues, \eg, Tracktor \cite{DBLP:conf/iccv/BergmannML19} uses external reID and motion priors.
%
Recent learning-based trackers still rely on motion priors~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21,DBLP:conf/eccv/ZhouKK20} or appearance cues, which may include external reid models~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/WuCS00Y21}. 
%
Modern trackers based on Transformers \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247} learn all necessary cues from data through self- and cross-attention between frames and tracked objects.
%
While powerful, these methods rely on large amounts of training data, e.g., pre-training on the large scale CrowdHuman~\cite{crowdhuman} has become a necessity to obtain state-of-the-art results. %\jenny{actually just realized that this is also done for Byte detections. Maybe we can change it somehow that using an off the shelf object detector pretrained also on several datasets is way easier / that the pre-trainig is a game changer / performance boost for the methods.} \lau{I think the main difference here is that you need to train the whole tracker with these extra datasets, which we do not do, so i think the message can still be said this way. Ofc we use strong private detections, but that is beyond the point here.}

%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects.


%
%Recently, the field drifted away from TbD towards new paradigms, e.g., tracking-by-regression \cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/eccv/ZhouKK20,DBLP:conf/cvpr/StadlerB21,DBLP:conf/cvpr/WuCS00Y21} and tracking-by-attention \cite{DBLP:journals/corr/abs-2012-15460,DBLP:journals/corr/abs-2101-02702,DBLP:journals/corr/abs-2105-03247}. The former utilizes object detectors to regress bounding box positions from one frame to another. The latter builds on Transformer \cite{DBLP:conf/nips/VaswaniSPUJGKP17} architectures and exploits attention mechanisms between frames and tracked objects. 
%
% In a third line, joint-detection-and-embedding approaches emerged that take appearance features directly from the detection backbone. 
%
%While powerful, these methods rely more and more on large amounts of training data, e.g., pre-training on the detection dataset CrowdHuman \lau{cite} has become a necessity to obtain state-of-the-art results. 
%




%\lau{Next is just the spirit of what we want to say, need to find better words.}

%In our view, it would make sense to revisit TbD to see if we can obtain a strong tracker that does not heavily depend on training data.

%\lau{Alternative, you know what i mean...}

%We believe tracking-by-detection should not be discarded just yet, as it shows the clear advantage of being a simple tracker that can be built without large amounts of data. Our question is then: \textit{Can we bring the performance of TbD closer to new paradigms?} \gui{I like this! I don't yet have solid proposal, but I'd like to have an additional motivation for TbD. Do we have any other options? (e.g. long history of research that can be exploited). I think that the link TbD $\approx$ small amounts of data is not super obvious. Another thing that comes to mind (going too deep maybe) is that I believe that the reason why our simple TbD method works so well is partly bc detections are now so good. And detections are so good bc of large amounts of training data... so not sure how solid it is to sell (overall) TbD as good in the low-data regime.}



%While they both differ with respect to their detailed pipeline, they have a strong focus on complex learning-based pipelines. \gui{Not sure that this applies to tracktor/centertrack.}.\lau{Def not, I would say that they do needs large amounts of data to be trained, that is actually true. CT was the first to introduce CH pretraining, so that shows you how much data they need. Trackformer same... tracktor a bit less, but we can generalize here.} Moreover, approaches based on the tracking-by-attention paradigm as well as joint-detection-and-embedding approaches require a large amount of training data. \gui{talking about joint-detection-and-embeddings but they have not yet been introduced }


%A recent work \cite{DBLP:journals/corr/abs-2110-06864} showed that in the presence of high quality object detections, a simple Kalman filter suffices to achieve state-of-the-art performance in MOT. This rises the question which advances are driving the progress in the field. \gui{This last sentence now feels a bit detached from what we've been saying} \lau{I do not know either. I would say, this motivates us to restudy TbD with the new knowledge in machine learning, detectors and architectures.}


% Introducing our approach
%In this work, we follow the spirit of revisiting the TbD paradigm but take the thought further. Instead of solely relying on motion cues which are said to perform bad with respect to long-term associations \textcolor{red}{REF} \gui{I don't like how 'are said to perform bad' sounds, it seems like a weakly presented 'argument from authority'. We need something more powerful as we'are about to motivate what we do differently}, we also utilize appearance features which are often used to overcome those shortcomings. Therefore, we ask the question: How can we leverage synergies between motion and appearance features to further make TbD competitive again? \jenny{MAKE TbD GREAT AGAIN!! :D}  \gui{Wasn't it also part of the story that we show 'the right way' to exploit ReID? Now it seems like the entire weight is on combining reid and motion, which is not that strong results/methodology wise...}
%\lau{Yes, I have always been a fan of the whole reid and not the motion, maybe i need to be more authoritative about this ahahah :D}
%
%We investigate on how to improve basic appearance-based cues as well as
%
%how to best combine motion and appearance within the online TbD framework, obtaining a strong tracker.
%: \textit{do we really need to use sophisticated learning-based frameworks for data association?}
%
%We revisit the association step, showing that it can significantly improve over state-of-the-art models in several datasets.
%
%We do so by exploiting two standard cues, \textit{appearance} and \textit{motion}, within the online TbD framework, obtaining a strong tracker.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/teaser.jpg}
    \caption{IDF1/Rank-1 of different state-of-the-art re-ID approaches. R50-TR \cite{torchreid}, BOT \cite{DBLP:conf/cvpr/0004GLL019}, BDB \cite{DBLP:conf/iccv/DaiCGZT19}, ABD \cite{DBLP:conf/iccv/ChenDXYCYRW19}. \textit{Basic} is our baseline, \textit{Ours} is our appearance model.}
    \label{fig:teaser}
\end{figure}

%\jenny{Maybe in line with the above comment: we should add here that a well trained detector + simple cues is enough maybe? Would be in line with what the positive reviewer said.} \lau{We are also sota on public detections, no? i do not see the problem then.}
We argue that if the appearance and motion cues are strong \jenny{our motion is actually not pretty strong/fancey?}, we do not need a complex tracker, and a simple frame-by-frame tracking-by-detection will suffice. %\jenny{Are our motion and reid cues strong? Actually they are quite basic, right? And also the detector we utilize was trained on many datasets which I think we cannot just leave our here right?} \lau{Detector is another thing, and we are actually sota with public dets, so I think we dont need to go deep into this in the intro. also strong and simple/basic are not antagonists :)}
%
We therefore propose to revist the roles of the appearance and motion cues for MOT.
%
Our first observation is that simply using state-of-the-art re-identification (reID) networks for appearance matching is not enough for the real scenarios of MOT. In Figure~\ref{fig:teaser}, we visualize the performance of several state-of-the-art reID approaches on Market-1501 dataset \cite{DBLP:conf/iccv/ZhengSTWWT15} (x-axis), as well as the models performance when used in a simple matching-based tracker (y-axis). It shows that the reID performance does not necessarily translate to MOT performance. %\jenny{Please check.} \lau{awesome}
%\jenny{Our model is far from SOTA in person ReID. We achieve 85 Rank-1 while there is currently stuff our there that reaches 97 Rank-1 or so. We had an analysis in the CVPR version though showing that SOTA ReID does not nessecarity work good. We could show this if we want to keep this message.}
%


We identify two problems causing the weak performance of reID models on MOT: (i) reID models need to account for the different challenges expected at different time horizons, \ie, while in nearby frames appearance of objects will vary minimally, in longer time gaps more severe changes are expected, and
%We identify two problems: (i) re-identification in nearby frames is different \lau{i feel my wording here is a tad weak, another for that is not just "different"?} from re-identification in far away frames, where the appearance of the object has potentially changed \gui{models need to account for the different challenges expected at different time horizons: while in nearby frames appearance of objects will vary minimally, in longer time gaps, more severe changes are expected.}. 
(ii) reID performance tends to be inconsistent across MOT sequences because of their varying image statistics, which in turn differ from the relatively stable conditions of the corresponding reID training dataset.
%training and test distributions will be different to the point of making reID methods weak on new sequences. \lau{too sexy?} \gui{I'd word it differently, bc 'all sequences are new sequences in MOT' (if u follow the common practice of not training on MOT seqs), and I'm not sure if this is clear?. Maybe I'd rephrase for smth like?: reid performance tends to be inconsistent across tracking sequences because of their varying image statistics, which in turn differ from the relatively stable conditions of their reid training dataset.'} \jenny{I'm with you Guillem, but I think we should still say sth that they are 'weak' because that's what we are also showing in the teaser. 'training and test distributions will be different and also across tracking sequences image statistics vary heavily. Compared to the relatively stable conditions of the reid training dataset this leads to surprisingly low performance of reID methods in MOT.'}
%
%
We propose two simple but key design choices to overcome the aforementioned problems, \ie, on-the-fly domain adaptation, and different policies for active and inactive tracks.

%We propose to enhance our reID algorithm with two key design choices: (i) different policies for active and inactive tracks, and (ii) on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracks, while the latter helps to close the dataset statistics gap between train data and MOT sequences. \lau{I would change the order and first mention the problem and then the solution.} \gui{I agree}
%
We then do an extensive analysis under different conditions of visibility, occlusion time, and camera movement, to determine in which situations reID is not enough and we are in need of a motion model.
%
%\lau{Ok here I think we should say nothing about the motion model. The sentence before and after already match, so I think we can leave it as is and not speculate here about motion. What do you think?}
%Maybe surprisingly, a linear motion model over the past tracks works incredibly well. \gui{I'd rewrite these two sentences but I like the overall approach of how motion is introduced into the conversation} \lau{I might delete the second sentence and just leave the first, and go from "we need a motion model" to the simple combo that reaches sota.} \gui{proposal (not sure if we wanna go there though): we find that while ReID might struggle under occlusions in some situations, a simple motion model can compensate for most its failures.}\lau{risky}\jenny{Maybe surprisingly, a linear motion model over the past tracks complements reID incredibly well.}
%
Our experiments show that combining our ReID with a linear motion model suffices to obtain a tracking-by-detection tracker without any bells and whistles that significantly outperforms state-of-the-art \jenny{to be adapted}.
%
Most notably, \textit{our reID model is never trained on any tracking dataset, showing good generalization.} %\ili{put this sentence in bold/italic!}
%\jenny{I'm still not sure if we can say it like this because our detections are. But I think this is just because recently detectors and trackers are more and more entangled :)}
%\lau{Yes but that is their problem, right? I mean detection datasets you have a million, tracking not so much, so training a strong detector is arguably easier. We dont really lie here, we jus say our tracker does not need much data, plus we are also strong in public detections, so its not only when detector is strong.} \jenny{Convinced :)}


% go a bit more precise

%Our approach consists of a matching-based tracker that performs association in one single step utilizing an affinity score based on the appearance and motion cues between past \gui{tracks} and current detections at every frame.
%
%We obtain our appearance information from a standard re-identification (ReID) network, whose performance we enhance with two design choices: different handling of active and inactive tracklets and on-the-fly domain adaptation. The former accounts for highly differing distributions of distances from new detections to active and inactive tracklets while the latter helps to close the dataset statistics gap between train data and MOT sequences. 
%
%Our motion term relies on the predictions of a linear motion model over past tracks. \gui{Maybe comment that we find it works incredibly well?
%}
% 
%We do an extensive analysis, determining that visibility, occlusion time, and camera movement heavily influence the performance of ReID and motion systems.
%
%Following that, we introduce a probabilistic policy to determine in which scenarios motion and ReID give more trustworthy similarity predictions given the underlying conditions and combine both appropriately.
%
%, and we demonstrate with our experimental analysis that our strong performance originates from improved data association.


% not sure if this goes here
\iffalse
Our work serves three main purposes. We demonstrate that using a strong, yet conceptually simple data association scheme can further revive the TbD paradigm.
%
We believe this is valuable by itself, and expect to make future work question the need for sophisticated learning-based approaches.
%
Furthermore, we demonstrate how to improve appearance cues following our simple design choices.
%Furthermore, our tracking analysis sheds light on what are the pressing challenges of tracking that both our method as well as previous top-performing ones still struggle to address.
Finally, based on a tracking analysis we shed light on how to combine motion and ReID in way to best exploit both cues.
%
We expect that the insights presented in this paper will encourage subsequent methods to target their effort towards solving them.

\fi 

\vspace{0.3cm}
%\lau{Contributions: 1. We propose key changes to reid so that it works. 2. We analyze where appearance and motion have the potential to be useful to increase performance wrt current trackers. 3. We show SOTA with a simple tracker cos we are awesome.}

\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We provide key design choices that significantly boost the performance of reID models for the MOT task.
    \item We extensively analyze in which cases appearance and motion have the potential to increase performance with respect to current trackers.
    \item We obtain state-of-the-art results on several benchmarks with a simple tracking-by-detection online tracker.
\end{itemize}
%All code and models will be made publicly available upon acceptance.

%\gui{I know this is not easy, but since we have a relatively 'exotic' paper, questioning current trends, I think it'd be nice if we were a bit more specific on how  we expect our results to impact future research. What should our paper make future tracking research change based on what we show, exactly? What is the main takeaway ? Example: people should think about Domain adaptation and appearance (ReID performance across diff sequences), the different challenges of short/long term association (e.g. we use two thresholds/proxies), people should think about interplay of motion and appearance in different circumstances. We showed a simple but strong version of how to operationalize these insights, people should look for fancier models while keeping these important tracking aspects in mind, not simply going all in on transformers. What do you think? Something along these lines could be placed either here in intro/conclusions, or at the experiments, after analysis, to make it look a bit more relevant for the overall paper.} \jenny{Really good idea/comment!! Tried to make a paragraph out of your thoughts, can you check? (below). We could acutally have the big paragraph here and then refer to it / repeat parts of it over the paper again at the corresponding sections.}

%\ili{is the part after the bullet points legit for this version of the paper?}

The current simplistic usage of of-the-shelf pre-trained ReID networks does not leverage the full potential appearance as networks only perform well on data that is highly similar to the train set. This leads to less stable results in tracking. Our work highlights the need of more robust models and domain adaptation which we hope inspires future works. 
%
Moreover, our analysis shows that the interplay between motion and appearance holds high potential. While our simple but strong version already achieves state-of-the-art performance, we hope future work to investigate this interplay even more. 
%
Consequently, we propose to rethink recent developments of ever increasing data-hungry trackers towards learning more from well-known concepts. Without much adaption between highly differing datasets, they still can achieve state-of-the-art performance.

%Overlooked by the community until now, we hope our work inspires future approaches to overthink the current usage of reID and the integration of domain adaption as well as how approach the differences between short and long term association, \textit{e.g.}, with different appearance proxies for active and inactive tracks. Moreover, our analysis shows the interplay between motion and appearance in different circumstances. Introducing a simple but strong version of how to utilize those insights, we hope to inspire future work to integrate this interplay into novel, sophisticated models further improving the state of the art.


%\lau{Totally agree with guillem, but i think the above paragraph is still not there yet. Things i would highlight: 1. We show that the previous idea of reid was far too simplistic, it only works if u train on extremely similar data as test. Current reid models do not work out of the box and the transfer to tracking is much less stable that previously thought --> adaptation is needed as we show or maybe more robust models --> future work. 2. analysis of the interplay between reid and motion, here again, it seems a simple combination is not the way to go but rather an analysis of when what can be used. 3. Overall, maybe learn-all transformers outperformed more classic models because classic models were not being used properly.  We should rethink the "let us throw data at the problem" for tracking because the "old" knowledge is still very much SOA. }

\iffalse
\noindent In summary, we make the following contributions:
\begin{itemize}
    \item We do an extensive analysis, determining the most important factors that determine the performance of ReID and motion systems.
    \item Based on our analysis, we provide a strong probabilistic scheme for data association that combines appearance and motion cues using a derived policy.
    \item We obtain state-of-the art results on several benchmarks, etc. \ili{more precise, give numbers already}
\end{itemize}
\fi

==> cvpr2023-author_kit-v1_1-1/latex/chapters/supp_extra.tex <==
\appendix

%%%%%%%%% ABSTRACT
\textbf{{\larger[2] Supplementary Material}}
\newline


In this supplementary material, we first comment on novelty in science in Section~\ref{sec:novelty} before we show results on integrating GHOST into to tracking appeoaches in Section~\ref{sec:baseline}. The, we give the per-class performance of GHOST on BDD100k validation set in Section~\ref{sec:bdd}. In Section~\ref{sec:detailed_rca} we introduce the computation of the rate of correct associations (RCA) followed by a deeper analysis of it. We then conduct a deeper analysis of our domain adaptation in Section~\ref{sec:inter}. Afterwards, we show how we choose parameters based on our analysis in Section~\ref{sec:knowledge} and deeper investigate on the usage of different proxies in Section~\ref{sec:proxies}, the combination of appearance and motion using different weights for the sum in Section~\ref{sec:weights}, the number of frames to be used to approximate the velocity in Section~\ref{sec:num_frames} as well as on how to utilize different thresholds in Section~\ref{sec:threshs}. Also, we conduct experiments on different values of inactive patience in Section~\ref{sec:memory}. Then, we introduce how we generated the distance histograms in Section~\ref{sec:distance_dist}.
%
Moreover, in Section~\ref{sec:similar} we first outline the difference between our approach and trackers with similar components and compare the generality of our model to the generality of ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} in Section~\ref{sec:generality}. Finally, we comment on the latency of our approach in Section~\ref{sec:latency}, and visualize several long-term occluded and low visibility bounding boxes on MOT17 public detection that GHOST successfully associates in Section~\ref{sec:vis}.


\section{"A painting can be beautiful even if it is simple and the technical complexity is low. So can a paper." \cite{OnNovelty}.}
\label{sec:novelty}
Inspired by the blog post of Michael Black on novelty in science \cite{OnNovelty}, we would like to discuss the common understanding of novelty in this paragraph.
%
Despite often confused, incremental changes do not necessarily mean that a paper can not introduce novelty and novel ideas. "If nobody thought to change that one term, then it is ipso facto novel. The inventive insight is to realize that a small change could have a big effect and to formulate the new loss" \cite{OnNovelty}.
%
Furthermore, it is of major importance to sometimes step back and formulate "a simple idea" since this "means stripping away the unnecessary to reveal the core of something. This is one of the most useful things that a scientist can do." \cite{OnNovelty}. If a simple idea improves the state of the art, "then it is most likely not trivial" \cite{OnNovelty}. 
%
Technical novelty is the most obvious type of novelty that reviewers look for in papers, but it is not the only one \cite{OnNovelty}.
%
In our understanding, if the reader takes away an idea from the paper that changes the way they do research, this can be considered a positive impact of the paper. Hence, the paper is novel (it has sparked a new idea in the reader’s mind). 
%
We hope readers also see it that way and we can progress with simpler, more interpretable, stronger models, and not only complex transformer-based pipelines trained on huge GPU farms. 
\input{tables_supp/bdd}
\begin{table}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}l|l|ccc|ccc@{}}
\hline
& & \multicolumn{3}{c}{Original} & \multicolumn{3}{c}{Original + GHOST} \\
\hline
 & dataset & HOTA & IDF1 & MOTA & HOTA & IDF1 & MOTA\\
 \hline
ByteTrack & DanceTrack & 47.1 & 51.9 & 88.3 & 54.0 & 89.5 & 54.5 \\
Tracktor & MOT17 & 57.7 & 65.9 & 61.8 & 58.7 & 67.5 & 61.8 \\
\hline
\end{tabular}}
\caption{Applying GHOST in other Trackers.}
\label{tab:reb1}
\end{table}


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-02-FRCNN_plot.png}
        \caption{MOT17-02 \textit{S}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-04-FRCNN_plot.png}
        \caption{MOT17-04 \textit{S}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-05-FRCNN_plot.png}
        \caption{MOT17-05 \textit{M}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-09-FRCNN_plot.png}
        \caption{MOT17-09 \textit{S}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-10-FRCNN_plot.png}
        \caption{MOT17-10 \textit{M}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-11-FRCNN_plot.png}
        \caption{MOT17-11 \textit{M}}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_visMOT17-13-FRCNN_plot.png}
        \caption{MOT17-13 \textit{M}}
    \end{subfigure}
    \caption{RCA for static \textit{S} and moving \textit{M} sequences with respect to visibility.}
    \label{fig:seq_analysis_vis}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-02-FRCNN_plot.png}
        \caption{MOT17-02 \textit{S}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-04-FRCNN_plot.png}
        \caption{MOT17-04 \textit{S}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-05-FRCNN_plot.png}
        \caption{MOT17-05 \textit{M}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-09-FRCNN_plot.png}
        \caption{MOT17-09 \textit{S}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-10-FRCNN_plot.png}
        \caption{MOT17-10 \textit{M}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-11-FRCNN_plot.png}
        \caption{MOT17-11 \textit{M}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{figures_supp/binned_frame_distMOT17-13-FRCNN_plot.png}
        \caption{MOT17-13 \textit{M}}
    \end{subfigure}
    \caption{RCA for static \textit{S} and moving \textit{M} sequences with respect to short-term vs. long-term associations.}
    \label{fig:seq_analysis_occ}
\vspace{-0.3cm}
\end{figure*}



\section{Integrating GHOST within Other Trackers.} 
\label{sec:baseline}
Our baseline in the main paper is the simple Hungarian tracker in introduced in Sec 3.1. Furthermore, we apply GHOST additionally to other trackers as visualized in Fig 3 of the main paper. However, to show that it can also be integrated into existing trackers, in Tab~\ref{tab:reb1} we provide the performance of utilizing our reID instead of the baseline reID in Tracktor on MOT17. Since Tracktor on its own is a motion model we cannot apply our linear motion. Moreover, we provide results on utilizing our reID model and our linear motion instead of the Kalman Filter in ByteTrack on DanceTrack. Apart from the gain of using reID, the Kalman Filter struggles with the extreme motion while we can adapt the number of frames for velocity computation to the dataset.  %\jenny{maybe remove following due to space}For example, not using any appearance features leads to a performance drop of 3.4 pp in IDF1 and 0.9 pp in HOTA metrics. Also, taking only a few frames to approximate the velocity in the linear motion model leads to an improvement of up to 2 pp in IDF1 and 1.4 pp in HOTA metric.



\section{Per-Class Evaluation on BDD100k Validation Set}
\label{sec:bdd}
In this section, we show the class-wise performance on the BDD100k validation set (Table~\ref{tab:bdd}). As on the test set (see main paper), we perform better than ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} and QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} in the overall IDF1 and HOTA metrics as well as in IDF1 and HOTA of less frequent classes like rider, bus, bycicle. 
%
On the other hand, QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} outperforms us in the overall IDF1 metric per detection box, mainly due to their higher performance for highly frequent classes like car or pedestrian. 
%
This shows that QDTrack works well only for highly frequent classes, indicating a high dependency to the train set. Note, our model is only trained on the pedestrian class, which makes our performance on other classes a good demonstration of the generality of our approach. 

\section{Detailed Analysis of Rate of Correct Associations per Sequence}
\label{sec:detailed_rca}
We show a per sequence analysis of the rate of correct associations (RCA) of motion and appearance with respect to visibility in Fig~\ref{fig:seq_analysis_vis}, and short-term vs. long-term association in Fig~\ref{fig:seq_analysis_occ} where \textit{M} indicates moving sequence and \textit{S} indicates static sequence. For this we first introduce how to compute the RCA value.

\noindent\textbf{Computation of RCA.}
Given the output file of a tracker, to compute the rate of correct associations (RCA), we first match the given detections to ground truth identities following the same matching as the one used for the computation of the MOTA metric \cite{DBLP:journals/pami/KasturiGSMGBBKZ09}. 
%
For each detection $o_i$, we then find the last previous detection that belongs to the same ground truth ID $o_{i, prev}$. If $o_{i}$ was assigned to the same tracker ID as $o_{i, prev}$, we count it as a true positive association (TP-Ass), and if it was assigned to a different tracker ID, we count it as a false positive association (FP-Ass). This leads to the RCA value:
\begin{equation}
    RCA = \frac{\text{TP-Ass}}{\text{FP-Ass} + \text{TP-Ass}},
\end{equation}
To get the performance for different visibility levels and occlusion time, we organize $o_i$ into bins. For example, when we investigate the performance for visibility $0-33\%$, we take only detections $o_i$ into account that are $0-33\%$ visible. The same holds for occlusion time: if we investigate occlusion time $0.5-0.7s$, we only take detections $o_i$ into account whose prior detection of the same ground truth ID was $0.5-0.7s$ ago.
%
This procedure allows us to investigate the performance of different trackers with respect to different influencing factors solely based on the detection output files. 

\begin{figure*}[htp!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures_supp/quantilles_actcenter.pdf}
        \caption{Without on-the-fly domain adaptation.}
        \label{fig:quantilles_act_without}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.45\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/on_the_fly_quantilles_actcenter.pdf}
        \caption{With on-the-fly domain adaptation.}
        \label{fig:quantilles_act_with}
    \end{subfigure}
    \caption{Cumulative sum of absolute bin difference between $f_{a,d}$ and $f_{a,s}$ on MOT17 validation set.}
    \label{fig:quantilles_act}
    \vspace{-0.3cm}
\end{figure*}

\begin{figure*}[htp!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures_supp/quantilles_inactcenter.pdf}
        \caption{Without on-the-fly domain adaptation.}
        \label{fig:quantilles_inact_without}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.45\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/on_the_fly_quantilles_inactcenter.pdf}
        \caption{With on-the-fly domain adaptation.}
        \label{fig:quantilles_inact_with}
    \end{subfigure}
    \caption{Cumulative sum of absolute bin difference between $f_{a,d}$ and $f_{a,s}$ on MOT17 validation set.}
    \label{fig:quantilles_inact}
    \vspace{-0.6cm}
\end{figure*}

\begin{figure}[htp!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures_supp/intersection.pdf}
    \caption{Visualization of the intersection points between distance histograms from detections to inactive tracks of the same and different identities when using domain adaptation (DA) compared to when not using it.}
    \label{fig:intersection_2}
\vspace{-0.6cm}
\end{figure}

\noindent\textbf{Visibility.} Motion cues perform better especially in the static sequences MOT17-02 and MOT17-04. In the static sequence MOT17-09, which is recorded from a low viewpoint, and the moving sequences MOT17-05, MOT17-10, and MOT17-11, motion and appearance perform approximately on par. 
%
In MOT17-13, which shows heavy camera movements, the performance of the motion model drops significantly.
%
Those observations show that for suitable camera angles in static sequences motion outperforms appearance independent of the visibility, while for sequences with severe camera movement or unsuitable camera angles, appearance outperforms motion even for low visibility scenarios.
%
For moving camera sequences, the motion of the object and the camera add up, resulting in more noisy and non-linear motion observed in pixel space, even though the underlying motion might be linear. 
%
Similarly, a low viewpoint leads to a distorted observation of the underlying motion from the camera perspective. %\lau{I do not understand the previous sentence: unsuitable and distracted seem weird word choices.}
%
When the camera angle comes closer to a bird's eye view perspective (MOT17-04) the observed motion is less distorted.


\noindent\textbf{Occlusion time.} Fig~\ref{fig:seq_analysis_occ} shows that all moving sequences show a higher RCA for appearance than motion cues. For static sequences, motion performs slightly better in MOT17-02 and MOT17-04. In the static sequence MOT17-09, the sequence recorded from a low viewpoint, both perform approximately on par. 
%
For suitable camera angles motion is a good cue even for long-term associations in static sequences, while appearance outperforms motion even for short-term associations in moving ones. This stems from the fact that motion gets more non-linear observed from camera perspective in moving camera sequences. While appearance still suffers from occlusion in static sequences even when recorded from a well-suited camera angle, those conditions allow for surprisingly well performance of motion even with respect to long-term associations.
%

\section{A Deeper Analysis on on-the-fly Domain Adaptation}
\label{sec:inter}
In the main paper, we visualize the distance histograms between active and inactive tracks to new detections of the same or different classes (see Fig 2 main paper). In this section, we show that the \textit{intersection point} that divides the distance histograms between active (inactive) tracks of the same and different classes well varies less over the different sequences when using our on-the-fly domain adaptation (see Fig 2(b) in main paper) compared to when not using it (see Fig 2(a) in main paper). Furthermore, we show that the distributions are generally more \textit{similar and stable} over different sequences with out on-ht-fly domain adaptation.


% definition intersection points
\noindent\textbf{Intersection Points.} Given the distribution $f_{a,d}$ of distances between active tracks ($a$) and new detections of a different ID ($d$) and the distribution $f_{a,s}$ of distances between active tracks and new detections of the same ID ($s$), we find a well suited intersection point ${x_{s,d}^a}^*$ separating both distributions by minimizing the sum of the costs of false positive and false negative matches.
% Definition of computation
Towards this end, for a given point $x_{s,d}^a$ we define the false positive costs as percentile value of $f_{a,d}$ at $x_{s,d}^a$ given by $p_{a,d}^{x_{s,d}}$, \textit{i.e.}, the percentile of $f_{a,d}$ that lies left to $x_{s,d}^a$. We define the false negative cost for $x_{s,d}^a$ as $100-p_{a,s}^{x_{s,d}}$ utilizing the percentile value of $f_{a,s}$ at $x_{s,d}^a$ since we want to punish the false negatives that lie to the right of this point.
%
% Use it
Similar points $x_{s, d}^{a}$ across sequences allow to choose one single well-suited threshold $\tau_{act}$ over all sequences. The same holds for the inactive track distributions $f_{i,s}$ and $f_{i,d}$ and the corresponding $x_{s, d}^{i}$ of the different sequences. As we visualize in Fig~\ref{fig:intersection_2}, $x_{s, d}^{i}$ varies significantly less across tracking sequences when using our on-the-fly DA compared to when not using it. 

\noindent\textbf{Similarity and Stability.} 
%
While the variance of $x_{s, d}^{a}$ is higher for both settings, \textit{i.e.}, with and without the on-the-fly DA, the distributions are generally more separated when using DA compared to when not using it. To show this, we conduct a second experiment. 
%
For each sequence, we define the same bins in the range from $0-1$ and turn the distributions $f_{a,d}$ and $f_{a,s}$ into histograms $h_{a,d}$ and $h_{a,s}$. In each bin $i$ we compute the absolute difference between the two histograms $d_{a, i}$ and normalize it by the sum of all absolute distances. Finally, we plot the cumulative histogram (see Fig~\ref{fig:quantilles_act}). The more aligned the cumulative histograms over all sequences and the broader the saddle point, the more similar the sequences across each other and the better separated the distributions of the same and different IDs, respectively. Note, that the cumulative sums of the different sequences are much more aligned when utilizing on-the-fly domain adaptation (see Fig~\ref{fig:quantilles_act_with}) than when not using it (see Fig~\ref{fig:quantilles_act_without}) which makes it easier to find a common threshold $\tau_{act}$.  Moreover, the saddle point is much broader when using on-the-fly domain adaptation which makes our approach more stable with respect to different thresholds $\tau_{act}$.

Despite the difference visualization for the inactive track distributions being less unified over the sequences in general, the differences over the different sequences when using on-the-fly domain adaptation are more aligned compared to when not using it (see Fig~\ref{fig:quantilles_inact}). Combined with the less varying ${x_{s, d}^{i}}^*$, this leads not only to an overall better suited but also more stable threshold $\tau_{inact}$. 

\section{Using the Knowledge of our Analysis.}
\label{sec:knowledge}
In our work we present an in-depth analysis on appearance distance computation based on embedding features (see Fig 2 in the main paper) as well as motion vs. appearance model performance (see Fig 3-6 in the main paper). Based on those insights we introduce our simple tracker GHOST. For example, we utilize the analysis of the differences between the reID distance of active and inactive tracks to detections to adapt the thresholds and and choose a proxy distance computation method. Also, we utilize the inisghts that reID performs worse for high occlusion levels and linear motion performs worse in moving camera scenes and with extreme motion to adapt the motion weight as well as the number of frames used in the motion model. We do not only present GHOST but also a large number of analysis that reveal insights for the community. 
%
% Practical uses of our analysis insights in GHOST include the following: 
% \begin{itemize}
%     \item Fig 2 main paper: difference between reID distance active and inactive tracks $\rightarrow$ adapting thresholds accordingly (see Sec 3.2 main paper)
%     \item Fig 4-6 main paper: reID bad for high occlusion, linear motion bad for moving camera (same holds for extreme motion as in DanceTrack) $\rightarrow$ adaption of motion weight and of \# frames motion model (see Tab~\ref{tab:reb2}).
% \end{itemize}
In the following we provide a deeper analysis on the hyperparameters and design choices of GHOST for the single datasets.


\begin{table*}
\centering
\resizebox{0.65\textwidth}{!}{
\begin{tabular}{@{}l|cccc@{}}
\hline
& BDD & DanceTrack & MOT17 & MOT20\\
\hline
motion & moving cam & extreme motion & partially moving cam & static cam \\
occlusion & medium & medium & medium & high \\
motion weight & 0.4 & 0.4 & 0.6 & 0.8 \\
\# frames motion model & 10 & 5 & 90 & 30 \\
\hline
\end{tabular}}
\vspace{-0.2cm}
\caption{Motion Model Parameters.}
\vspace{-0.4cm}
\label{tab:reb2}
\end{table*}


\vspace{-0.1cm}
\subsection{The Usage of Different Proxies}
\vspace{-0.1cm}
\label{sec:proxies}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/proxies_HOTA.pdf}
        \vspace{-0.6cm}
        \caption{HOTA}
        %\caption{Drop in Performance in HOTA Metric}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/proxies_IDF1.pdf}
        \vspace{-0.6cm}
        \caption{IDF1}
        %\caption{MOT17-04 \textit{S}}
    \end{subfigure}
    \vspace{-0.3cm}
\caption{Drop in Performance for Different Proxies on Different Datasets. M17Pr = MOT17 private detections, M17Pu = MOT17 public detections, M20 = MOT20 public detections, DT = DanceTrack, BDD = BDD100k. Mean = Mean Feature, Mode = Mode Features, Median = Median Features, Mv Av = Moving Average of Features, Last = Last Features, Ours = Our Proxy Distance.}
    \label{fig:proxies}
\vspace{-0.5cm}
\end{figure*}

We now explore different proxies for the distance computation between new detections and inactive tracks. We start from the feature vectors generated using our reID network and normalize them before further processing. As introduced in the main paper, we utilize the mean of the distances of a new detection to all detections of an inactive track. This proxy distance between new detection $i$ and inactive track $k$ is given by:

\vspace{-0.2cm}
\begin{equation}
\begin{split}
    \Tilde{d}(i, k) & = \frac{1}{N_k} \sum_{n=1}^{N_k} d(f_i,f_k^n) \\
    & = \frac{1}{N_k} \sum_{n=1}^{N_k} 1-\frac{f_i \cdot f_k^n}{||f_i||\cdot||f_k^n||} \\
    & = 1-\frac{1}{N_k} \sum_{n=1}^{N_k} f_i \cdot f_k^n
\end{split}
\end{equation}
where $N_k$ is the number of detections in the inactive track and $f_{k}^n$ is the feature vector corresponding to its $n$-th detection. We omit $||f_i||\cdot||f_k^n||$ as we normalize all feature vectors.

Another option is to first compute a proxy feature vector and then compute the distance between a new detection and the proxy feature vector. We investigate four proxy feature vector computations and compare them on the validation set of all four datasets.

\noindent\textbf{Mean Feature Vector.} The mean feature vector of all detections in the inactive track $k$ which is also used in Tracktor \cite{DBLP:conf/iccv/BergmannML19} is given by
\begin{equation}
    \Tilde{f}_k = \frac{1}{N_k} \sum_{n=0}^{N_k} f_{k}^n
\end{equation}
Computing the cosine distance of this mean feature vector leads to 
\begin{equation}
\begin{split}
    \Tilde{d}(i, k) & = 1- \frac{f_i \cdot \frac{1}{N_k} \sum_{n=1}^{N_k} f_k^n}{||f_i||\cdot||\frac{1}{N_k} \sum_{n=1}^{N_k} f_k^n||} \\
    & = 1- \frac{\sum_{n=1}^{N_k} f_i \cdot f_k^n}{||\sum_{n=1}^{N_k} f_k^n||}
\end{split}
\end{equation}
This differs from our proxy distance by the normalization constant $\frac{1}{||\sum_{n=1}^{N_k} f_k^n||}$.

\noindent\textbf{Mode Feature Vector.} Compared to the mean feature vector, the feature vector of inactive track $k$ is given by the value that appeared most in each feature dimension.

\noindent\textbf{Median Feature Vector.} Viewing $f_k^n$ as a random variable, in each dimension the median feature vector contains the value for which $50\%$ of the probability mass of feature values in this dimension lies on the right and left of it, \ie, it divides the probability mass into two equal masses. 

\noindent\textbf{Exponential Moving Average Feature Vector.} Utilizing the exponential moving average (EMA) as feature vector as done in JDE \cite{DBLP:conf/nips/RenHGS15} or FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} means that at given a new detection, the feature vector is updated by:

\begin{equation}
    \Tilde{f}_k^t = \Tilde{f}_k^{t-1} * \alpha + f_k^t * (1-\alpha)
\end{equation}
where $\Tilde{f}_k^{t-1}$ is the EMA feature vector at the previous time step, $f_k^t$ is the feature vector of the new detection, and $\alpha=0.9$ is a weighting factor. The EMA feature vectors build on the underlying assumption that feature vectors should change only slightly and, therefore, smooths the feature vector development.

We show the performance drop on different datasets when using different proxies in Fig~\ref{fig:proxies}. Ours, \textit{i.e.}, the mean distance shows the most stable performance over the different datasets and we, therefore, decided to utilize this proxy.

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/motion_weight_HOTA.pdf}
        %\caption{Drop in Performance in HOTA Metric}
        \vspace{-0.6cm}
        \caption{HOTA}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/motion_weight_IDF1.pdf}
        %\caption{MOT17-04 \textit{S}}
        \vspace{-0.6cm}
        \caption{IDF1}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Drop in Performance for Different Motion Weights on Different Datasets. M17Pr = MOT17 private detections, M17Pu = MOT17 public detections, M20 = MOT20 public detections, DT = DanceTrack, BDD = BDD100k.}
    \vspace{-0.3cm}
    \label{fig:weights}
\end{figure*}


\subsection{The Impact of Motion Weights}
\label{sec:weights}

In this subsection, we visualize the performance drop when utilizing different motion weights on different datasets (see Fig~\ref{fig:weights}). On MOT17 public detections, the best performance is achieved when using motion weight 0.4 while for private detections the best weight is 0.6. This is caused by the fact, that the appearance model gets less certain with increasing occlusion level and the private detections set contains more difficult, \textit{i.e.}, occluded detections. 
%
On MOT20 private detections a motion weight of 0.8 for private detections performs best as the occlusion level is generally much higher than on MOT17 dataset. 
%
On DanceTrack dataset, the best motion weight is 0.4. Since the motion and articulation on this dataset are generally more diverse and extreme, the performance of the motion model is less certain compared to the appearance model. 
%
BDD dataset solely contains sequences recorded using a moving camera. As we showed in the main paper, the performance of the motion distance decreases when moving cameras are used. This is due to the fact, that the observed motion gets less linear since the motion of the camera and the object add up. Consequently, a motion weight of 0.4 works best on BDD100k MOT dataset.
%
All those observations are in line with our analysis in the main paper as well as the more detailed analysis in this supplementary in Section~\ref{sec:detailed_rca}.


\subsection{The Impact of Different Numbers of Frames for Velocity Computation}
\label{sec:num_frames}

The less linear the motion or the observed motion, the fewer frames approximate the future motion better. We visualize the impact of different numbers of frames in Fig~\ref{fig:num_frames}.
%
While on MOT17 private detections, the linear motion model performs well using the positions of the last 90 tracks (or less if a track contains less), on MOT20 using only the last 30 frames performs best since the scenes are highly crowded and, therefore, the motion is less linear.
%
On DanceTrack, the motion is more extreme and, therefore, using only the last 5 frames approximates the future motion best. 
%
Similarly, on BDD100k as the observed motion is more non-linear due to the combination of the camera motion and the object motion utilizing only the last 10 frames to approximate the motion performs best. The lower frame rate of BDD sequences compared to the frame rate of MOT17, MOT20 and DanceTrack even increases this effect, since more time passes within the same number of frames on BDD.
%
Overall, as already stated in the main paper, short-term future motion can be approximated fairly well utilizing a linear motion model. Depending on the characteristics of the motion, a different number of frames approximates the future motion best and, therefore, leads to the best tracking results.

\subsection{How to use Different Thresholds $\tau_{i}$}
\label{sec:threshs}
As stated in Subsection 3.2. in the main paper, we utilize different thresholds for active and inactive tracks. While commonly only one threshold is used, we empirically find that it is beneficial to allow different ones. Therefore, we apply the thresholds \textit{after} the bipartite matching to filter the detection-trajectory pairs ($i, j$). We visualize our matching in Algorithm~\ref{alg:matching}. $n$ represents the number of active track, $\tau_{act}$ and $\tau_{inact}$ the threshold for active and inactive tracks and $d$ the cost matrix.

\section{Different Inactive Patience Values}
\label{sec:memory}
Similar to other approaches~\cite{DBLP:conf/iccv/BergmannML19,DBLP:conf/cvpr/StadlerB21,DBLP:journals/ijcv/ZhangWWZL21,DBLP:conf/nips/RenHGS15,DBLP:conf/ijcai/LiuC0Y20} that only keep inactive tracks for a fixed number of frames, called inactive patience, we keep them for 50 frames for all datasets. To show that this choice is reasonable, we visualize HOTA, IDF1, and MOTA on MOT17 validation set for different inactive patience values in Fig~\ref{fig:mem}. We use the same setting as in sections 4.4 and 4.5 in the main paper, \textit{i.e.}, we use the bounding boxes of MOT17 validation set of several private trackers. The performance drops heavily for inactive patience 0 and then only slightly changes up to using all frames of a sequence after 30 frames.


\RestyleAlgo{ruled}
\begin{algorithm}
\caption{Assignment with different thresholds}\label{alg:matching}
\KwData{$n, \tau_{act}, \tau_{inact}, \text{cost matrix } d\in\mathcal{R}^{|T|\times|D|}$\;}
\KwResult{approved rows, approved cols\;}
$\text{approved rows} = \emptyset$, $\text{approved cols} = \emptyset$\;
$\text{matched rows}, \text{matched cols} = \text{Bipartite}(c)$\;
\For{$r, c \text{ in } \text{zip}(\text{matched rows}, \text{matched cols})$}{
     \uIf{$r < n \text{ and } d_{r, c} < \tau_{act}$}{
        $\text{approved rows} = \text{approved rows}  + r$\;
        $\text{approved cols} = \text{approved cols}  + c$\;}
     \uElseIf{$r >= n \text{ and } d_{r, c} < \tau_{inact}$}{
        $\text{approved rows} = \text{approved rows}  + r$\;
        $\text{approved cols} = \text{approved cols}  + c$\;}
     \Else{
        \text{Discard Match.}\;}
     }
\end{algorithm}


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/num_frames_HOTA.pdf}
        \vspace{-0.6cm}
        \caption{HOTA}
        %\caption{Drop in Performance in HOTA Metric}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/num_frames_IDF1.pdf}
        \vspace{-0.6cm}
        \caption{IDF1}
        %\caption{MOT17-04 \textit{S}}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Drop in Performance for Different Number of Frames for Velocity Computation on Different Datasets. M17Pr = MOT17 private detections, M17Pu = MOT17 public detections, M20 = MOT20 public detections, DT = DanceTrack, BDD = BDD100k.}
    \label{fig:num_frames}
    \vspace{-0.1cm}
\end{figure*}

\begin{figure*}[htp!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[height=3.5cm]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/memory_hota.pdf}
        \caption{HOTA}
    \end{subfigure}
    \begin{subfigure}[b]{0.29\textwidth}   
        \centering 
        \includegraphics[height=3.5cm]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/memory_idf1.pdf}
        \caption{IDF1}
    \end{subfigure}
    \begin{subfigure}[b]{0.39\textwidth}   
        \centering 
        \includegraphics[height=3.5cm]{cvpr2023-author_kit-v1_1-1/latex/figures_supp/memory_mota.pdf}
        \caption{MOTA}
    \end{subfigure}
     \vspace{-0.1cm}
    \caption{Performance on MOT17 public validateion set with respect to different inactive patience values.}
    \label{fig:mem}
   \vspace{-0.5cm}
\end{figure*} 

\section{Computation of Distance Histograms}
\label{sec:distance_dist}
In the main paper, we visualize distributions of distances from active and inactive tracks to detections of the same and different classes in Fig 2. In Fig 2(a) we utilize the embeddings of the last detection of any existing track to compute the distance to the embeddings of new detections, in Fig 2(b) we utilize the distance computation as introduced in Sec 3.2, and in 2(c) we visualize the motion distance. Since different distance metrics could be applied for feature vector distance and motion distance, we define both in Sec 4.1.
%
To generate those distributions, we first match given detections to ground truth identities following the same matching as used for the computation of the MOTA metric \cite{DBLP:journals/pami/KasturiGSMGBBKZ09}. %Given a detection of ID $i$. 
%
If a detection of the same ID occurred in the last frame, we compute the distance to it and add it to the distances between active tracks and detections of the same ID. 
%
Similarly, if there was a detection present but not in the last frame, we compute the distance and add it to the distances from inactive tracks to detections of the same ID. 
%
Afterwards, we compute the distances to all other IDs that occurred in the last frame as well as to all other IDs that occurred prior to the last frame and add them to the distances from detections to active and inactive tracks of a different ID, respectively.
%
We can add inactive patience and proxy computation methods to this basic framework. Despite we only show the distributions for MOT17 validation set, this method can be used for any dataset for which ground truth detections are available.

\section{On Similar Approaches}
\label{sec:similar}
In this section, we discuss the differences between state-of-the-art trackers that share some of their components with GHOST.
%
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} uses a Kalman Filter as motion model while we use a more simple linear motion model. More importantly, the authors treat active and inactive \textbf{tracks} the same but distinguish between high and low confidence \textbf{detections}, \textit{i.e.}, they differentiate on a detection level while we differentiate on track level. However, as we showed in the main paper, active and inactive tracks show significant differences and treating them the same way does not leverage the full potential of the underlying cues. Also, their assignment strategy leads to a multi-level association process while GHOST only requires a single association step.
%
Similarly, in \cite{DBLP:conf/cvpr/BaeY14} the authors treat \textbf{high and low confidence tracks} differently, \textit{i.e.}, high confidence tracks are assigned locally to new detections and low confidence tracks are globally assigned with other tracks and detections. The inactivity of a track is only one factor of confidence. Note that this again involves multiple bipartite matchings while we assign active and inactive tracks \textbf{at the same time} which only requires one.
%
The authors of DeepSORT \cite{DBLP:conf/icip/WojkeBP17} utilize a Kalman filter as well as an appearance model. However, the parameter that weights appearance and motion is set to $\lambda=0$, \textit{i.e.}, only appearance is considered. However, as we show in our analysis motion can compensate for failure cases of appearance, especially in low visibility regimes making our approach more robust.
%By this, the authors do not leverage the full potential of the simple cues while the combination of both leads bears significant potential. \lau{What does the previous sentence mean?} 
%\jenny{check}
Moreover, the authors propose a cascaded matching strategy that requires more than one bipartite matching per frame while we, again, only require one.
%
With respect to domain adaptation, HCC \cite{DBLP:conf/accv/MaTBG18} trains on tracking sequences and uses sophisticated test-time mining to fine-tune. We rely on a simpler scheme and do not need any of the above.

Despite all of the above-mentioned approaches showing similarities to our approach, they still differ with respect to significant design choices positioning our approach as a complementary work with respect to them. Furthermore, our approach leverages the motion and appearance cues in a simple yet highly effective and general way without multi-level association procedures. %\jenny{Better? :)}

\section{On the Generality of ByteTrack \cite{DBLP:journals/corr/abs-2110-06864}}
\label{sec:generality}
Recently, ByteTrack \cite{DBLP:journals/corr/abs-2110-06864}, which also follows the tracking-by-detection paradigm, also reported results on MOT17 and MOT20 as well as on the highly different datasets DanceTrack and BDD100k MOT. In this section, we compare GHOST to ByteTrack with respect to generality. Despite not being mentioned in the paper, the authors add tricks to the tracking procedure which are different for each dataset.
%
%Recently, several approaches reported results on MOT17 and MOT20 as well as on the highly different datasets DanceTrack and BDD100k MOT. In this section, we especially compare our approach to ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} since it also follows the tracking-by-detection paradigm. Despite not being mentioned in the paper, the authors add tricks to the tracking procedure on the different datasets.
%
\textbf{First}, they multiply their IoU cost matrix, which they obtain by using a Kalman Filter, by the detection confidence when applying their tracker to MOT17, but not when applying it to other datasets. 
\textbf{Second}, the authors apply interpolation on MOT17 and MOT20 datasets which turns their approach into an offline approach. 
\textbf{Third}, on DanceTrack and BDD100k, they allow all bounding boxes to be used, while they filter out bounding boxes if $\frac{w}{h} > 1.6$ on MOT17 and MOT20, where $w$ and $h$ are bounding box width and height, respectively. 
\textbf{Fourth}, ByteTrack uses a reID model, namely UniTrack \cite{DBLP:conf/nips/WangZLWTB21}, on BDD100k dataset whilst they do not use any reID model on the other datasets. 
\textbf{Fifth}, they adapt the tracking thresholds \textit{per sequence} on MOT17 and MOT20 during training \textit{and testing}. On BDD and DanceTrack the tracking thresholds are applied per dataset.
\textbf{Sixth}, as commonly done the authors adapt other model parameters, \textit{e.g.}, the matching thresholds, confidence threshold for detections as well as the confidence threshold for new tracks.
% they fuse conv and bn for testing

We believe these are small but significant changes that put into question the generality of ByteTrack. 
%
In contrast, we keep our tracking pipeline the same over different datasets but solely change our model parameters for each dataset as a \textbf{whole}. To be specific, we adapt the thresholds $\tau_i$, the detection confidence thresholds to filter plain detections and start new tracks, the motion weights, as well as the number of frames used in the linear motion model. %\lau{Ok this still sounds like a lot. Is this something bytetrack also does? adapt their parameters? make sure we write we dont do this for every sequence, just for every dataset as a WHOLE.} 
This makes our approach more general and easier to apply to new datasets. %\jenny{Better? :)}

\section{Latency}
\label{sec:latency}
For a fair comparison with other methods, we evaluated GHOST, Tracktor \cite{DBLP:conf/iccv/BergmannML19}, and FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} on the public detections on the MOT17 validation set utilizing the same GPU, namely a Quadra P6000. Note that we utilize CenterTrack pre-processed detections here.
%
With 10FPS GHOST is on the same magnitude of speed as current SOTA trackers. While Tracktor \cite{DBLP:conf/iccv/BergmannML19} runs at 2FPS, FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} runs at 17FPS as it was optimized for real-time. 
%
When evaluating the private detection setting, our method's latency increases slightly due to the increase of bounding boxes to process to 6FPS.
%
The average latency per frame and per model part is given by 10ms for the computation of the reID features, 30ms for the reID distance computation, 0.1 ms for updating the velocity per track, 0.0025ms for the motion step per track, 0.4ms for the motion distance computation, 0.35ms for the biparite matching, and 0.1ms for updating all tracks.

\section{Visualizations}
\label{sec:vis}
In this section, we visualize associations on CenterTrack re-fined public bounding boxes that our model is able to correctly associate while CenterTrack is not. Correct and wrong associations are determined in the same way as done for the computation of the RCA Section~\ref{sec:detailed_rca}. This means we determine wrong associations by first matching all detection bounding boxes to the ground truth IDs. A wrong association is given if the prior detection of the same ground truth ID as a current detection was assigned to a different tracker ID than the current detection. In Figures \textcolor{red}{10}-\textcolor{red}{17}, we visualize the prior detection on the left side and the current detection on the right side. All examples were associated wrongly by CenterTrack and correctly by GHOST.
%
We give the time distance between the prior and the current frame in the caption as well as the visibility level of the re-appearing pedestrian. 
%
By our combination of appearance and motion, we are able to correctly associate pedestrians after long occlusions and low visibility in highly varying sequences. 


% MOT17 02
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_329_389_35_prev.jpg}
        
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_329_389_35.jpg}
        
    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_329_389_35_prev.jpg}
        
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_329_389_35.jpg}
    
    \end{subfigure}
    \caption{Occlusion time: $2s$, visibility of re-appearing pedestrian: $0.6$.}
    \label{fig:mot17_2_1}
\end{figure*}

\iffalse
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_379_431_23_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_379_431_23.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_379_431_23_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_379_431_23.jpg}

    \end{subfigure}
    \caption{Occlusion time: 1.7s, visibility of re-appearing pedestrian: 0.3.}
    \label{fig:mot17_2_2}
\end{figure*}
\fi

% MOT17 04
\begin{figure*}
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_651_684_78_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_651_684_78.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_651_684_78_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_651_684_78.jpg}

    \end{subfigure}
    \caption{Occlusion time: 1.1s, visibility of re-appearing pedestrian: 0.3.}
    \label{fig:mot17_4_1}
\end{figure*}
\iffalse
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_650_668_38_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_650_668_38.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_650_668_38_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_650_668_38.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.6 s, visibility of re-appearing pedestrian: 0.3.}
    \label{fig:mot17_4_2}
\end{figure*}
\fi
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_732_1013_38_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_732_1013_38.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_732_1013_38_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_732_1013_38.jpg}

    \end{subfigure}
    \caption{Occlusion time: 9.4s, visibility of re-appearing pedestrian: 0.4.}
    \label{fig:mot17_4_2}
\end{figure*}


% MOT17 05
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_502_518_120_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_502_518_120.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_502_518_120_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_502_518_120.jpg}

    \end{subfigure}
    \caption{Occlusion time: 1.1s, visibility of re-appearing pedestrian: 0.5.}
    \label{fig:mot17_5_1}
\end{figure*}

\iffalse
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_514_528_51_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_514_528_51.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_514_528_51_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_514_528_51.jpg}

    \end{subfigure}
    \caption{Occlusion time: 1s, visibility of re-appearing pedestrian: 0.4.}
    \label{fig:mot17_5_2}
\end{figure*}
\fi

\newpage
\iffalse
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_598_611_121_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_598_611_121.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_598_611_121_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_598_611_121.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.9s, visibility of re-appearing pedestrian: 0.2.}
    \label{fig:mot17_5_3}
\end{figure*}
\fi
\iffalse
\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_745_756_84_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_745_756_84.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_745_756_84_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_745_756_84.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.8s, visibility of re-appearing pedestrian: visibility 0.5}
    \label{fig:mot17_5_4}
\end{figure*}
\fi

%MOT17-09

\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_342_374_10_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_342_374_10.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_342_374_10_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_342_374_10.jpg}

    \end{subfigure}
    \caption{Occlusion time: 1.1s, visibility of re-appearing pedestrian: 0.2.}
    \label{fig:mot17_9_1}
\end{figure*}

%MOT17-10

\begin{figure*}[t]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_630_632_62_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_630_632_62.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_630_632_62_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_630_632_62.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.1s, visibility of re-appearing pedestrian: 0.6.}
    \label{fig:mot17_10_1}
\end{figure*}

%MOT17-11

\begin{figure*}[t!]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_694_721_20_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_694_721_20.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_694_721_20_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_694_721_20.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.9s, visibility of re-appearing pedestrian: 0.5.}
    \label{fig:mot17_11_1}
\end{figure*}

%MOT17-13
\begin{figure*}[t!]
    \centering
    \iffalse
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_444_448_58_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ct/center_track_O_errors_clear_444_448_58.jpg}

    \end{subfigure}
    \fi
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_444_448_58_prev.jpg}

    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{vis_ours/center_track_Ours_errors_clear_444_448_58.jpg}

    \end{subfigure}
    \caption{Occlusion time: 0.2s, visibility of re-appearing pedestrian: 0.8.}
    \label{fig:mot17_13_1}
\end{figure*}



\clearpage

==> cvpr2023-author_kit-v1_1-1/latex/tables/ablation_last_n_motion.tex <==
\begin{table}[t!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}l|ccc@{}}
\hline

& \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ & \textbf{IDF1} $\uparrow$ \\
\hline
\hline

last 10000000 & 77.3 & 88.7 & 93.9 \\
last 10 frames & 77.6 & 89.3 & 94.0 \\
last 30 frames & 78.0 & 89.8 & 94.0 \\
last 60 frames & 77.7 & 89.4 & 94.0 \\
last 90 frames & 77.8 & 89.5 & 93.9 \\
last 120 frames & 77.7 & 89.4 & 93.9 \\
last 150 frames & 77.7 & 89.3 & 93.9 \\

\hline
\end{tabular}}
\caption{Ablation of using different number of frames for velocity computation on MOT20.}
\label{tab:last_n_frames_ablation}
\end{table}


==> cvpr2023-author_kit-v1_1-1/latex/tables/ablations.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}l|c|cc|cc|cc|cc|cc|cc|cc@{}}
\hline
& & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Basic ReID} & \multicolumn{2}{c}{Our ReID} & \multicolumn{2}{c}{Kalman} &\multicolumn{2}{c}{Linear Motion} & \multicolumn{2}{c}{Sum} & \multicolumn{2}{c}{Ours} \\

\hline
&Occ Det & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1\\
\hline
JDE & 0.20 & 59.9 & 64.1 & 60.1 & 62.1 & 60.0 & 63.9 & 59.9 & 64.9 & 60.1 & 65.9 & 60.3 & 67.1 & 60.4 & 66.8 \\
FairMOT & 0.27 & 69.1 & 72.8 & 69.2 & 67.0 & 69.2 & 68.5 & 69.2 & 73.8 & 69.3 & 73.0 & 69.5 & 73.2 & 69.5 & 74.1 \\
TransTrack & 0.17 & 67.7 & 68.6 & 67.6 & 67.6 & 67.7 & 69.5 & 67.4 & 71.4 &  67.7 & 71.1 & 68.0 & 73.7 & 67.9 & 72.7 \\
QDTrack & 0.24 & 67.2 & 67.8 & 67.3 & 64.8 & 67.3 & 68.2 & 67.0 & 70.1  & 67.3 & 71.0 & 67.5 & 71.2 & 67.5 & 72.8 \\
TraDeS & 0.18 & 68.5 & 71.9 & 68.6 & 72.0 & 68.7 & 71.9 & 68.5 & 72.8 & 68.4 & 72.9 & 68.8 & 74.9 & 68.8 & 75.5 \\
CSTrack & 0.25 & 68.2 & 72.3 & 68.3 & 66.5 & 68.2 & 68.2 & 68.3 & 72.0 & 68.3 & 72.8 & 68.4 & 73.4 & 68.5 & 72.8 \\
CenterTrack & 0.18 & 66.7 & 64.5 & 67.5 & 67.6 & 67.4 & 72.7 & 67.3 & 72.7 & 67.3 & 72.7 & 67.5 & 74.6 & 67.5 & 74.6 \\
\hline
\end{tabular}}


\caption{Analysis of the contribution of ReID and motion cues. Occ Det = average occlusion level of detected bounding boxes.}
\label{tab:ablations}
\vspace{-0.7cm}
\end{table}

==> cvpr2023-author_kit-v1_1-1/latex/tables/bdd_short.tex <==
\begin{table}[t!]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}

\toprule

 &  \textbf{mHOTA} $\uparrow$  &  \textbf{mIDF1} $\uparrow$ & \textbf{mMOTA} $\uparrow$  &  \textbf{HOTA} $\uparrow$ &  \textbf{IDF1} $\uparrow$  &  \textbf{MOTA} $\uparrow$ \\
\hline\hline

\textit{validation} \\

Yu et. al. \cite{DBLP:conf/cvpr/YuCWXCLMD20} & - & 44.5 & 25.9 & - & 66.8 & 56.9 \\ 
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & \textcolor{red}{45.4} & \textcolor{red}{54.6} & \textbf{45.2} & \textcolor{red}{61.6} & \textcolor{blue}{70.2} & \textbf{68.7} \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & \textcolor{blue}{41.7} & 51.5 & 36.3 & \textcolor{blue}{60.9} & \textbf{71.4} & \textcolor{blue}{63.7} \\
% Unicorn \cite{DBLP:conf/eccv/YanJSWYLL22} & - & \textcolor{blue}{54.0} & \textcolor{blue}{41.2} & - & 71.3 & \textcolor{blue}{66.6} \\
MOTR \cite{DBLP:journals/corr/abs-2105-03247} & - & 43.5 & 32.0 & - & - & - \\
TETer \cite{DBLP:conf/eccv/LiDDHY22} & - & \textcolor{blue}{53.3} & \textcolor{blue}{39.1} & - & - & - \\

\hline

GHOST  & \textbf{45.7} & \textbf{55.6} & \textcolor{red}{44.9} &\textbf{61.7} & \textcolor{red}{70.9} & \textcolor{red}{68.1} \\
\hline
\hline
\textit{test} \\

Yu et. al. \cite{DBLP:conf/cvpr/YuCWXCLMD20} & - & 44.7 & 26.3 & - & 68.2 & 58.3 \\ 
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & - & \textcolor{red}{55.8} & \textbf{40.1} & - & \textcolor{blue}{71.3} & \textbf{69.6} \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & - & \textcolor{blue}{52.3} & \textcolor{blue}{35.5} & - & \textbf{72.3} & \textcolor{blue}{64.3} \\

\hline

GHOST  & \textbf{46.8} & \textbf{57.0} & \textcolor{red}{39.5} &\textbf{62.2} & \textcolor{red}{72.0} & \textcolor{red}{68.9} \\

\bottomrule

\end{tabular}}
\vspace{-0.25cm}
\caption{Comparison to state-of-the-art on BDD100k.}
\vspace{-0.65cm}
\label{tab:bdd_short}
\end{table}

\iffalse
\begin{table}[t!]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{}l|cccccc@{}}
\toprule

 &  \textbf{mHOTA} $\uparrow$  &  \textbf{mMOTA} $\uparrow$ & \textbf{mIDF1} $\uparrow$  &  \textbf{HOTA} $\uparrow$ &  \textbf{IDF1} $\uparrow$  &  \textbf{MOTA} $\uparrow$ \\
\hline\hline
Yu et. al. \cite{DBLP:conf/cvpr/YuCWXCLMD20} & - & 44.7 & 26.3 & - & 68.2 & 58.3 \\ 
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & - & \textcolor{red}{55.8} & \textbf{40.1} & - & \textcolor{blue}{71.3} & \textbf{69.6} \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & - & \textcolor{blue}{52.3} & \textcolor{blue}{35.5} & - & \textbf{72.3} & \textcolor{blue}{64.3} \\

\hline

Ours  & \textbf{46.6} & \textbf{56.8} & \textcolor{red}{39.7} &\textbf{62.0} & \textcolor{red}{71.6} & \textcolor{red}{68.4} \\



\bottomrule

\end{tabular}}
\vspace{-0.2cm}
\caption{BDD test set performance.}
\vspace{-0.2cm}
\label{tab:bdd_short_test}
\end{table}
\fi

==> cvpr2023-author_kit-v1_1-1/latex/tables/da_ablation.tex <==
\begin{table}[t!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}l|ccc@{}}
\hline

& \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ & \textbf{IDF1} $\uparrow$ \\
\hline
\hline

BN update random patches  & 59.1 & 68.6 & 68.4 \\
BN update 10 frames before  & 62.0 & 73.0 & 68.6 \\
BN update whole sequence first & 62.4 & 73.8 & 69.1 \\
fine tuning on MOT17 & 63.0 & 74.3 & 69.6 \\
ResNet50 IBN & 63.2 & 74.6 & 69.7 \\
\hline
our domain adaptation & 63.2 & 75.4 & 69.7  \\
\hline
\end{tabular}}
\vspace{-0.1cm}
\caption{Ablation of different domain adaptation approaches.}
\vspace{-0.5cm}
\label{tab:domain_adaptation_ablation}
\end{table}

==> cvpr2023-author_kit-v1_1-1/latex/tables/dancetrack.tex <==
\begin{table}[t!]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule

& \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ &  \textbf{MOTA} $\uparrow$  & \textbf{DetA} $\uparrow$ & \textbf{AssA} $\uparrow$\\
\hline
\hline
CenterTrack \cite{DBLP:conf/eccv/ZhouKK20} & 41.8 & 35.7  & 86.8 & \textcolor{blue}{78.1} & 22.6\\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & 39.7 & 40.8 & 82.2 & 66.7 & 23.8 \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & \textcolor{red}{54.2} & 50.4  & \textcolor{blue}{87.7} & \textcolor{red}{80.1} & \textcolor{blue}{36.8}\\
% TransTrack & 45.5 & 45.2  & 88.4 & 75.9 & 27.5 \\
TraDeS \cite{DBLP:conf/cvpr/WuCS00Y21} & 43.3 & 41.2 & 86.2 & 74.5 & 25.4 \\
MOTR \cite{DBLP:journals/corr/abs-2105-03247} & \textcolor{red}{54.2} & \textcolor{blue}{51.5} & 79.7 & 73.5 & \textbf{40.2} \\
GTR \cite{DBLP:conf/cvpr/ZhouYKK22} & \textcolor{blue}{48.0} & 50.3 & 84.7 & 72.5 & 31.9 \\
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & 47.7  & \textcolor{red}{53.9} & \textcolor{red}{89.6} & 71.0 & 32.1 \\
% OCSort & 55.1 & 54.6  & 92.0 & 80.3 & 38.3 \\
\hline
GHOST & \textbf{56.7} & \textbf{57.7} & \textbf{91.3} & \textbf{81.1} & \textcolor{red}{39.8} \\
\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\caption{Comparison to state-of-the-art on DanceTrack.}
\vspace{-0.3cm}
\label{tab:dance}
\end{table}


==> cvpr2023-author_kit-v1_1-1/latex/tables/mot_challenge_comparison_detailed.tex <==
\begin{table}[thb!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule

 & \textbf{HOTA} $\uparrow$ &  \textbf{IDF1} $\uparrow$ & \textbf{MOTA} $\uparrow$ & \textbf{IDSW} $\downarrow$ \\

\hline
\hline
\textit{Public MOT17} \\
FAMNet \cite{DBLP:conf/iccv/ChuL19} & - & 48.7 & 52.0  & 3072  \\
OneShotDA \cite{DBLP:journals/access/YoonGSYJ20} & 36.9 & 54.0 & 51.4 & 2188 \\
MOTDT \cite{DBLP:conf/icmcs/ChenAZS18} & 41.2 & 52.7 &  50.9& 2474\\
TAMA \cite{DBLP:journals/isci/YoonKSYJ21} & 42.0 & 53.5 & 50.3 & 2192  \\
DeepMOT$^{\dagger}$ \cite{DBLP:conf/cvpr/XuOBHLA20} & 42.4 & 53.8 & 53.7  & \textcolor{black}{1947}  \\
UMA \cite{DBLP:conf/cvpr/YinWMYS20} & - & 54.4 & 53.1 & 2251  \\
STRN \cite{DBLP:conf/iccv/Xu0ZH19} & 42.6 & 56.0 &  50.9& 2397  \\
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & 44.8 & 55.1 & 56.3 & 1987  \\
GNNMatch$^{\dagger}$ \cite{DBLP:conf/cvpr/DaiWCZHD21} & 45.4 & 56.3 & 57.3 & 1911 \\
GSM$^{\dagger}$ \cite{DBLP:conf/ijcai/LiuC0Y20} &  45.7 & 57.8& 56.4 & \textcolor{red}{1485} \\
UNS$^{\dagger}$ \cite{DBLP:journals/corr/abs-2111-05943} & \textcolor{black}{46.4} & \textcolor{black}{58.3} & \textcolor{black}{56.8} & 19114 \\
UnsupTrack$^{\ddagger}$ \cite{DBLP:journals/corr/abs-2006-02609} & 46.9 & 58.1 & \textcolor{red}{61.7} & 1864 \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 60.1 & 58.8 & 47.2 & 2065 & 13503 & 209475 & 26.0 & 29.7 \\
TrackPool$^{\dagger}$ \cite{DBLP:conf/cvpr/KimLAR21} & - & \textcolor{red}{60.5} & 55.9 & \textbf{1188}   \\
CenterTrack$^{\ddagger}$ \cite{DBLP:conf/eccv/ZhouKK20}&\textcolor{blue}{48.2}&\textcolor{black}{59.6}& \textcolor{blue}{61.5} & 3039  \\
ArTIST-C$^{\ddagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{red}{48.9} & \textcolor{blue}{59.7} & \textbf{62.3} & 2062  \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 65.0 & 62.1 & 1768 \\
%TMHO \cite{DBLP:conf/cvpr/StadlerB21}&62.1&62.8& 50.4 & 1897 & 10951 & 201195 & 26.9 & 31.4 \\
\hline
% Ours Tracktor \textcolor{red}{OLD} & 56.3 & 61.1 & 47.3 &1920 & & & 21.1 & 35.5\\
GHOST$^{\dagger}$ & 47.0 & 59.6 & 56.4 &1517 \\
GHOST$^{\ddagger}$ & \textbf{50.9} & \textbf{64.2} & \textcolor{red}{61.7} & \textcolor{blue}{1639} \\
%Ours & 61.7 & 64.1 & 50.6 & 1788 & 14001 & 200571 & 26.4 & 31.8 \\

\hline
\hline
\textit{Private MOT17} \\

DAN \cite{DBLP:journals/pami/SunASMS21} & 39.3 & 49.5 & 52.4 & 8431\\
TubeTK \cite{DBLP:conf/cvpr/PangLZLL20} & 48.0  & 58.6 & 63.0 & 5727  \\
CTracker \cite{DBLP:conf/eccv/PengWWWWTWLHF20} & 49.0  & 57.4 & 66.6& 5529 \\
% TransCenter unpiblished \\
% MAT Motion-aware MOT unpublished \\
CenterTrack \cite{DBLP:conf/eccv/ZhouKK20} & 52.2  & 64.7 & 67.8 & \textcolor{blue}{3039}\\
TraDeS \cite{DBLP:conf/cvpr/WuCS00Y21} & 52.7 & 63.9 & 69.1 & 3555\\
% MOTR unpublished \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & 53.9 & 66.3 & 68.7 & 3378  \\
GSDT \cite{DBLP:conf/icra/0002KW21} &55.2  & 66.5 & 73.2 & 3891  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{blue}{59.3} & \textcolor{blue}{72.3} & 73.7 & 3303  \\
CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & 60.3 & \textcolor{red}{73.6} & \textcolor{blue}{75.6} & \textcolor{red}{2544}  \\
CorrTracker \cite{DBLP:conf/cvpr/WangZPX21} & \textcolor{red}{60.7} & \textcolor{red}{73.6}  & \textcolor{red}{76.5} & 3369  \\
% GRTU \cite{Wang2021AGR} & \textbf{62.0} & \textcolor{red}{75.0} & 74.9  & \textbf{1812} & 32007 &	107616 & \textbf{49.7} & 18.9 \\
% OUTrack \cite{DBLP:journals/corr/abs-2201-01297} & 58.7 & 70.2 & 73.5 & 4122 & 34731 & 110586 & 43.3 & 15.0 \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  56.9 & 72.5 & 69.0 & 2724 \\
GTR \cite{DBLP:conf/cvpr/ZhouYKK22} & 59.1 & 71.5 & 75.3 & 2859 \\
MTrack \cite{DBLP:conf/cvpr/YuLH22} & & 73.5 & 72.1 & 2028 \\
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & 62.8 & 77.1 & 78.9	& 2363 \\
% \textcolor{pink}{ByteTrack + tricks} \cite{DBLP:journals/corr/abs-2110-06864} & 63.1 & 77.3 & 80.3 & 2196 \\
Unicorn \cite{DBLP:conf/eccv/YanJSWYLL22} & 61.7 & 75.5 & 77.2 & 5379 \\
MOTR \cite{DBLP:journals/corr/abs-2105-03247} & 57.8 & 68.6 & 73.4 & 2439 \\
P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & 78.1 & 81.2  & 1893 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 75.9 & 77.3 & 3255 \\
\hline
GHOST & \textbf{62.8} & \textbf{77.1} & \textbf{78.7} & \textbf{2325} \\
%GHOST & \textbf{62.4} & \textbf{76.4} & \textbf{78.8} & \textbf{2199} \\
%Ours & 78.2 & 76.0 & 62.1 & 2346 & 18840 &	101979 & 47.5 & 14.1 \\

\hline
\hline
\textit{Public MOT20} \\
TFT \cite{DBLP:conf/icpram/Lohn-JaramilloJ21} & 33.0 & 35.6 & 45.1 & 6492 \\
GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492  \\ 
%GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492 & 42778 & 236116 & 23.6 & \textcolor{red}{22.1} \\
SORT \cite{DBLP:conf/icip/BewleyGORU16} &36.1  & 45.1 & 42.7 & 4470 \\
ArTIST$^{\dagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{blue}{41.6} & \textcolor{blue}{51.0} & \textbf{53.6} & \textcolor{red}{1531}  \\ 
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & \textcolor{red}{42.1} & \textcolor{red}{52.7} & \textcolor{blue}{52.6} & \textcolor{blue}{1648} \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% mfi\_tst \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% TMOH \cite{DBLP:conf/cvpr/StadlerB21} & 60.1 & 61.2 & 48.9 & 2342 & 38043 & 165899  & 46.7 & 17.8 \\
% MPTC \cite{DBLP:conf/avss/StadlerB21} &  60.6 & 59.7 & 48.5 & 4533 & 45318 & 153978 & 51.1 & 16.7 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 65.0 & 55.6 & 480 \\
\hline
GHOST$^{\dagger}$ & \textbf{43.4} & \textbf{55.3} & \textcolor{red}{52.7} & \textbf{1437}\\
%Ours & 52.7 & 54.9 & 43.3 & 1456 & 6763 & 236454 & 29.1 & 26.8 \\
\hline
\hline
\textit{Private MOT20} \\
%MPTC \cite{DBLP:conf/avss/StadlerB21} & 48.5 & 59.7 & 60.6 	& 4533 & 46.5 & 51.1 & 15.7 \\
%TMOH \cite{DBLP:conf/cvpr/StadlerB21} &48.9  & 61.2 & 60.1 & \textcolor{blue}{2342} & 48.4 & 46.7 & 17.8 \\
MLT \cite{DBLP:journals/iotj/ZhangSWWKX20} & 43.2 & 54.6 & 48.9 & \textcolor{red}{2187} \\
GSDT \cite{DBLP:conf/icra/0002KW21} & 53.6 & \textcolor{blue}{67.5} & \textcolor{blue}{67.1} & 3230  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{blue}{54.6} & 67.3 & 61.8 & 5243  \\
CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & \textcolor{red}{55.0} & \textcolor{red}{68.2} & \textcolor{red}{70.7} & 3198  \\
% OUTrack & \textcolor{red}{56.2} & \textcolor{red}{69.4} & \textcolor{blue}{68.6} & \textcolor{blue}{2223} & 36816 & \textcolor{red}{123208} & \textcolor{red}{57.9} & \textcolor{blue}{12.2} \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  54.1 & 66.1 & 63.7 & 1938 \\
MTrack \cite{DBLP:conf/cvpr/YuLH22} & & 69.2 & 63.5 & 6031 \\
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & 60.4 & 74.5 & 74.2	& 925 \\
%\textcolor{pink}{ByteTrack + tricks} \cite{DBLP:journals/corr/abs-2110-06864} & 61.3 & 75.2 & 77.8 & 1223 \\
P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & 76.4 & 78.1 & 1332 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 67.7 & 66.3 & 2715 \\
\hline
% GHOST &  \textbf{60.0} & \textbf{73.7} & \textbf{71.5} & \textbf{1137} \\
%GHOST & 60.3 & 73.7 & 73.1 & 1332 \\ % new track thresh + lower conf
GHOST & 61.2 & 75.2 & 73.7 & 1264 \\ % new track thresh + lower conf
\bottomrule

\end{tabular}}

\vspace{0.5cm}

\caption{Comparison to state-of-the-art public and private detection trackers on both MOT17 and MOT20. $^{\dagger}$ and $^{\ddagger}$ indicate bounding boxes refined by Tracktor \cite{DBLP:conf/iccv/BergmannML19} and CenterTrack \cite{DBLP:conf/eccv/ZhouKK20}, respectively.}

\label{tab:sota}
\end{table}






==> cvpr2023-author_kit-v1_1-1/latex/tables/private_detectors.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c@{}}
\hline

 &  \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \downarrow & & & \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \\
\hline
JDE & 64.1 & 50.5 & 537 &&  QDTrack & 67.8 & 56.3 & 386  \\
JDE with ours &  66.8 & 51.9 & 315 && QDTrack with ours &  72.8 & 58.7 & 288  \\
\hline
FairMOT & 72.8 & 57.2 & 318  && TraDeS &  71.9 & 58.7 & 293  \\
FairMOT with ours  & 74.1 & 60.0 & 246  && TraDeS with ours & 75.5 & 61.0 & 168 \\
\hline
TransTrack &  68.6 & 58.1 & 261 && CSTrack &  72.3 & 59.0 & 423 \\
TransTrack with ours  & 72.7 & 59.9 & 209  && CSTrack with ours &  72.8 & 58.9 & 275 \\
\hline
CenterTrack & 64.5 & 55.3 & 528&& \\
CenterTrack with ours & 74.6 & 60.4 & 173 &&\\
\hline
\end{tabular}}


\caption{Potential of our approach when applied upon several state-of-the-art private trackers.}
\label{tab:private}

\end{table*}


\iffalse
\begin{table}[hbt!]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c@{}}
\hline

 & \textbf{MOTA} \uparrow &  \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \downarrow & \textbf{FP} \downarrow & \textbf{FN} \downarrow &  \textbf{MTR} \uparrow & \textbf{MLR} \downarrow\\
\hline
JDE & 59.9 & 64.1 & 50.5 & 537 & 2950 & 18117 & 31.6 & 18.3 \\
JDE with ours & 60.4 & 66.8 & 51.9 & 315 & 2903 & 18145 & 32.2 & 18.0 \\
\hline
FairMOT & 69.1 & 72.8 & 57.2 & 318 & 1957 & 14358 & 41.3 & 15.9 \\
FairMOT with ours & 69.5 & 74.1 & 60.0 & 246 & 1823 & 14394 & 41.0 & 16.5 \\
\hline
TransTrack & 67.7 & 68.6 & 58.1 & 261 & 1313 & 15820 & 41.9 & 18.3 \\
TransTrack with ours & 67.9 & 72.7 & 59.9 & 209 & 1253 & 15853 & 41.9 & 18.6 \\
\hline
QDTrack & 67.2 & 67.8 & 56.3 & 386 & 2637 & 14605 & 44.0 & 14.8 \\
QDTrack with ours & 67.5 & 72.8 & 58.7 & 288 & 2603 & 14635 & 43.7 & 15.6 \\
\hline
TraDeS & 68.5 & 71.9 & 58.7 & 293 & 1691 & 14977 & 42.2 & 19.2 \\
TraDeS with ours & 68.8 & 75.5 & 61.0 & 168 & 1658 & 14995 & 42.2 & 19.5 \\
\hline
CSTrack & 68.2 & 72.3 & 59.0 & 423 & 2476 & 14152 & 40.1 & 16.6 \\
CSTrack with ours & 68.5 & 72.8 & 58.9 & 275 & 2432 & 14201 & 40.2 & 17.2 \\
\hline
CenterTrack & 66.7 & 64.5 & 55.3 & 528 & 2075 & 15288 & 41.3 & 38.1 \\
CenterTrack with ours & 67.5 & 74.6 & 60.4 & 173 & 2044 & 15320 & 41.3 & 20.9 \\
\hline
\end{tabular}}


\caption{Ours on detections pre-processed by several private detections.\alj{This is cool!!!}}
\label{tab:private}
\end{table}
\fi

==> cvpr2023-author_kit-v1_1-1/latex/tables/public_detections.tex <==
\begin{table}[thb!]
\centering
\resizebox{0.385\textwidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule

 & \textbf{HOTA} $\uparrow$ &  \textbf{IDF1} $\uparrow$ & \textbf{MOTA} $\uparrow$ & \textbf{IDSW} $\downarrow$ \\

\hline
\hline
\textit{Public MOT17} \\
%FAMNet \cite{DBLP:conf/iccv/ChuL19} & - & 48.7 & 52.0  & 3072  \\
%OneShotDA \cite{DBLP:journals/access/YoonGSYJ20} & 36.9 & 54.0 & 51.4 & 2188 \\
%MOTDT \cite{DBLP:conf/icmcs/ChenAZS18} & 41.2 & 52.7 &  50.9& 2474\\
%TAMA \cite{DBLP:journals/isci/YoonKSYJ21} & 42.0 & 53.5 & 50.3 & 2192  \\
%DeepMOT$^{\dagger}$ \cite{DBLP:conf/cvpr/XuOBHLA20} & 42.4 & 53.8 & 53.7  & \textcolor{black}{1947}  \\
%UMA \cite{DBLP:conf/cvpr/YinWMYS20} & - & 54.4 & 53.1 & 2251  \\
%STRN \cite{DBLP:conf/iccv/Xu0ZH19} & 42.6 & 56.0 &  50.9& 2397  \\
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & 44.8 & 55.1 & 56.3 & 1987  \\
%GNNMatch$^{\dagger}$ \cite{DBLP:conf/cvpr/DaiWCZHD21} & 45.4 & 56.3 & 57.3 & 1911 \\
%GSM$^{\dagger}$ \cite{DBLP:conf/ijcai/LiuC0Y20} &  45.7 & 57.8& 56.4 & \textcolor{red}{1485} \\
UNS$^{\dagger}$ \cite{DBLP:journals/corr/abs-2111-05943} & \textcolor{black}{46.4} & \textcolor{black}{58.3} & \textcolor{black}{56.8} & 1914 \\
%UnsupTrack$^{\ddagger}$ \cite{DBLP:journals/corr/abs-2006-02609} & 46.9 & 58.1 & \textcolor{red}{61.7} & 1864 \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 60.1 & 58.8 & 47.2 & 2065 & 13503 & 209475 & 26.0 & 29.7 \\
TrackPool$^{\dagger}$ \cite{DBLP:conf/cvpr/KimLAR21} & - & \textcolor{blue}{60.5} & 55.9 & \textcolor{red}{1188}   \\
CenterTrack$^{\ddagger}$ \cite{DBLP:conf/eccv/ZhouKK20}&\textcolor{blue}{48.2}&\textcolor{black}{59.6}& \textcolor{blue}{61.5} & 3039  \\
ArTIST-C$^{\ddagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{red}{48.9} & \textcolor{black}{59.7} & \textbf{62.3} & 2062  \\
%MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & - & 65.0 & 62.1 & 1768 \\
%TMHO \cite{DBLP:conf/cvpr/StadlerB21}&62.1&62.8& 50.4 & 1897 & 10951 & 201195 & 26.9 & 31.4 \\
\hline
% Ours Tracktor \textcolor{red}{OLD} & 56.3 & 61.1 & 47.3 &1920 & & & 21.1 & 35.5\\
GHOST$^{\dagger}$ & 47.4 & \textcolor{red}{60.6} & 56.5 & \textbf{1144} \\ % \emoji{ghost}
GHOST$^{\ddagger}$ & \textbf{50.7} & \textbf{63.5} & \textcolor{red}{61.6} & \textcolor{blue}{1715} \\
%Ours & 61.7 & 64.1 & 50.6 & 1788 & 14001 & 200571 & 26.4 & 31.8 \\

\hline
\hline
\textit{Private MOT17} \\

%DAN \cite{DBLP:journals/pami/SunASMS21} & 39.3 & 49.5 & 52.4 & 8431\\
%TubeTK \cite{DBLP:conf/cvpr/PangLZLL20} & 48.0  & 58.6 & 63.0 & 5727  \\
%CTracker \cite{DBLP:conf/eccv/PengWWWWTWLHF20} & 49.0  & 57.4 & 66.6& 5529 \\
% TransCenter unpiblished \\
% MAT Motion-aware MOT unpublished \\
CenterTrack \cite{DBLP:conf/eccv/ZhouKK20} & 52.2  & 64.7 & 67.8 & 3039\\
TraDeS \cite{DBLP:conf/cvpr/WuCS00Y21} & 52.7 & 63.9 & 69.1 & 3555\\
% MOTR unpublished \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & 53.9 & 66.3 & 68.7 & 3378  \\
%GSDT \cite{DBLP:conf/icra/0002KW21} &55.2  & 66.5 & 73.2 & 3891  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{red}{59.3} & \textcolor{blue}{72.3} & 73.7 & 3303  \\
%CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & 60.3 & \textcolor{red}{73.6} & \textcolor{blue}{75.6} & \textcolor{red}{2544}  \\
%CorrTracker \cite{DBLP:conf/cvpr/WangZPX21} & \textcolor{red}{60.7} & \textcolor{red}{73.6}  & \textcolor{red}{76.5} & 3369  \\
% GRTU \cite{Wang2021AGR} & \textbf{62.0} & \textcolor{red}{75.0} & 74.9  & \textbf{1812} & 32007 &	107616 & \textbf{49.7} & 18.9 \\
% OUTrack \cite{DBLP:journals/corr/abs-2201-01297} & 58.7 & 70.2 & 73.5 & 4122 & 34731 & 110586 & 43.3 & 15.0 \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  56.9 & \textcolor{red}{72.5} & 69.0 & 2724 \\
GTR \cite{DBLP:conf/cvpr/ZhouYKK22} & \textcolor{blue}{59.1} & 71.5 & \textcolor{blue}{75.3} & \textcolor{blue}{2859} \\
%MTrack \cite{DBLP:conf/cvpr/YuLH22} & - & 73.5 & 72.1 & 2028 \\
MOTR \cite{DBLP:journals/corr/abs-2105-03247} & 57.8 & 68.6 & 73.4 & 2439 \\
ByteTrack$^{\star}$ \cite{DBLP:journals/corr/abs-2110-06864} & \textbf{62.8} & \textbf{77.1} & \textbf{78.9}	& \textcolor{red}{2363} \\
\textcolor{gray}{ByteTrack$^{\star}$} \cite{DBLP:journals/corr/abs-2110-06864} & \textcolor{gray}{63.1} & \textcolor{gray}{77.3} & \textcolor{gray}{80.3} & \textcolor{gray}{2196} \\
%Unicorn \cite{DBLP:conf/eccv/YanJSWYLL22} & \textcolor{red}{61.7} & 75.5 & 77.2 & 5379 \\
%P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & \textbf{78.1} & \textbf{81.2}  & 1893 \\
%MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & - & \textcolor{blue}{75.9} & 77.3 & 3255 \\
\hline
GHOST & \textbf{62.8} & \textbf{77.1} & \textcolor{red}{78.7} & \textbf{2325} \\
%GHOST & \textbf{62.4} & \textbf{76.4} & \textbf{78.8} & \textbf{2199} \\
%Ours & 78.2 & 76.0 & 62.1 & 2346 & 18840 &	101979 & 47.5 & 14.1 \\

\hline
\hline
\textit{Public MOT20} \\
%TFT \cite{DBLP:conf/icpram/Lohn-JaramilloJ21} & 33.0 & 35.6 & 45.1 & 6492 \\
GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492  \\ 
%GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492 & 42778 & 236116 & 23.6 & \textcolor{red}{22.1} \\
SORT \cite{DBLP:conf/icip/BewleyGORU16} &36.1  & 45.1 & 42.7 & 4470 \\
ArTIST$^{\dagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{blue}{41.6} & \textcolor{blue}{51.0} & \textbf{53.6} & \textcolor{red}{1531}  \\ 
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & \textcolor{red}{42.1} & \textcolor{red}{52.7} & \textcolor{blue}{52.6} & \textcolor{blue}{1648} \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% mfi\_tst \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% TMOH \cite{DBLP:conf/cvpr/StadlerB21} & 60.1 & 61.2 & 48.9 & 2342 & 38043 & 165899  & 46.7 & 17.8 \\
% MPTC \cite{DBLP:conf/avss/StadlerB21} &  60.6 & 59.7 & 48.5 & 4533 & 45318 & 153978 & 51.1 & 16.7 \\
%MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & - & 65.0 & 55.6 & 480 \\
\hline
GHOST$^{\dagger}$ & \textbf{43.4} & \textbf{55.3} & \textcolor{red}{52.7} & \textbf{1437}\\
%Ours & 52.7 & 54.9 & 43.3 & 1456 & 6763 & 236454 & 29.1 & 26.8 \\
\hline
\hline
\textit{Private MOT20} \\
%MPTC \cite{DBLP:conf/avss/StadlerB21} & 48.5 & 59.7 & 60.6 	& 4533 & 46.5 & 51.1 & 15.7 \\
%TMOH \cite{DBLP:conf/cvpr/StadlerB21} &48.9  & 61.2 & 60.1 & \textcolor{blue}{2342} & 48.4 & 46.7 & 17.8 \\
%MLT \cite{DBLP:journals/iotj/ZhangSWWKX20} & 43.2 & 54.6 & 48.9 & \textcolor{red}{2187} \\
GSDT \cite{DBLP:conf/icra/0002KW21} & 53.6 & 67.5 & 67.1 & 3230  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{blue}{54.6} & 67.3 & 61.8 & 5243  \\
%CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & \textcolor{blue}{55.0} & 68.2 & 70.7 & 3198  \\
% OUTrack & \textcolor{red}{56.2} & \textcolor{red}{69.4} & \textcolor{blue}{68.6} & \textcolor{blue}{2223} & 36816 & \textcolor{red}{123208} & \textcolor{red}{57.9} & \textcolor{blue}{12.2} \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  54.1 & 66.1 & \textcolor{blue}{63.7} & \textcolor{blue}{1938} \\
MTrack \cite{DBLP:conf/cvpr/YuLH22} & - & \textcolor{blue}{69.2} & 63.5 & 6031 \\
ByteTrack$^{\star}$ \cite{DBLP:journals/corr/abs-2110-06864} & \textcolor{red}{60.4} & \textcolor{red}{74.5} & \textbf{74.2}	& \textbf{925} \\
\textcolor{gray}{ByteTrack$^{\star}$} \cite{DBLP:journals/corr/abs-2110-06864} & \textcolor{gray}{61.3} & \textcolor{gray}{75.2} & \textcolor{gray}{77.8} & \textcolor{gray}{1223} \\
%P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & \textbf{76.4} & \textbf{78.1} & \textcolor{blue}{1332} \\
%MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & - & 67.7 & 66.3 & 2715 \\
\hline
% GHOST &  \textbf{60.0} & \textbf{73.7} & \textbf{71.5} & \textbf{1137} \\
%GHOST & 60.3 & 73.7 & 73.1 & 1332 \\ % new track thresh + lower conf
GHOST & \textbf{61.2} & \textbf{75.2} & \textcolor{red}{73.7} & \textcolor{red}{1264} \\ % new track thresh + lower conf
\bottomrule

\end{tabular}}
\vspace{-0.25cm}
\caption{Comparison to state-of-the-art for public and private detections on MOT17 and MOT20. $^{\dagger}$ and $^{\ddagger}$ indicate bounding boxes refined by Tracktor \cite{DBLP:conf/iccv/BergmannML19} and CenterTrack \cite{DBLP:conf/eccv/ZhouKK20}. $^{\star}$ since ByteTrack uses different thresholds for different sequences of the test set and interpolation we recomputed their results without both (recomputed black / \textcolor{gray}{original gray}).}
\vspace{-0.65cm}
\label{tab:sota}
\end{table}






==> cvpr2023-author_kit-v1_1-1/latex/tables/reid_balation.tex <==
\begin{table}[t!]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{@{}c|c|c|ccc|ccc@{}}
\hline

\multicolumn{3}{c}{} & \multicolumn{3}{|c|}{MOT 17} & \multicolumn{3}{|c}{BDD} \\
\hline

\textbf{diff $\tau$} & \textbf{IP} & \textbf{DA} & \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ & \textbf{MOTA} $\uparrow$ & \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ & \textbf{MOTA} $\uparrow$ \\
\hline
\hline
 & & & 61.6 & 72.2 & 69.5 & 41.3 & 47.7 & 42.0 \\
 \checkmark & & & 61.8 & 72.7 & 69.6 & 41.9 & 48.6 & 41.9  \\
 \checkmark & \checkmark & & 62.4 & 73.6 & 69.6 & 42.9 & 50.4 & 43.7 \\
 \checkmark & \checkmark & \checkmark & 63.3 & 75.3 & 69.6 & 43.7 & 51.5 & 43.9 \\
 
\hline
\end{tabular}}
\vspace{-0.1cm}
\caption{Ablation of the single parts of our method on the validation set of CenterTrack pre-processed bounding boxes. IP=inactive proxies, DA=domain adaptation.}
\vspace{-0.5cm}
\label{tab:reid_blation}
\end{table}


\iffalse
\begin{table*}[hbt!]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
\hline

 & \textbf{MOTA} \uparrow &  \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \downarrow & \textbf{FP} \downarrow & \textbf{FN} \downarrow &  \textbf{MTR} \uparrow & \textbf{MLR} \downarrow\\
\hline
Linear Motion Model & 69.4 & 73.5 & 62.4 & 255 & 1104 & 15117 & 44.4 & 15.3 \\
Kalman Filter & 69.4 & 73.8 & 62.5 & 285 & 1111 & 15105 & 44.1 & 15.3 \\
\hline
\end{tabular}}
\caption{Ablation of the our motion model on the validation set of CenterTrack pre-processed bounding boxes.}
\label{tab:motion}
\end{table*}
\fi

==> tables/ablation_last_n_motion.tex <==
\begin{table}[t!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}l|ccc@{}}
\hline

& \textbf{HOTA} $\uparrow$ & \textbf{IDF1} $\uparrow$ & \textbf{IDF1} $\uparrow$ \\
\hline
\hline

last 10000000 & 77.3 & 88.7 & 93.9 \\
last 10 frames & 77.6 & 89.3 & 94.0 \\
last 30 frames & 78.0 & 89.8 & 94.0 \\
last 60 frames & 77.7 & 89.4 & 94.0 \\
last 90 frames & 77.8 & 89.5 & 93.9 \\
last 120 frames & 77.7 & 89.4 & 93.9 \\
last 150 frames & 77.7 & 89.3 & 93.9 \\

\hline
\end{tabular}}
\caption{Ablation of using different number of frames for velocity computation on MOT20.}
\label{tab:last_n_frames_ablation}
\end{table}


==> tables/ablations.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}l|c|cc|cc|cc|cc|cc|cc|cc@{}}
\hline
& & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Basic ReID} & \multicolumn{2}{c}{Our ReID} & \multicolumn{2}{c}{Kalman} &\multicolumn{2}{c}{Linear Motion} & \multicolumn{2}{c}{Sum} & \multicolumn{2}{c}{Ours} \\

\hline
&Occ Det & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1 & MOTA &  IDF1\\
\hline
JDE & 0.20 & 59.9 & 64.1 & 60.1 & 62.1 & 60.0 & 63.9 & 59.9 & 64.9 & 60.1 & 65.9 & 60.3 & 67.1 & 60.4 & 66.8 \\
FairMOT & 0.27 & 69.1 & 72.8 & 69.2 & 67.0 & 69.2 & 68.5 & 69.2 & 73.8 & 69.3 & 73.0 & 69.5 & 73.2 & 69.5 & 74.1 \\
TransTrack & 0.17 & 67.7 & 68.6 & 67.6 & 67.6 & 67.7 & 69.5 & 67.4 & 71.4 &  67.7 & 71.1 & 68.0 & 73.7 & 67.9 & 72.7 \\
QDTrack & 0.24 & 67.2 & 67.8 & 67.3 & 64.8 & 67.3 & 68.2 & 67.0 & 70.1  & 67.3 & 71.0 & 67.5 & 71.2 & 67.5 & 72.8 \\
TraDeS & 0.18 & 68.5 & 71.9 & 68.6 & 72.0 & 68.7 & 71.9 & 68.5 & 72.8 & 68.4 & 72.9 & 68.8 & 74.9 & 68.8 & 75.5 \\
CSTrack & 0.25 & 68.2 & 72.3 & 68.3 & 66.5 & 68.2 & 68.2 & 68.3 & 72.0 & 68.3 & 72.8 & 68.4 & 73.4 & 68.5 & 72.8 \\
CenterTrack & 0.18 & 66.7 & 64.5 & 67.5 & 67.6 & 67.4 & 72.7 & 67.3 & 72.7 & 67.3 & 72.7 & 67.5 & 74.6 & 67.5 & 74.6 \\
\hline
\end{tabular}}


\caption{Analysis of the contribution of ReID and motion cues. Occ Det = average occlusion level of detected bounding boxes.}
\label{tab:ablations}
\vspace{-0.7cm}
\end{table}

==> tables/mot_challenge_comparison_detailed.tex <==
\begin{table}[thb!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule

 & \textbf{HOTA} $\uparrow$ &  \textbf{IDF1} $\uparrow$ & \textbf{MOTA} $\uparrow$ & \textbf{IDSW} $\downarrow$ \\

\hline
\hline
\textit{Public MOT17} \\
FAMNet \cite{DBLP:conf/iccv/ChuL19} & - & 48.7 & 52.0  & 3072  \\
OneShotDA \cite{DBLP:journals/access/YoonGSYJ20} & 36.9 & 54.0 & 51.4 & 2188 \\
MOTDT \cite{DBLP:conf/icmcs/ChenAZS18} & 41.2 & 52.7 &  50.9& 2474\\
TAMA \cite{DBLP:journals/isci/YoonKSYJ21} & 42.0 & 53.5 & 50.3 & 2192  \\
DeepMOT$^{\dagger}$ \cite{DBLP:conf/cvpr/XuOBHLA20} & 42.4 & 53.8 & 53.7  & \textcolor{black}{1947}  \\
UMA \cite{DBLP:conf/cvpr/YinWMYS20} & - & 54.4 & 53.1 & 2251  \\
STRN \cite{DBLP:conf/iccv/Xu0ZH19} & 42.6 & 56.0 &  50.9& 2397  \\
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & 44.8 & 55.1 & 56.3 & 1987  \\
GNNMatch$^{\dagger}$ \cite{DBLP:conf/cvpr/DaiWCZHD21} & 45.4 & 56.3 & 57.3 & 1911 \\
GSM$^{\dagger}$ \cite{DBLP:conf/ijcai/LiuC0Y20} &  45.7 & 57.8& 56.4 & \textcolor{red}{1485} \\
UNS$^{\dagger}$ \cite{DBLP:journals/corr/abs-2111-05943} & \textcolor{black}{46.4} & \textcolor{black}{58.3} & \textcolor{black}{56.8} & 19114 \\
UnsupTrack$^{\ddagger}$ \cite{DBLP:journals/corr/abs-2006-02609} & 46.9 & 58.1 & \textcolor{red}{61.7} & 1864 \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 60.1 & 58.8 & 47.2 & 2065 & 13503 & 209475 & 26.0 & 29.7 \\
TrackPool$^{\dagger}$ \cite{DBLP:conf/cvpr/KimLAR21} & - & \textcolor{red}{60.5} & 55.9 & \textbf{1188}   \\
CenterTrack$^{\ddagger}$ \cite{DBLP:conf/eccv/ZhouKK20}&\textcolor{blue}{48.2}&\textcolor{black}{59.6}& \textcolor{blue}{61.5} & 3039  \\
ArTIST-C$^{\ddagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{red}{48.9} & \textcolor{blue}{59.7} & \textbf{62.3} & 2062  \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 65.0 & 62.1 & 1768 \\
%TMHO \cite{DBLP:conf/cvpr/StadlerB21}&62.1&62.8& 50.4 & 1897 & 10951 & 201195 & 26.9 & 31.4 \\
\hline
% Ours Tracktor \textcolor{red}{OLD} & 56.3 & 61.1 & 47.3 &1920 & & & 21.1 & 35.5\\
GHOST$^{\dagger}$ & 47.0 & 59.6 & 56.4 &1517 \\
GHOST$^{\ddagger}$ & \textbf{50.9} & \textbf{64.2} & \textcolor{red}{61.7} & \textcolor{blue}{1639} \\
%Ours & 61.7 & 64.1 & 50.6 & 1788 & 14001 & 200571 & 26.4 & 31.8 \\

\hline
\hline
\textit{Private MOT17} \\

DAN \cite{DBLP:journals/pami/SunASMS21} & 39.3 & 49.5 & 52.4 & 8431\\
TubeTK \cite{DBLP:conf/cvpr/PangLZLL20} & 48.0  & 58.6 & 63.0 & 5727  \\
CTracker \cite{DBLP:conf/eccv/PengWWWWTWLHF20} & 49.0  & 57.4 & 66.6& 5529 \\
% TransCenter unpiblished \\
% MAT Motion-aware MOT unpublished \\
CenterTrack \cite{DBLP:conf/eccv/ZhouKK20} & 52.2  & 64.7 & 67.8 & \textcolor{blue}{3039}\\
TraDeS \cite{DBLP:conf/cvpr/WuCS00Y21} & 52.7 & 63.9 & 69.1 & 3555\\
% MOTR unpublished \\
QDTrack \cite{DBLP:conf/cvpr/PangQLCLDY21} & 53.9 & 66.3 & 68.7 & 3378  \\
GSDT \cite{DBLP:conf/icra/0002KW21} &55.2  & 66.5 & 73.2 & 3891  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{blue}{59.3} & \textcolor{blue}{72.3} & 73.7 & 3303  \\
CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & 60.3 & \textcolor{red}{73.6} & \textcolor{blue}{75.6} & \textcolor{red}{2544}  \\
CorrTracker \cite{DBLP:conf/cvpr/WangZPX21} & \textcolor{red}{60.7} & \textcolor{red}{73.6}  & \textcolor{red}{76.5} & 3369  \\
% GRTU \cite{Wang2021AGR} & \textbf{62.0} & \textcolor{red}{75.0} & 74.9  & \textbf{1812} & 32007 &	107616 & \textbf{49.7} & 18.9 \\
% OUTrack \cite{DBLP:journals/corr/abs-2201-01297} & 58.7 & 70.2 & 73.5 & 4122 & 34731 & 110586 & 43.3 & 15.0 \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  56.9 & 72.5 & 69.0 & 2724 \\
GTR \cite{DBLP:conf/cvpr/ZhouYKK22} & 59.1 & 71.5 & 75.3 & 2859 \\
MTrack \cite{DBLP:conf/cvpr/YuLH22} & & 73.5 & 72.1 & 2028 \\
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & 62.8 & 77.1 & 78.9	& 2363 \\
% \textcolor{pink}{ByteTrack + tricks} \cite{DBLP:journals/corr/abs-2110-06864} & 63.1 & 77.3 & 80.3 & 2196 \\
Unicorn \cite{DBLP:conf/eccv/YanJSWYLL22} & 61.7 & 75.5 & 77.2 & 5379 \\
MOTR \cite{DBLP:journals/corr/abs-2105-03247} & 57.8 & 68.6 & 73.4 & 2439 \\
P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & 78.1 & 81.2  & 1893 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 75.9 & 77.3 & 3255 \\
\hline
GHOST & \textbf{62.8} & \textbf{77.1} & \textbf{78.7} & \textbf{2325} \\
%GHOST & \textbf{62.4} & \textbf{76.4} & \textbf{78.8} & \textbf{2199} \\
%Ours & 78.2 & 76.0 & 62.1 & 2346 & 18840 &	101979 & 47.5 & 14.1 \\

\hline
\hline
\textit{Public MOT20} \\
TFT \cite{DBLP:conf/icpram/Lohn-JaramilloJ21} & 33.0 & 35.6 & 45.1 & 6492 \\
GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492  \\ 
%GMPHD \cite{DBLP:journals/jvcir/Baisa21a} & 35.6 & 43.5 & 44.7 & 7492 & 42778 & 236116 & 23.6 & \textcolor{red}{22.1} \\
SORT \cite{DBLP:conf/icip/BewleyGORU16} &36.1  & 45.1 & 42.7 & 4470 \\
ArTIST$^{\dagger}$ \cite{DBLP:conf/cvpr/SalehARSG21} & \textcolor{blue}{41.6} & \textcolor{blue}{51.0} & \textbf{53.6} & \textcolor{red}{1531}  \\ 
Tracktor v2$^{\dagger}$ \cite{DBLP:conf/iccv/BergmannML19} & \textcolor{red}{42.1} & \textcolor{red}{52.7} & \textcolor{blue}{52.6} & \textcolor{blue}{1648} \\
%mfi \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% mfi\_tst \cite{DBLP:journals/apin/YangGYTS22} & 59.3 & 59.1 & 47.1 & 1919 & 36150 & 172782 & 41.1 & 17.3 \\
% TMOH \cite{DBLP:conf/cvpr/StadlerB21} & 60.1 & 61.2 & 48.9 & 2342 & 38043 & 165899  & 46.7 & 17.8 \\
% MPTC \cite{DBLP:conf/avss/StadlerB21} &  60.6 & 59.7 & 48.5 & 4533 & 45318 & 153978 & 51.1 & 16.7 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 65.0 & 55.6 & 480 \\
\hline
GHOST$^{\dagger}$ & \textbf{43.4} & \textbf{55.3} & \textcolor{red}{52.7} & \textbf{1437}\\
%Ours & 52.7 & 54.9 & 43.3 & 1456 & 6763 & 236454 & 29.1 & 26.8 \\
\hline
\hline
\textit{Private MOT20} \\
%MPTC \cite{DBLP:conf/avss/StadlerB21} & 48.5 & 59.7 & 60.6 	& 4533 & 46.5 & 51.1 & 15.7 \\
%TMOH \cite{DBLP:conf/cvpr/StadlerB21} &48.9  & 61.2 & 60.1 & \textcolor{blue}{2342} & 48.4 & 46.7 & 17.8 \\
MLT \cite{DBLP:journals/iotj/ZhangSWWKX20} & 43.2 & 54.6 & 48.9 & \textcolor{red}{2187} \\
GSDT \cite{DBLP:conf/icra/0002KW21} & 53.6 & \textcolor{blue}{67.5} & \textcolor{blue}{67.1} & 3230  \\
FairMOT \cite{DBLP:journals/ijcv/ZhangWWZL21} & \textcolor{blue}{54.6} & 67.3 & 61.8 & 5243  \\
CrowdTrack \cite{DBLP:conf/avss/StadlerB21a} & \textcolor{red}{55.0} & \textcolor{red}{68.2} & \textcolor{red}{70.7} & 3198  \\
% OUTrack & \textcolor{red}{56.2} & \textcolor{red}{69.4} & \textcolor{blue}{68.6} & \textcolor{blue}{2223} & 36816 & \textcolor{red}{123208} & \textcolor{red}{57.9} & \textcolor{blue}{12.2} \\
MeMOT \cite{DBLP:conf/cvpr/CaiX0XXTS22} &  54.1 & 66.1 & 63.7 & 1938 \\
MTrack \cite{DBLP:conf/cvpr/YuLH22} & & 69.2 & 63.5 & 6031 \\
ByteTrack \cite{DBLP:journals/corr/abs-2110-06864} & 60.4 & 74.5 & 74.2	& 925 \\
%\textcolor{pink}{ByteTrack + tricks} \cite{DBLP:journals/corr/abs-2110-06864} & 61.3 & 75.2 & 77.8 & 1223 \\
P3AFromer \cite{DBLP:conf/eccv/ZhaoWZLJ22} & - & 76.4 & 78.1 & 1332 \\
MTracker \cite{DBLP:conf/eccv/ZhangWWZL22} & & 67.7 & 66.3 & 2715 \\
\hline
% GHOST &  \textbf{60.0} & \textbf{73.7} & \textbf{71.5} & \textbf{1137} \\
%GHOST & 60.3 & 73.7 & 73.1 & 1332 \\ % new track thresh + lower conf
GHOST & 61.2 & 75.2 & 73.7 & 1264 \\ % new track thresh + lower conf
\bottomrule

\end{tabular}}

\vspace{0.5cm}

\caption{Comparison to state-of-the-art public and private detection trackers on both MOT17 and MOT20. $^{\dagger}$ and $^{\ddagger}$ indicate bounding boxes refined by Tracktor \cite{DBLP:conf/iccv/BergmannML19} and CenterTrack \cite{DBLP:conf/eccv/ZhouKK20}, respectively.}

\label{tab:sota}
\end{table}






==> tables/private_detectors.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c@{}}
\hline

 &  \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \downarrow & & & \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \\
\hline
JDE & 64.1 & 50.5 & 537 &&  QDTrack & 67.8 & 56.3 & 386  \\
JDE with ours &  66.8 & 51.9 & 315 && QDTrack with ours &  72.8 & 58.7 & 288  \\
\hline
FairMOT & 72.8 & 57.2 & 318  && TraDeS &  71.9 & 58.7 & 293  \\
FairMOT with ours  & 74.1 & 60.0 & 246  && TraDeS with ours & 75.5 & 61.0 & 168 \\
\hline
TransTrack &  68.6 & 58.1 & 261 && CSTrack &  72.3 & 59.0 & 423 \\
TransTrack with ours  & 72.7 & 59.9 & 209  && CSTrack with ours &  72.8 & 58.9 & 275 \\
\hline
CenterTrack & 64.5 & 55.3 & 528&& \\
CenterTrack with ours & 74.6 & 60.4 & 173 &&\\
\hline
\end{tabular}}


\caption{Potential of our approach when applied upon several state-of-the-art private trackers.}
\label{tab:private}

\end{table*}


\iffalse
\begin{table}[hbt!]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c@{}}
\hline

 & \textbf{MOTA} \uparrow &  \textbf{IDF1} \uparrow & \textbf{HOTA} \uparrow & \textbf{IDSW} \downarrow & \textbf{FP} \downarrow & \textbf{FN} \downarrow &  \textbf{MTR} \uparrow & \textbf{MLR} \downarrow\\
\hline
JDE & 59.9 & 64.1 & 50.5 & 537 & 2950 & 18117 & 31.6 & 18.3 \\
JDE with ours & 60.4 & 66.8 & 51.9 & 315 & 2903 & 18145 & 32.2 & 18.0 \\
\hline
FairMOT & 69.1 & 72.8 & 57.2 & 318 & 1957 & 14358 & 41.3 & 15.9 \\
FairMOT with ours & 69.5 & 74.1 & 60.0 & 246 & 1823 & 14394 & 41.0 & 16.5 \\
\hline
TransTrack & 67.7 & 68.6 & 58.1 & 261 & 1313 & 15820 & 41.9 & 18.3 \\
TransTrack with ours & 67.9 & 72.7 & 59.9 & 209 & 1253 & 15853 & 41.9 & 18.6 \\
\hline
QDTrack & 67.2 & 67.8 & 56.3 & 386 & 2637 & 14605 & 44.0 & 14.8 \\
QDTrack with ours & 67.5 & 72.8 & 58.7 & 288 & 2603 & 14635 & 43.7 & 15.6 \\
\hline
TraDeS & 68.5 & 71.9 & 58.7 & 293 & 1691 & 14977 & 42.2 & 19.2 \\
TraDeS with ours & 68.8 & 75.5 & 61.0 & 168 & 1658 & 14995 & 42.2 & 19.5 \\
\hline
CSTrack & 68.2 & 72.3 & 59.0 & 423 & 2476 & 14152 & 40.1 & 16.6 \\
CSTrack with ours & 68.5 & 72.8 & 58.9 & 275 & 2432 & 14201 & 40.2 & 17.2 \\
\hline
CenterTrack & 66.7 & 64.5 & 55.3 & 528 & 2075 & 15288 & 41.3 & 38.1 \\
CenterTrack with ours & 67.5 & 74.6 & 60.4 & 173 & 2044 & 15320 & 41.3 & 20.9 \\
\hline
\end{tabular}}


\caption{Ours on detections pre-processed by several private detections.\alj{This is cool!!!}}
\label{tab:private}
\end{table}
\fi
